Decoding the Secrets of Machine Learning in Malware Classification: A Deep Dive into Datasets, Feature Extraction, and Model Performance

Many studies have proposed machine-learning (ML) models for malware detection and classification, reporting an almost-perfect performance. However, they assemble ground-truth in different ways, use diverse static- and dynamic-analysis techniques for feature extraction, and even differ on what they consider a malware family. As a consequence, our community still lacks an understanding of malware classification results: whether they are tied to the nature and distribution of the collected dataset, to what extent the number of families and samples in the training dataset influence performance, and how well static and dynamic features complement each other. This work sheds light on those open questions. by investigating the key factors influencing ML-based malware detection and classification. For this, we collect the largest balanced malware dataset so far with 67K samples from 670 families (100 samples each), and train state-of-the-art models for malware detection and family classification using our dataset. Our results reveal that static features perform better than dynamic features, and that combining both only provides marginal improvement over static features. We discover no correlation between packing and classification accuracy, and that missing behaviors in dynamically-extracted features highly penalize their performance. We also demonstrate how a larger number of families to classify make the classification harder, while a higher number of samples per family increases accuracy. Finally, we find that models trained on a uniform distribution of samples per family better generalize on unseen data.

==> sec/combined.tex <==
\clearpage
\section{Combining static and dynamic features} 
\label{sec:static}

\subsection{Feature merging}
Explain the that we take the top 70,170,..,670 according to dynamic analysis and
compute static features accordingly. We then run the classifier for both binary
and family classification

\subsection{Binary classification}
Results clearly improve for binary classification. The reported confusion matrix
refers to the case with 70 families (best case). For 670 families accuracy drops
just of 1.5\%
\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/combined-binary-accuracy-heatmap.pdf}
	\caption{Accuracy heatmap for family classification when combining features}
\label{fig:multiclassAccuracy}
\end{figure}
\input{tbl/tbl_combined_binary_featImportance}

\subsection{Family classification}
Results clearly improve for a few families (e.g., 70,170). But then it looks
like the contribution of dynamic features does not add anything to static.
Results are available for the best and worst families for all the cases (e.g.,
70,170, and so on). However since the number of families is different, it's
difficult to have a single table.

\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/combined-multiclass-accuracy-heatmap.pdf}
	\caption{Accuracy heatmap for family classification when combining features}
\label{fig:multiclassAccuracy}
\end{figure}
\input{tbl/tbl_combined_multiclass_featImportance}



==> sec/comparison.tex <==
\section{Static vs Dynamic comparison} 
\label{sec:comparison}




==> sec/dynamic.tex <==
\section{Dynamic Results}
\label{sec:dynamic}


\subsection{The Results of Malware Family and Binary Classification without Preprocessing}
\noindent \textbf{Binary Classification.} A 500-tree \textit{Random Forest}-based classifier is built over the positive and negative data to achieve binary classification. The output from the classifier is to decide whether a sample is malicious (positive class) or benign (negative class).  To balance the training set, we inherit the same setting of training and testing data split in the test using statistical analysis features, as given in Section 4.1. The true positive rate (TPR), true negative rate (TNR), false negative rate (FNR) and false positive rate (FPR) of the detection results over the testing data are 0.9528, 0.9479, 0.0472 and 0.0521 respectively. We provide Precision, Recall and F1-score of the detection result in Table.\ref{tbl/tbl_binary_accuracy_dynamic}. 




%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/f1_heatmap_bin_prep.pdf}
%	\caption{F1 score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:binclassF1_prep}
%\end{figure}

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/acc_heatmap_bin_prep.pdf}
%	\caption{Acc score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:binclassAcc_prep}
%\end{figure}

%Figure.\ref{fig:binaryclassF1} and Figure.\ref{fig:binaryclassAcc} give the \textit{F1} score and \textit{Accuracy} scores of the binary classification task obtained with different combinations of $K$ and $M$.

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/f1_heatmap_bin_nprep.pdf}
%	\caption{F1 score heatmap for \textbf{binary classification} using Random Forest on dynamic analysis features}
%\label{fig:binaryclassF1}
%\end{figure}

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/acc_heatmap_bin_nprep.pdf}
%	\caption{Acc score heatmap for \textbf{binary classification} using Random Forest on dynamic analysis features}
%\label{fig:binaryclassAcc}
%\end{figure}


\noindent \textbf{Family Classification.} Theoretically, increasingly more classes in building a machine learning classifier augments the difficulty of learning accurately the boundaries between different classes. We empirically observe the impact of the varying number of malware families over the classifier accuracy. We randomly select $K$ out of 670 families, where $K$ ranges as 70, 170, 270, 370, 470, 570 and 670. Given each level of the number of families, we repeat the family sampling step for $N$ rounds. For $K\geq{450}$ and $K<{450}$, we set $N=5$ and $N=15$ to provide as comprehensive as possible coverage the families in the dataset. Furthermore, freezing the value $K$, we randomly choose $M$ out of 100 malware samples per family as the training data. The rest $100-M$ malware samples are considered as the testing instances. We start from $M=100$ and gradually decrease $M$ as $M$=80,70,60 and 50, to demonstrate whether the varying number of training samples would bring significant changes to the resultant multi-class classification accuracy. 

%We provide the F1-score results with different settings of $N$ and $M$ using \textit{Random Forest}, \textit{GradientBoosted Trees} and \textit{2-layered Neural Network} with ReLU activation nodes in Figure.\ref{fig:multiclassF1rf}, Figure.\ref{fig:multiclassF1gbt} and Figure.\ref{fig:multiclassF12nn} respectively. The value and the varying tendency of the accuracy scores are close to those of the F1-scores. We thus choose to show the F1-score results without loss of clarity. 

We provide the \textit{F1} score and \textit{Accuracy} score results with different settings of $K$ and $M$ using \textit{Random Forest} in Figure.\ref{fig:multiclassF1_prep}. We leave the accuracy scores derived with different $K$ and $M$ in Figure.\ref{fig:multiclassAcc_prep}, given in the appendix.  

\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/f1_heatmap_fam_prep.pdf}
	\caption{F1 score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
\label{fig:multiclassF1_prep}
\end{figure}

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/acc_heatmap_fam_prep.pdf}
%	\caption{Acc score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:multiclassAcc_prep}
%\end{figure}

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/f1_heatmap_fam_nprep.pdf}
%	\caption{F1 score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:multiclassF1}
%\end{figure}

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/acc_heatmap_fam_nprep.pdf}
%	\caption{Accuracy score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:multiclassAcc}
%\end{figure}


%\subsection{The Results of Family and Binary Classification with Preprocessing}

%Instead of randomly selecting $K$ families, we perform the preprocessing of feature completeness check. We rank the families by the average level of missing observation per family and choose the top $K$ families with the most completed feature observations for family and binary classification. In each of the selected family, we choose $M$ malware samples to build the malware training / testing data. For the convenience of comparative study, we inherit the same settings of $K$ and $M$ in the family classification task from Figure.\ref{fig:multiclassF1} and Figure.\ref{fig:multiclassAcc}. For the binary classification task, we use the same settings from Figure.\ref{fig:binaryclassF1} and Figure.\ref{fig:binaryclassAcc}. In the followings, Figure.\ref{fig:multiclassF1_prep} and Figure.\ref{fig:multiclassAcc_prep} provide the heatmaps of \textit{F1} and \textit{Accuracy} score of the family classification task with the preprocessing step to exclude the families with a high level of missing observations in the feature vectors.  Figure.\ref{fig:binclassF1_prep} and Figure.\ref{fig:binclassAcc_prep} provide the heatmaps of \textit{F1} and \textit{Accuracy} score of the binary classification task. By comparing the classification performances with and without the feature completeness check, we can find that performing classification tests over the families of the most completed features produces significantly better classification performances than randomly selected families with more missing features. The results show the completeness of dynamic analysis features is important to build accurate ML-based classification models. As a data-driven method, ML-based classifiers are designed to capture statistical correlation between features and the expected output, e.g. the predicted class labels. The existence of missing features lead to loss of the statistical correlation and make the trained classifier unstable and inaccurate. 

 
%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/f1_heatmap_fam_prep.pdf}
%	\caption{F1 score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:multiclassF1_prep}
%\end{figure}

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/acc_heatmap_fam_prep.pdf}
%	\caption{Acc score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:multiclassAcc_prep}
%\end{figure}


%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/f1_heatmap_bin_prep.pdf}
%	\caption{F1 score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:binclassF1_prep}
%\end{figure}

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/acc_heatmap_bin_prep.pdf}
%	\caption{Acc score heatmap for \textbf{family classification} using Random Forest on dynamic analysis features}
%\label{fig:binclassAcc_prep}
%\end{figure}

\subsection{The Results of Binary Classification over Singletons and Unseen families}
We choose the most complete 170 families of malware samples as the positive training set in the binary classification test, which considers the trade-off between feature completeness and coverage of malware families. We train a binary classifier using the samples of the 170 malware families and 10,697 benignwares, following the definition of the training dataset given in the classification experiment setup. Once it is obtained, we apply the binary classifier over the singletons and unseen families to evaluate the detection accuracy. It is worth noting that all the singletons are malware. Same as the unseen families, the malware campaigns of the singletons never appear in the training dataset of the classifier. We thus aim to measure the out-of-distribution (OOD) performance of the classifier. We repeat the sampling of the training data for 5 times and report the averaged detection accuracy. As a result, the average accuracy score is 97.74\% over singleton files with the standard deviation of 0.08 and 98.23\% over unseen families with the standard deviation of 0.10 respectively 

\subsection{The Results of Family Classification over Singleton and Unseen families}
We are unable to measure the family classification accuracy over the singletons and malware of unseen families. No ground truth family labels of these testing samples are given by AVClass. However, we find that the uncertainty level of the family classification output over the out-of-distribution testing malware samples increase significantly, compared to those derived with the testing samples sharing the same families of the training data. To measure the uncertainty difference, we define Relative Entropy Score (RES) as below: 
\begin{equation}\label{eq:RES}
RES = \frac{\sum_{k=1}^{C} p_{k}\log{p_{k}}}{ \sum_{k=1}^{C} 1/C\log{1/C}}
\end{equation}
where $C$ is the number of the families covered by the training data building the classifier. In this experiment, as we choose the most complete 170 families of malware samples to train the family classifier, $C$ is therefore set to 170 in Eq.\ref{eq:RES}.  For a sample of singletons / unseen families, the output of the family classifier is a 170-dimensional probability-valued vector $\{p_{k}\}$ (k=1,2,3,...,C). Each $p_{k}$ gives the probabilistic confidence that the sample belongs to the corresponding family.  By definition, the numerator $\sum_{k=1}^{C} p_{k}\log{p_{k}}$ provides the entropy of the classifier's output. The denominator $\sum_{k=1}^{C} 1/C\log{1/C}$ denotes the maximum entropy that the classifier's classification output may have. More specifically, the denominator gives the entropy achieved if every class has uniformly the same decision confidence. As a result, the magnitude of RES is strictly normalized between 0 and 1. Higher/Lower RES denotes that the classifier shows higher/lower uncertainty level over the classification output. Instead of using the entropy directly, we introduce RES is to reflect the relative uncertainty level of the classification output, compared to the uniformly random classification output. The value range of the vanilla entropy is unbounded and increases / decreases globally as the number of the families $C$ becomes bigger / smaller. The normalized value of RES is hence used to set up a fair comparison of the uncertainty levels of the classifiers built with different number of malware families. 

Over the singleton malware samples, the average, median and variance of the RES scores are 0.46, 0.49 and 0.18. On the malware samples of unseen families, the average, median and variance of the RES scores are 0.56, 0.62 and 0.19 respectively. 




%There are 18 families, namely \textit{dumpex}, \textit{ruskill}, \textit{bulz}, \textit{refroso}, \textit{stop}, \textit{conduit}, \textit{tweakbit}, \textit{malmaker}, \textit{umbra}, \textit{lassorm}, \textit{utorrent}, \textit{kuaizip}, \textit{installtoolbar}, \textit{hckpk}, \textit{zlob}, \textit{guloader}, \textit{sabsik}, and \textit{spigot} that the multi-class classifier can't correctly categorise at all in the classification test.

 
%In addition in Figure.\, we also illustrate the F1-score results derived by applying \textit{Random Forest} over the time-series-based representation of the dynamic analysis traces. 

%\begin{figure}[h]
%\centering
%	\includegraphics[width=\columnwidth]{fig/f1-score-heatmap_ts.pdf}
%	\caption{F1 score heatmap for family classification using Random Forest on time series of api calls}
%\label{fig:multiclassF12ts}
%\end{figure}


==> sec/overview.tex <==
\section{Overview}\label{sec:overview}

\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/PEPipeline.jpg}
	\caption{Algorithmic Pipeline}
\label{fig:pepipeline}
\end{figure}


==> sec/sandbox.tex <==
\subsection{Sandbox}
\label{sec:sandbox}

We created a Windows 10 Pro 32-bit virtual machine with 2 CPUs (Intel Xeon Platinum 8160 @ 2.10GHz) and 2 GiB of RAM.
We installed some most popular apps from the Microsoft Store (like VLC, 7-Zip, and Telegram), and we populated the file system with documents, pictures, and other common types of files to resemble a legitimate desktop workstation that malware may identify as a more valuable target~\cite{miramirkhani2017spotless}.

Recent findings~\cite{maffia2021longitudinal,galloro2022systematical} about evasive behaviors in Windows malware show that the prevalence of samples that resort to evasive techniques had a slight but steady increase over the years.
Some results of the abovementioned works are diverse because they consider a different number of techniques: Galloro et al.~\cite{galloro2022systematical} report that 80\% of modern malware use at least one evasive technique, while Maffia et al.~\cite{maffia2021longitudinal} the 40\%.
However, both percentages are not negligible, and therefore we have based our analysis on the (only available) open-source code of \emph{JuanLesPIN}~\cite{JLP} by the authors of~\cite{maffia2021longitudinal}, which in turn is based on Intel PIN~\cite{intelpin}, a dynamic binary instrumentation (DBI) framework.
This tool is able to detect and mitigate common evasive techniques, thereby increasing the likelihood that malware detonates.
Unfortunately it does not support executables for 64-bit version of Windows, and for this reason we have decided to focus our study on malware targeting the 32-bit version, preferring a more reliable dynamic analysis that tries to observe all the behavior of the specimen under analysis.
We modified their tool to also monitor the Windows APIs and their arguments responsible for interacting with the following system's components: network, processes, services, registry, mutexes, file system, and dynamic loading of DLLs.
We provide the complete list of the APIs in Appendix~\ref{sec:monitoredAPIs}.

Then, as some participants of the interview by Wong et al.~\cite{yong2021inside} mentioned, we tested our analysis environment with Al-Khaser~\cite{alkhaser}; it is an executable that provides a list of several evasion techniques that the system is susceptible to.
\emph{None} of the techniques implemented in Al-Khaser are able to detect our environment nor our PIN tool.

Our PIN tool introduces an overhead that must be considered; thus, we set up a similar test performed by the same authors of JuanLesPIN~\cite{maffia2021longitudinal}.
We randomly selected 1000 malware samples from our dataset among those who: I) terminate the execution, II) resort to at least one evasive technique, and III) call at least 50 Windows API (the authors of~\cite{kuechler2021} use the same threshold to determine whether a specimen has detonated).
Then, we ran each sample with and without our instrumentation, and we measured the time between the beginning and the end of the execution.
Compared to the non-instrumented version, we obtained a percentage increase of: $\mu=125$, $\sigma=31$, $min=26$, $med=106$, $max=206$.
These results are in line with~\cite{maffia2021longitudinal}, and in the worst case the instrumented sample ran for less than five minutes.

A recent study by Kuechler et al.~\cite{kuechler2021} shows that the amount of code executed by malware samples tends to plateau after only two minutes, and very little additional information can be gained by running samples for more extended periods of time.
Therefore, considering the overhead introduced by our tool and state-of-the-art works that employ a DBI for malware analysis~\cite{polino2017measuring, maffia2021longitudinal,galloro2022systematical}, we decided to run each sample for a maximum of five minutes.

Our infrastructure is composed of 50 clones of the virtual machine described above that we orchestrate using Proxmox VE~\cite{proxmoxve}.
We also took a snapshot of the VM already turned on, and after the user had logged into the system.
We restore the snapshot at the end of the analysis of each sample in order to start the analysis with a clean environment.
It is worth mentioning that we stored all the virtual disk images and the snapshots in a RAM disk, and this trick allowed us to greatly improve performance, especially when restoring a snapshot.

Finally, following the best practices for malware experiments~\cite{rossow2012prudent}, each machine runs on a separate local network with no other machine connected, and we granted full internet access through a dedicated ADSL line of our institution to the samples for communicating with their control servers or downloading external resources.




==> sec/static.tex <==
\section{Static Results} 
\label{sec:static}

\subsection{Binary Classification - Malware Detection} 
\label{sec:binary_static}

\input{tbl/tbl_binary_confusionMatrix}
\input{tbl/tbl_binary_classificationReport}
\input{tbl/tbl_binary_featImportance}
\input{tbl/tbl_binary_bestAndWorst}

\clearpage

\subsection{Mutliclass Classification - Family Classification} 
\label{sec:multiclass_static}
\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/accuracy-heatmap.pdf}
	\caption{Accuracy heatmap for family classification}
\label{fig:multiclassAccuracy}
\end{figure}
\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/f1-score-heatmap.pdf}
	\caption{F1 score heatmap for family classification}
\label{fig:multiclassF1}
\end{figure}

\subsubsection{Worst families accuracy-wise} 
\input{tbl/tbl_multiclass_bestAndWorst}

\subsubsection{Feature importance} 
The values in the table are averaged across all the rounds.
I would discuss general importance and then one vs all classifiers to show that
for some families the importance of the features is not the same.
\input{tbl/tbl_multiclass_featImportance}

One vs rest classifier

\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/oneVsRest_featureImportanceBoxplot.pdf}
	\caption{Importance of each feature class when training one vs rest
	classifiers}
\label{fig:onevsrest_featImportance}
\end{figure}
Discuss interesting cases where ngrams are not the most important
Correlate with VT score

\subsubsection{Singleton} 
Binary classification: here we are using previously trained classifiers to
predict on unseen samples that are not classified by AVClass in any family we
used to train our models. Average accuracy is 94.28 (i.e., it drops slightly
less than 2\% with respect to the classifier trained on the 670 families)
\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/CDF_predictions_singleton.pdf}
	\caption{Error distribution for singleton}
\end{figure}

\subsubsection{Unseen families}
Binary classification: here we are using previously trained classifiers to
predict on samples that belong to families that we did not use in our study
(e.g., those families do not reach 100 samples. Average accuracy drops
significantly to 81.50\% with std 2.27\% (i.e., )

\subsubsection{Family Classification}
\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth]{fig/entropy_distribution.pdf}
	\caption{Entropy distribution comparison}
\end{figure}


==> sec/takeaways.tex <==
\section{Final Recommendations} 

The goal of this work was to understand the key factors that influence the
performance of machine-learning models for malware detection and
classification. 
Based on the results of the individual experiments that we conducted,
we can draw some general recommendations on the use of ML for
malware classification:

\begin{enumerate}
\item \revision{Ideally, experiments on malware classification (both binary and family) should
    be performed on hundreds of different families, each containing a sufficient
    and balanced number of samples. However, this is often difficult to 
    achieve in the malware field. Thus, we believe the contribution of our paper
    is not to simply re-state this obvious finding, but to provide for the first time
    a quantitative assessment of the impact of the lack of these
    characteristics on the classification results. For instance, we show that
    classifiers trained on few
    families (like the ones using the popular Microsoft dataset) can provide
    misleadingly high accuracy scores and experiments conducted on unbalanced datasets
    tend to generalize poorly when tested over different distributions.
    This can also be used to better understand and compare results reported
    in previous studies. For example, our results show that a family
    classifier with a F1 score of 0.89 over 600 families is likely
    better than a classifier with a score of 0.93 on 30 families.}

% \item Experiments on malware classification (both binary and family) should be 
%    performed on hundreds of different families. Classifiers trained on a few
%    families (like the ones on the popular Microsoft dataset) can provide
%    misleadingly high accuracy scores.

% \item Each family in the dataset should contain a sufficient number of samples. 
%    In particular, results from experiment performed on very unbalanced
%    datasets (e.g., where many families only contain a handful of samples)
%    tend to generalize poorly when tested over different distributions.

\item Static features dominate detection and classification of samples from
   \textit{known} families, by relying on signature-like information extracted
   from sequences of bytes and opcodes. Packing, in its current widespread implementation,
   does not seem to have a considerable negative effect on this.
   The addition of dynamic features, which are much more time-consuming and
   error-prone to extract, has only a marginal impact on the classification accuracy
   and therefore its use should be carefully considered if the goal is to detect
   known families.
   However, static features are unable to capture samples from
   \textit{unknown} families, where instead models based on dynamic
   behavior show a better ability to generalize.

\item The performance of \textit{all} ML models drop drastically when tested on OOD samples.
   Therefore, the completeness and the regular update of the training data 
   (which are both difficult to achieve in the real world) are key to
   obtain good results. ML models, especially if integrating dynamic features,
   might still be used to flag suspicious previously-unseen samples, but with 
   much less accuracy and higher false positive rates.
\end{enumerate}



==> sec/xgboost.tex <==
\input{tbl/tbl_xgboost}

\subsection{XGBoost results}\label{sec:xgboost}
\revision{As for \textit{Random Forest} models, we tuned \emph{XGBoost} hyper-parameters
(i.e., learning rate, max tree depth, and the loss type) on a validation set
obtained for each experiment by setting aside 20\% of the samples. Results are
obtained by employing 10-fold cross validation, and by averaging partial
performance scores. Table~\ref{tbl:overallResultsXGboost} summarizes classification results for all
the experiments with this architecture. On average, \emph{XGBoost} classifiers
show 4.4\% and 8.2\% lower F1-score respectively for binary and family
classification. One potential explanation is that
Gradient Boosted trees do not use ensemble voting to deliver the decision.
Their design is similar to AdaBoost or RealBoost~\cite{Friedman2001aos}, which use a cascade
structure to approximate the gradient descent process to a generalized
linear model~\cite{NIPS1999_96a93ba8}. In this way, \textit{XGBoost}
intrinsically achieves low variance in its decision by trading it with
larger bias. If some of the features used by the early layers of Gradient
Boosted trees contain noise or contain misleading information for
classification, this bias will be propagated to the decision stage of the
model, which in turn cause final misclassification.
On the contrary, \textit{Random Forest} models deliver the decision using
the averaged - majority vote of the composing trees. Theoretically, this
approach has a decision output with low bias and low bias, as discussed in
Chapter 9.2.3 of \cite{hastie01statisticallearning}. Intuitively, even if some of the component
trees use ambiguous or noisy features to reach incorrect decision, the voting
output can offer compensation to the misclassification.}



==> tbl/tbl_ALL_binary_100_FP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  TP &  TN &     FP &  FN \\
\midrule
xorist            & NaN & NaN &  100.0 & NaN \\
copidmbe          & NaN & NaN &  100.0 & NaN \\
skintrim          & NaN & NaN &  100.0 & NaN \\
updane            & NaN & NaN &  100.0 & NaN \\
babar             & NaN & NaN &  100.0 & NaN \\
ezsoftwareupdater & NaN & NaN &  100.0 & NaN \\
pistolar          & NaN & NaN &  100.0 & NaN \\
esfury            & NaN & NaN &  100.0 & NaN \\
hotbar            & NaN & NaN &  100.0 & NaN \\
softonic          & NaN & NaN &  100.0 & NaN \\
trickster         & NaN & NaN &  100.0 & NaN \\
pondfull          & NaN & NaN &  100.0 & NaN \\
miniduke          & NaN & NaN &  100.0 & NaN \\
vrbrothers        & NaN & NaN &  100.0 & NaN \\
vindor            & NaN & NaN &  100.0 & NaN \\
pochi             & NaN & NaN &  100.0 & NaN \\
cheatengine       & NaN & NaN &  100.0 & NaN \\
multibar          & NaN & NaN &  100.0 & NaN \\
qbot              & NaN & NaN &  100.0 & NaN \\
kolab             & NaN & NaN &  100.0 & NaN \\
Goodware          & NaN & NaN &  100.0 & NaN \\
\bottomrule
\end{tabular}


==> tbl/tbl_avClassConfidence_correlation.tex <==
\begin{table}[h]
\centering
\caption{The 10 malware families with the lowest family classification accuracy 
using the static analysis-based features correlated with AVClass2 average
	confidence}
\label{tbl:multiclass_static_avClassConfidence}
\begin{tabular}{lrr}
\toprule
	\textbf{Family} & \textbf{Avg Accuracy} &  \textbf{AVClass2 confidence}\\
\midrule
zpevdo              &   15.01 &                 66.43 \\
vitro               &   23.97 &                 72.16 \\
uwamson             &   25.24 &                 68.50 \\
gendal              &   28.04 &                 83.20 \\
dumpex              &   29.04 &                 98.66 \\
alman               &   29.34 &                100.00 \\
sality              &   32.83 &                100.00 \\
pasta               &   34.55 &                 86.18 \\
cobra               &   38.06 &                 87.08 \\
copidmbe            &   38.74 &                 78.70 \\
refroso             &   39.27 &                 72.76 \\
llac                &   40.15 &                 78.49 \\
bifrose             &   40.21 &                 80.50 \\
%atraps              &   40.88 &                 90.99 \\
%pioneer             &   41.86 &                100.00 \\
%coins               &   43.52 &                 84.14 \\
%bancos              &   44.91 &                 92.67 \\
%convagent           &   45.08 &                 94.71 \\
%kiser               &   45.25 &                 88.22 \\
%buzy                &   45.88 &                 75.62 \\
%bestafera           &   48.31 &                 85.93 \\
%ldpinch             &   48.90 &                 87.90 \\
%menti               &   49.02 &                 81.84 \\
%midie               &   49.06 &                 91.45 \\
%alien               &   49.27 &                 85.78 \\
%occamy              &   49.75 &                 79.09 \\
%bulz                &   50.40 &                 92.20 \\
%wsgame              &   50.87 &                 58.54 \\
%sabsik              &   51.43 &                 80.69 \\
%diskwriter          &   51.52 &                 80.01 \\
%tibia               &   52.19 &                 81.33 \\
%oficla              &   52.33 &                 68.49 \\
%klone               &   52.76 &                 71.91 \\
%sdum                &   52.91 &                 72.34 \\
%ramnit              &   53.19 &                 81.20 \\
%presenoker          &   54.00 &                 88.68 \\
%ruskill             &   54.41 &                 60.11 \\
%diztakun            &   54.52 &                 83.32 \\
%bredolab            &   54.54 &                 82.94 \\
%jatif               &   55.82 &                 54.40 \\
%jacard              &   56.16 &                 79.93 \\
%noon                &   57.02 &                 72.66 \\
%scarsi              &   57.90 &                 81.42 \\
%clipbanker          &   57.96 &                 96.27 \\
%poison              &   58.08 &                 76.83 \\
%flystudio           &   58.77 &                 90.93 \\
%ulise               &   59.09 &                 83.86 \\
%pcclient            &   59.16 &                 83.62 \\
%parite              &   59.42 &                100.00 \\
%dorkbot             &   59.51 &                 77.52 \\
%gify                &   59.71 &                 96.00 \\
%kasidet             &   59.84 &                 84.85 \\
%emogen              &   59.85 &                 90.12 \\
%winwebsec           &   59.91 &                 79.44 \\
%zard                &   59.93 &                 44.43 \\
%geral               &   59.93 &                 68.13 \\
%dynamer             &   59.96 &                 88.15 \\
%tdss                &   60.62 &                 88.34 \\
%lethic              &   60.63 &                 74.50 \\
%mucc                &   60.67 &                 73.59 \\
%fareit              &   60.88 &                 74.53 \\
%virut               &   60.91 &                100.00 \\
%gimemo              &   60.94 &                 80.45 \\
%farfli              &   61.13 &                 92.12 \\
%constructor         &   61.44 &                 88.39 \\
%mudrop              &   61.68 &                 76.63 \\
%netwiredrc          &   61.75 &                 87.50 \\
%polypatch           &   61.81 &                 98.35 \\
%vemply              &   61.91 &                 67.30 \\
%cossta              &   62.21 &                 90.09 \\
%carberp             &   62.43 &                 75.79 \\
%usteal              &   62.45 &                 75.07 \\
%bingoml             &   62.96 &                 89.76 \\
%predator            &   63.09 &                 72.58 \\
%cridex              &   63.15 &                 66.76 \\
%ekstak              &   63.30 &                 85.24 \\
%rozena              &   63.35 &                 78.56 \\
%fraudpack           &   63.36 &                 72.54 \\
%buterat             &   63.43 &                 65.90 \\
%siscos              &   63.73 &                 76.80 \\
%crysis              &   63.77 &                 89.69 \\
%palevo              &   63.82 &                 90.84 \\
%ymacco              &   64.33 &                 88.18 \\
%emotet              &   64.51 &                 98.81 \\
%zlob                &   64.69 &                 78.85 \\
%quasar              &   65.01 &                 73.00 \\
%tenga               &   65.42 &                100.00 \\
%macri               &   65.43 &                 73.95 \\
%simda               &   65.44 &                 91.82 \\
%locky               &   65.58 &                 84.05 \\
%kraddare            &   65.95 &                 92.19 \\
%babar               &   66.52 &                 94.00 \\
%induc               &   66.75 &                 86.62 \\
%banbra              &   66.85 &                 99.00 \\
%dorgam              &   67.02 &                 77.84 \\
%gamarue             &   67.08 &                 98.47 \\
%fraudrop            &   67.11 &                 86.44 \\
%zeroaccess          &   67.14 &                 80.20 \\
%lotok               &   67.15 &                 78.14 \\
%blackhole           &   67.29 &                 94.82 \\
%tnega               &   67.63 &                 86.03 \\
%rebhip              &   67.73 &                 70.38 \\
%titirez             &   67.74 &                 45.26 \\
%vbinder             &   67.95 &                 49.60 \\
%spyeye              &   68.07 &                 80.87 \\
%ursnif              &   68.21 &                 83.27 \\
%nanocore            &   68.28 &                 79.38 \\
%mokes               &   68.54 &                 99.29 \\
%buzus               &   68.57 &                 92.14 \\
%hupigon             &   69.40 &                 96.52 \\
%fugrafa             &   69.46 &                 96.96 \\
%sysn                &   69.57 &                 76.20 \\
%slugin              &   70.01 &                100.00 \\
%onlinegames         &   70.42 &                 87.47 \\
%cerbu               &   70.66 &                 95.00 \\
%expiro              &   70.75 &                 96.90 \\
%vittalia            &   70.82 &                 73.00 \\
%yoddos              &   71.09 &                 71.84 \\
%injuke              &   71.19 &                 95.27 \\
%ursu                &   71.43 &                 94.00 \\
%elex                &   71.46 &                 75.84 \\
%rbot                &   71.55 &                 89.23 \\
%deyma               &   71.56 &                 76.36 \\
%emotetu             &   71.60 &                 85.08 \\
%gamini              &   71.62 &                 71.19 \\
%pornoblocker        &   71.70 &                 77.09 \\
%waldek              &   71.73 &                 68.77 \\
%racealer            &   71.79 &                 74.59 \\
%wacatac             &   71.85 &                 97.02 \\
%killmbr             &   72.05 &                 74.82 \\
%xtrat               &   72.66 &                 85.67 \\
%neconyd             &   72.68 &                 69.30 \\
%brresmon            &   72.89 &                 91.10 \\
%qqware              &   72.93 &                 65.90 \\
%stopcrypt           &   73.00 &                100.00 \\
%zegost              &   73.02 &                 71.74 \\
%autinject           &   73.03 &                 99.55 \\
%tonmye              &   73.10 &                 59.46 \\
%startsurf           &   73.18 &                 68.10 \\
%schoolboy           &   73.26 &                 84.72 \\
%tasker              &   73.34 &                 84.39 \\
%bsymem              &   73.62 &                 97.42 \\
%wlksm               &   73.64 &                 51.54 \\
%garrun              &   74.13 &                 74.81 \\
%gamevance           &   74.25 &                 84.40 \\
%sillyfdc            &   74.62 &                 88.99 \\
%zapchast            &   74.64 &                 86.04 \\
%kuluoz              &   74.66 &                 68.20 \\
%agentb              &   74.67 &                 97.63 \\
%ipamor              &   74.78 &                100.00 \\
%blamon              &   74.87 &                 89.77 \\
%orcus               &   74.93 &                 85.41 \\
%dorifel             &   75.16 &                 85.96 \\
%stop                &   75.36 &                 99.17 \\
%wajam               &   75.40 &                 88.00 \\
%fragtor             &   75.58 &                 96.00 \\
%fsysna              &   75.70 &                100.00 \\
%conduit             &   75.87 &                 97.37 \\
%kelihos             &   75.89 &                 78.71 \\
%bandit              &   75.95 &                 89.46 \\
%cutwail             &   76.13 &                 73.91 \\
%bladabindi          &   76.21 &                 98.00 \\
%dadobra             &   76.42 &                 84.60 \\
%speedingupmypc      &   76.55 &                 73.64 \\
%passview            &   76.55 &                 64.94 \\
%zurgop              &   76.75 &                 51.31 \\
%shopper             &   76.79 &                 49.89 \\
%pincav              &   76.87 &                100.00 \\
%glupteba            &   76.99 &                 93.48 \\
%ngrbot              &   77.02 &                 88.22 \\
%stelega             &   77.04 &                 85.01 \\
%spesr               &   77.18 &                 45.62 \\
%jaik                &   77.20 &                 91.00 \\
%voltar              &   77.23 &                 34.83 \\
%swizzor             &   77.32 &                 85.48 \\
%nymeria             &   77.42 &                 98.48 \\
%vebzenpak           &   77.57 &                 70.64 \\
%windigo             &   77.58 &                 52.46 \\
%cryptowall          &   77.64 &                 82.93 \\
%shutdowner          &   77.66 &                 93.34 \\
%tibs                &   77.66 &                 87.03 \\
%dupzom              &   77.67 &                 84.42 \\
%blackmoon           &   78.23 &                 76.46 \\
%teslacrypt          &   78.24 &                 70.89 \\
%amonetize           &   78.30 &                 87.55 \\
%lazy                &   78.33 &                 87.67 \\
%wonton              &   78.51 &                 73.48 \\
%cerber              &   78.57 &                 92.79 \\
%woozlist            &   78.58 &                 50.71 \\
%renos               &   78.65 &                 87.44 \\
%spigot              &   78.93 &                 84.03 \\
%sdbot               &   79.51 &                 98.00 \\
%asparnet            &   79.60 &                 82.69 \\
%vbkryjetor          &   79.80 &                 62.84 \\
%iobit               &   79.90 &                 85.40 \\
%bitmin              &   79.96 &                 98.11 \\
%dofoil              &   80.13 &                 96.00 \\
%lightstone          &   80.18 &                 71.91 \\
%killwin             &   80.28 &                100.00 \\
%fujacks             &   80.30 &                 82.47 \\
%petya               &   80.31 &                 75.77 \\
%ascentive           &   80.32 &                 31.74 \\
%remcos              &   80.41 &                 88.09 \\
%doina               &   80.74 &                 88.88 \\
%mint                &   80.82 &                 95.20 \\
%nymaim              &   80.91 &                 89.41 \\
%chifrax             &   80.91 &                 86.92 \\
%citeary             &   80.92 &                 73.57 \\
%mytob               &   80.99 &                 80.46 \\
%softcnapp           &   81.37 &                100.00 \\
%zbot                &   81.41 &                 72.84 \\
%plugx               &   81.80 &                 63.73 \\
%speedbit            &   81.80 &                 77.09 \\
%binder              &   82.11 &                 88.60 \\
%cryptinject         &   82.24 &                 99.50 \\
%multiplier          &   82.32 &                 86.15 \\
%gatak               &   82.34 &                 87.96 \\
%xyligan             &   82.42 &                 70.00 \\
%azorult             &   82.42 &                100.00 \\
%dorv                &   82.51 &                 71.71 \\
%skillis             &   82.65 &                 93.44 \\
%arkeistealer        &   82.79 &                 85.28 \\
%scrop               &   82.80 &                 93.70 \\
%hacdef              &   82.87 &                 81.12 \\
%brook               &   82.96 &                 75.71 \\
%redcap              &   82.98 &                 83.27 \\
%tofsee              &   82.98 &                 89.78 \\
%qbot                &   83.36 &                 70.03 \\
%darkkomet           &   83.49 &                 89.51 \\
%staser              &   83.49 &                 88.73 \\
%systweak            &   83.81 &                 64.66 \\
%zusy                &   83.86 &                 98.00 \\
%taranis             &   83.91 &                 82.39 \\
%cyfin               &   83.94 &                 99.00 \\
%balrok              &   84.05 &                100.00 \\
%guloader            &   84.05 &                 90.40 \\
%johnnie             &   84.08 &                 98.00 \\
%diss                &   84.14 &                 76.99 \\
%prorat              &   84.41 &                100.00 \\
%tiggre              &   84.42 &                 97.00 \\
%autoitinject        &   84.47 &                 96.22 \\
%mabezat             &   84.47 &                100.00 \\
%schoolgirl          &   84.49 &                 97.87 \\
%avemaria            &   84.50 &                 78.01 \\
%trickster           &   84.61 &                 54.66 \\
%beastdoor           &   84.71 &                 89.70 \\
%hematite            &   84.71 &                 85.02 \\
%reline              &   84.72 &                 84.61 \\
%shade               &   84.84 &                 76.65 \\
%deceptpcclean       &   84.88 &                 59.67 \\
%gandcrypt           &   85.01 &                 54.93 \\
%zenlod              &   85.03 &                 77.04 \\
%spybot              &   85.07 &                 95.81 \\
%xanfpezes           &   85.25 &                 59.98 \\
%yandex              &   85.33 &                 82.54 \\
%gandcrab            &   85.34 &                 83.04 \\
%stampado            &   85.39 &                 74.44 \\
%bactera             &   85.43 &                 83.16 \\
%khalesi             &   85.47 &                 98.73 \\
%omaneat             &   85.47 &                 80.22 \\
%jimmy               &   85.50 &                 73.11 \\
%raccrypt            &   85.69 &                 87.98 \\
%dalexis             &   85.76 &                 77.60 \\
%xorist              &   85.81 &                 69.73 \\
%webprefix           &   85.82 &                 68.33 \\
%installcore         &   85.86 &                 80.20 \\
%driverpack          &   85.96 &                 96.18 \\
%trickbot            &   86.06 &                 83.05 \\
%sodinokibi          &   86.27 &                       NaN \\
%manbat              &   86.40 &                 82.67 \\
%utorrent            &   86.56 &                 92.15 \\
%offend              &   86.62 &                 93.40 \\
%burden              &   86.78 &                 85.65 \\
%skintrim            &   87.08 &                 70.40 \\
%lokibot             &   87.09 &                 97.29 \\
%esfury              &   87.12 &                 49.77 \\
%neutrinopos         &   87.17 &                 66.02 \\
%recex               &   87.28 &                 26.03 \\
%onescan             &   87.33 &                 82.41 \\
%hotbar              &   87.66 &                 87.51 \\
%smartpcsolutions    &   87.78 &                 88.69 \\
%solmyr              &   87.84 &                 89.65 \\
%shylock             &   87.87 &                 77.74 \\
%subseven            &   87.95 &                 89.13 \\
%bunitu              &   88.09 &                 89.83 \\
%lovgate             &   88.26 &                 87.22 \\
%ficker              &   88.38 &                 63.57 \\
%turkojan            &   88.40 &                 85.72 \\
%yahlover            &   88.43 &                 69.46 \\
%mulinex             &   88.47 &                 73.92 \\
%crossrider          &   88.54 &                 92.61 \\
%stihat              &   88.63 &                 34.36 \\
%sogou               &   88.64 &                 73.04 \\
%bezigate            &   88.83 &                 66.63 \\
%opensupdater        &   88.90 &                 74.32 \\
%strab               &   88.94 &                 75.99 \\
%istartsurf          &   88.96 &                 58.68 \\
%xorer               &   89.02 &                 58.80 \\
%dlhelper            &   89.17 &                 80.32 \\
%nitol               &   89.19 &                 99.50 \\
%pterodo             &   89.30 &                 66.03 \\
%mepaow              &   89.53 &                 30.60 \\
%xiaobaminer         &   89.56 &                 99.00 \\
%winwrapper          &   89.63 &                 58.46 \\
%necurs              &   89.65 &                 83.81 \\
%privateexeprotector &   89.70 &                 91.84 \\
%techsnab            &   89.84 &                 84.64 \\
%mbrlock             &   90.06 &                100.00 \\
%hpdefender          &   90.07 &                 93.84 \\
%vawtrak             &   90.16 &                 57.52 \\
%lockbit             &   90.17 &                 93.00 \\
%miancha             &   90.30 &                 73.74 \\
%convertad           &   90.40 &                100.00 \\
%mywebsearch         &   90.45 &                 92.49 \\
%ardamax             &   90.55 &                 97.85 \\
%bobax               &   90.62 &                 89.87 \\
%agobot              &   90.84 &                 91.37 \\
%filefinder          &   90.93 &                 73.53 \\
%gamania             &   90.98 &                100.00 \\
%lamer               &   90.99 &                 93.78 \\
%woool               &   91.02 &                 61.21 \\
%bebloh              &   91.07 &                100.00 \\
%pirminay            &   91.10 &                 81.59 \\
%bandoo              &   91.13 &                 91.54 \\
%relevantknowledge   &   91.16 &                 93.11 \\
%cobaltstrike        &   91.20 &                 76.61 \\
%klez                &   91.25 &                100.00 \\
%kolovorot           &   91.25 &                 91.38 \\
%schwarzesonne       &   91.41 &                 59.91 \\
%kovter              &   91.45 &                 96.51 \\
%sohanad             &   91.52 &                100.00 \\
%shandaadd           &   91.59 &                 68.52 \\
%ranumbot            &   91.71 &                 77.78 \\
%dealply             &   91.74 &                 99.50 \\
%loadmoney           &   91.76 &                 98.87 \\
%linkury             &   91.87 &                 84.58 \\
%netstream           &   91.98 &                 48.93 \\
%hider               &   92.05 &                 96.58 \\
%koobface            &   92.10 &                 73.02 \\
%lollipop            &   92.28 &                 62.97 \\
%vilsel              &   92.32 &                100.00 \\
%pidgeon             &   92.37 &                100.00 \\
%blackie             &   92.40 &                 96.61 \\
%icedid              &   92.40 &                 99.52 \\
%malex               &   92.42 &                100.00 \\
%msposer             &   92.48 &                 69.50 \\
%scrarev             &   92.52 &                 56.26 \\
%fakefolder          &   92.64 &                100.00 \\
%toptools            &   92.77 &                 91.95 \\
%gozi                &   92.83 &                 82.60 \\
%cycbot              &   92.85 &                 91.78 \\
%benjamin            &   93.06 &                100.00 \\
%browsefox           &   93.09 &                 96.72 \\
%eyestye             &   93.27 &                 85.08 \\
%urelas              &   93.28 &                100.00 \\
%fosniw              &   93.41 &                 89.69 \\
%auslogics           &   93.42 &                 60.96 \\
%agentc              &   93.42 &                 84.43 \\
%virbox              &   93.62 &                 79.56 \\
%upatre              &   93.72 &                100.00 \\
%fakefire            &   93.84 &                100.00 \\
%opencandy           &   93.84 &                 98.51 \\
%adpack              &   93.86 &                 75.80 \\
%pcacceleratepro     &   93.86 &                 82.37 \\
%aitinject           &   93.92 &                100.00 \\
%dodiw               &   94.00 &                 70.05 \\
%remoteutilities     &   94.10 &                 94.60 \\
%horst               &   94.16 &                 80.01 \\
%adgazelle           &   94.19 &                 98.16 \\
%silentall           &   94.21 &                 67.82 \\
%seraph              &   94.22 &                 59.67 \\
%refinka             &   94.24 &                 41.50 \\
%softpulse           &   94.29 &                 99.43 \\
%neoreklami          &   94.32 &                 97.34 \\
%formbook            &   94.32 &                 87.97 \\
%imali               &   94.36 &                 88.59 \\
%winactivator        &   94.38 &                 96.38 \\
%qzonit              &   94.40 &                 80.16 \\
%explorerhijack      &   94.41 &                 55.63 \\
%multibar            &   94.70 &                 91.54 \\
%perion              &   94.71 &                 80.09 \\
%qshell              &   94.85 &                 76.06 \\
%tremp               &   94.91 &                 57.62 \\
%installerex         &   94.98 &                100.00 \\
%offergenerator      &   95.09 &                 56.84 \\
%firseria            &   95.10 &                100.00 \\
%screenmate          &   95.13 &                 92.07 \\
%tufik               &   95.13 &                 95.92 \\
%chir                &   95.13 &                 99.44 \\
%speedcat            &   95.26 &                 48.56 \\
%shiz                &   95.31 &                 90.22 \\
%frosparf            &   95.36 &                 77.91 \\
%qihoo               &   95.38 &                 97.26 \\
%megasearch          &   95.48 &                 69.93 \\
%duote               &   95.49 &                 96.17 \\
%ibryte              &   95.53 &                100.00 \\
%domaiq              &   95.55 &                 85.45 \\
%zygug               &   95.55 &                 99.00 \\
%swisyn              &   95.56 &                100.00 \\
%daws                &   95.57 &                 99.00 \\
%installbrain        &   95.61 &                100.00 \\
%vundo               &   95.66 &                 52.76 \\
%xcnfe               &   95.73 &                 99.50 \\
%tinba               &   95.75 &                100.00 \\
%downloadsponsor     &   95.76 &                 87.39 \\
%autog               &   95.88 &                100.00 \\
%icloader            &   95.94 &                 86.34 \\
%veil                &   95.96 &                 69.34 \\
%lecna               &   95.96 &                 89.83 \\
%downloadassistant   &   95.98 &                 97.10 \\
%mewsspy             &   95.98 &                 88.83 \\
%regsup              &   96.02 &                 67.41 \\
%kuaizip             &   96.04 &                100.00 \\
%bublik              &   96.06 &                 64.58 \\
%simbot              &   96.08 &                 70.49 \\
%vobfus              &   96.09 &                 99.89 \\
%lunastorm           &   96.16 &                 61.14 \\
%sohana              &   96.18 &                100.00 \\
%downloadadmin       &   96.18 &                 91.99 \\
%filetour            &   96.23 &                 89.22 \\
%reptile             &   96.25 &                 49.15 \\
%kolweb              &   96.30 &                 92.68 \\
%pacex               &   96.35 &                 90.29 \\
%xolxo               &   96.41 &                 98.00 \\
%axespec             &   96.43 &                 70.48 \\
%betload             &   96.45 &                 96.00 \\
%kolab               &   96.46 &                 99.00 \\
%lydra               &   96.51 &                100.00 \\
%idsohtu             &   96.51 &                 60.15 \\
%wapomi              &   96.55 &                 91.56 \\
%miniduke            &   96.56 &                 81.35 \\
%wannacry            &   96.57 &                100.00 \\
%wakme               &   96.57 &                 74.29 \\
%plurox              &   96.65 &                 97.87 \\
%phorpiex            &   96.66 &                 89.64 \\
%koutodoor           &   96.66 &                 84.75 \\
%webcompanion        &   96.66 &                 79.87 \\
%installmonster      &   96.68 &                100.00 \\
%protux              &   96.72 &                 90.94 \\
%blackshades         &   96.73 &                 97.88 \\
%detrahere           &   96.82 &                 51.91 \\
%rostpay             &   96.87 &                 92.75 \\
%moarider            &   96.93 &                100.00 \\
%gofot               &   96.96 &                 75.60 \\
%growtopia           &   96.99 &                 63.64 \\
%fesber              &   97.04 &                 98.00 \\
%sytro               &   97.11 &                100.00 \\
%bayrob              &   97.12 &                 84.19 \\
%spyrix              &   97.13 &                 88.01 \\
%cosmu               &   97.18 &                100.00 \\
%shipup              &   97.25 &                 72.50 \\
%lmir                &   97.27 &                 77.75 \\
%4shared             &   97.28 &                 98.44 \\
%snojan              &   97.29 &                100.00 \\
%broskod             &   97.35 &                 75.36 \\
%socelars            &   97.37 &                 79.49 \\
%egroupdial          &   97.37 &                100.00 \\
%dinwod              &   97.38 &                 87.94 \\
%havex               &   97.39 &                100.00 \\
%dstudio             &   97.41 &                 96.57 \\
%memery              &   97.43 &                 67.37 \\
%vrbrothers          &   97.46 &                100.00 \\
%alyak               &   97.46 &                 83.29 \\
%mooqkel             &   97.48 &                 86.70 \\
%mocrt               &   97.53 &                 45.79 \\
%bundlore            &   97.55 &                 95.03 \\
%anmalpro            &   97.57 &                 80.26 \\
%getnow              &   97.57 &                 83.82 \\
%qqhack              &   97.58 &                100.00 \\
%webdialer           &   97.61 &                 58.55 \\
%maener              &   97.61 &                 94.76 \\
%wecod               &   97.62 &                 46.95 \\
%expressdownloader   &   97.62 &                 80.30 \\
%unruy               &   97.62 &                100.00 \\
%dexel               &   97.67 &                 91.23 \\
%reconyc             &   97.68 &                100.00 \\
%installiq           &   97.69 &                 89.97 \\
%bcryptinject        &   97.73 &                 99.60 \\
%ceatrg              &   97.75 &                 86.86 \\
%tougle              &   97.75 &                 65.14 \\
%pajetbin            &   97.76 &                 70.93 \\
%neshta              &   97.81 &                100.00 \\
%webalta             &   97.86 &                 54.95 \\
%lipler              &   97.87 &                 56.22 \\
%mira                &   97.94 &                 95.10 \\
%aauto               &   97.94 &                 92.26 \\
%plingky             &   97.95 &                 88.88 \\
%cardspy             &   97.96 &                 58.64 \\
%banload             &   98.00 &                100.00 \\
%macoute             &   98.00 &                 63.25 \\
%cjishu              &   98.01 &                 87.85 \\
%kuaiba              &   98.04 &                100.00 \\
%slimware            &   98.06 &                 66.28 \\
%inbox               &   98.06 &                 60.97 \\
%airinstaller        &   98.10 &                100.00 \\
%bloored             &   98.11 &                100.00 \\
%kingsoft            &   98.12 &                 96.20 \\
%youxun              &   98.19 &                100.00 \\
%mediaget            &   98.20 &                 99.00 \\
%qjwmonkey           &   98.21 &                 99.72 \\
%disttrack           &   98.27 &                 62.50 \\
%softonic            &   98.32 &                100.00 \\
%fasong              &   98.34 &                100.00 \\
%safebytes           &   98.36 &                 50.31 \\
%babonock            &   98.37 &                 94.74 \\
%goldrv              &   98.41 &                100.00 \\
%detroie             &   98.43 &                100.00 \\
%gobot               &   98.46 &                 98.38 \\
%cosmicduke          &   98.49 &                 76.58 \\
%openinstall         &   98.49 &                100.00 \\
%paneidix            &   98.52 &                 86.92 \\
%rising              &   98.52 &                 90.44 \\
%gepys               &   98.57 &                 96.95 \\
%ksdler              &   98.59 &                 79.78 \\
%hebchengjiu         &   98.60 &                 57.91 \\
%lolbot              &   98.62 &                 84.30 \\
%cheatengine         &   98.63 &                100.00 \\
%zvuzona             &   98.64 &                 98.30 \\
%outbyte             &   98.66 &                 99.00 \\
%laqma               &   98.67 &                 79.00 \\
%winloadsda          &   98.67 &                 83.76 \\
%powerless           &   98.69 &                 68.26 \\
%sillyp2p            &   98.72 &                 64.14 \\
%agentino            &   98.73 &                 99.00 \\
%tupym               &   98.73 &                 94.37 \\
%agentcrypt          &   98.74 &                 99.60 \\
%seven               &   98.74 &                 79.89 \\
%kronosbot           &   98.74 &                 64.56 \\
%dumpy               &   98.76 &                 73.87 \\
%cmy3u               &   98.77 &                 91.64 \\
%elemental           &   98.77 &                 74.42 \\
%aenjaris            &   98.78 &                 80.27 \\
%dluca               &   98.79 &                 84.03 \\
%oberal              &   98.81 &                 50.57 \\
%antavmu             &   98.82 &                100.00 \\
%konus               &   98.86 &                 76.50 \\
%apost               &   98.86 &                 79.83 \\
%virlock             &   98.88 &                100.00 \\
%addlyrics           &   98.91 &                 76.03 \\
%viking              &   98.92 &                100.00 \\
%gippers             &   98.96 &                 82.67 \\
%pluto               &   98.97 &                 96.89 \\
%virfire             &   99.03 &                 52.45 \\
%stone               &   99.04 &                100.00 \\
%connectwise         &   99.05 &                 94.10 \\
%downer              &   99.08 &                100.00 \\
%mailru              &   99.09 &                 80.26 \\
%lassorm             &   99.11 &                 55.49 \\
%bzub                &   99.12 &                 75.23 \\
%pedex               &   99.14 &                 98.82 \\
%lulusoftware        &   99.17 &                 94.30 \\
%pondfull            &   99.17 &                 82.09 \\
%pistolar            &   99.18 &                100.00 \\
%gorillaprice        &   99.21 &                 79.48 \\
%taskloader          &   99.25 &                 72.88 \\
%brontok             &   99.25 &                100.00 \\
%winner              &   99.33 &                 85.28 \\
%vkontaktedj         &   99.37 &                 71.51 \\
%hafen               &   99.39 &                 50.64 \\
%gigex               &   99.40 &                100.00 \\
%clipspy             &   99.43 &                 92.00 \\
%eyoorun             &   99.45 &                 70.94 \\
%lunam               &   99.51 &                100.00 \\
%tisandr             &   99.52 &                 84.76 \\
%fakens              &   99.52 &                 69.42 \\
%roxer               &   99.54 &                 72.34 \\
%gamemodding         &   99.59 &                 78.64 \\
%goabeny             &   99.61 &                 62.94 \\
%jevafus             &   99.61 &                 81.94 \\
%offercore           &   99.62 &                 97.21 \\
%pahooka             &   99.63 &                100.00 \\
%salgorea            &   99.64 &                100.00 \\
%zepfod              &   99.66 &                100.00 \\
%qqpass              &   99.73 &                100.00 \\
%lolojan             &   99.81 &                 98.76 \\
%pochi               &   99.82 &                 97.33 \\
%mydoom              &   99.82 &                100.00 \\
%allaple             &   99.87 &                100.00 \\
%socks               &   99.87 &                100.00 \\
%xihet               &   99.89 &                 79.70 \\
%tempedreve          &   99.90 &                 45.40 \\
%griptolo            &   99.92 &                100.00 \\
%shyape              &   99.93 &                 76.03 \\
%sivis               &   99.93 &                 86.41 \\
%wabot               &   99.94 &                100.00 \\
%moonlight           &   99.94 &                 90.06 \\
%prepscram           &   99.95 &                 97.97 \\
%grenam              &   99.96 &                 74.48 \\
%phishbank           &   99.96 &                 57.00 \\
%coroxy              &   99.96 &                 58.45 \\
%jeefo               &   99.98 &                100.00 \\
%zylom               &   99.98 &                 96.00 \\
%hebogo              &   99.98 &                 87.48 \\
%loring              &   99.98 &                 61.15 \\
%rums                &   99.99 &                 96.60 \\
%pykspa              &   99.99 &                 85.66 \\
%fakedoc             &   99.99 &                 53.01 \\
%houndhack           &   99.99 &                 36.69 \\
%diamin              &   99.99 &                 88.63 \\
%syncopate           &   99.99 &                 98.60 \\
%drstwex             &   99.99 &                 96.37 \\
%enosch              &   99.99 &                 50.31 \\
%gator               &  100.00 &                 86.56 \\
%gametea             &  100.00 &                 26.46 \\
%eggnog              &  100.00 &                 90.22 \\
%finfish             &  100.00 &                 64.96 \\
%updane              &  100.00 &                 71.55 \\
%esaprof             &  100.00 &                 95.52 \\
%upantix             &  100.00 &                 99.37 \\
%facido              &  100.00 &                100.00 \\
%umbra               &  100.00 &                 99.50 \\
%esecn               &  100.00 &                 70.81 \\
%ezsoftwareupdater   &  100.00 &                 99.00 \\
%downloadguide       &  100.00 &                 96.95 \\
%geegly              &  100.00 &                 83.60 \\
%gogo                &  100.00 &                100.00 \\
%dostre              &  100.00 &                100.00 \\
%lyposit             &  100.00 &                 97.30 \\
%chrop               &  100.00 &                 93.53 \\
%swjoy               &  100.00 &                100.00 \\
%digs                &  100.00 &                 39.69 \\
%stormattack         &  100.00 &                 83.32 \\
%inlog               &  100.00 &                 98.02 \\
%vtflooder           &  100.00 &                100.00 \\
%itorrent            &  100.00 &                 60.34 \\
%ludbaruma           &  100.00 &                 76.00 \\
%vybab               &  100.00 &                 95.13 \\
%vbclone             &  100.00 &                100.00 \\
%keydoor             &  100.00 &                100.00 \\
%krol                &  100.00 &                 49.66 \\
%wavipeg             &  100.00 &                100.00 \\
%trymedia            &  100.00 &                 98.10 \\
%lebreat             &  100.00 &                 99.60 \\
%jpgiframe           &  100.00 &                100.00 \\
%dropware            &  100.00 &                 74.08 \\
%sinau               &  100.00 &                 95.00 \\
%dpsk                &  100.00 &                 99.00 \\
%neojit              &  100.00 &                 83.62 \\
%blihan              &  100.00 &                100.00 \\
%sfone               &  100.00 &                100.00 \\
%cambot              &  100.00 &                 46.41 \\
%qaccel              &  100.00 &                100.00 \\
%shodi               &  100.00 &                100.00 \\
%mimdau              &  100.00 &                100.00 \\
%burn                &  100.00 &                 50.53 \\
%mimail              &  100.00 &                 81.47 \\
%mapsgory            &  100.00 &                 90.15 \\
%catalina            &  100.00 &                100.00 \\
%adaebook            &  100.00 &                 99.00 \\
%nevereg             &  100.00 &                100.00 \\
%recodrop            &  100.00 &                 72.27 \\
%adposhel            &  100.00 &                 80.98 \\
%primecasino         &  100.00 &                 97.00 \\
%powerspider         &  100.00 &                 64.40 \\
%wenper              &  100.00 &                 98.26 \\
%triusor             &  100.00 &                 75.02 \\
%obit                &  100.00 &                 99.60 \\
%rikihaki            &  100.00 &                 90.13 \\
%contenedor          &  100.00 &                100.00 \\
%rungbu              &  100.00 &                100.00 \\
%drolnux             &  100.00 &                100.00 \\
%atcpa               &  100.00 &                 99.80 \\
%amigo               &  100.00 &                100.00 \\
%picsys              &  100.00 &                100.00 \\
%rifdoor             &  100.00 &                 74.63 \\
%berbew              &  100.00 &                 99.37 \\
%plemood             &  100.00 &                100.00 \\
%regrun              &  100.00 &                100.00 \\
%ruledor             &  100.00 &                 63.12 \\
%soulclose           &  100.00 &                100.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_avClassConfidence_correlation_dyn.tex <==
\begin{table}[h]
\centering
\caption{Top-10 malware families with the lowest binary classification accuracy 
using the dynamic analysis-based features
(i.e., highest mispredictions as goodware) correlated with AVClass2 average
	confidence}
\label{tbl:multiclass_static_avClassConfidence}
\begin{tabular}{lrr}
\toprule
	\textbf{Family} & \textbf{Avg Accuracy} &  \textbf{AVClass2 confidence}\\
\midrule
tasker              &   0.0 &                 84.39 \\
malex               &   0.0 &                 92.42 \\
rostpay             &   0.0 &                 92.75 \\
constructor              &   0.0 &                 88.39 \\
atcpa              &   0.0 &                 99.80 \\
mocrt               &   0.0 &                45.79 \\
mokes              &   0.0 &                99.29 \\
bingoml               &   0.0 &                 89.76 \\
safebytes               &   0.0 &                50.31 \\
trymedia            &   0.0 &                 98.10 \\
\bottomrule
\end{tabular}
\end{table}

==> tbl/tbl_avc2_beh.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{llrr}
\hline
\textbf{Beh} & \textbf{Samples} & \textbf{Samples Perc} \\
\hline
 Unknown                & 53764  & 27.5 \\
 execdownload           & 49065  & 25.1 \\
 server                 & 17184  & 8.8 \\
 filemodify             & 15540  & 7.9 \\
 selfpropagate          & 13861  & 7.1 \\
 inject                 & 9123   & 4.7 \\
 filecrypt              & 7813   & 4.0 \\
 infosteal              & 6344   & 3.2 \\
 jswebinject            & 2621   & 1.3 \\
 mining                 & 2293   & 1.2 \\
 alertuser              & 2250   & 1.1 \\
 browsermodify:toolbar  & 1927   & 1.0 \\
 clicks                 & 1783   & 0.9 \\
 keylogging             & 1376   & 0.7 \\
 infosteal:gamethief    & 1365   & 0.7 \\
 browsermodify          & 1143   & 0.6 \\
 dials                  & 1124   & 0.6 \\
 osmodify               & 1022   & 0.5 \\
 killproc:killsectool   & 922    & 0.5 \\
 proxy                  & 756    & 0.4 \\
 autorun                & 583    & 0.3 \\
 ddos                   & 528    & 0.3 \\
 mining:bitcoinmining   & 494    & 0.3 \\
 network                & 437    & 0.2 \\
 files                  & 404    & 0.2 \\
 sms:sendssms           & 327    & 0.2 \\
 servstart              & 316    & 0.2 \\
 hostsmodify            & 228    & 0.1 \\
 spam                   & 211    & 0.1 \\
 killproc               & 182    & 0.1 \\
 search                 & 174    & 0.1 \\
 irc                    & 168    & 0.1 \\
 phishing               & 116    & 0.1 \\
 dnsmodify              & 115    & 0.1 \\
 lockscreen             & 113    & 0.1 \\
 proxychanger           & 94     & 0.0 \\
 defaulttab             & 28     & 0.0 \\
 filedelete             & 8      & 0.0 \\
 vmdetect               & 5      & 0.0 \\

\hline
\end{tabular}
\caption{AVClass2 malware behaviours.}
\label{tbl:avc2_beh}
\end{table}

% cat avc2_beh.csv |  tail -n+2 | awk -F $'\t' '{print $1 " & " $2 " & " $3 " \\\\"}' | sed 's/_/\\_/g' |  sed 's/,/ /g' | ocdTex


==> tbl/tbl_avc2_class.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{llrr}
\hline
\textbf{Class} & \textbf{Samples} & \textbf{Samples Perc} \\
\hline
 grayware           & 83018  & 42.4 \\
 downloader         & 35471  & 18.1 \\
 Unknown            & 19778  & 10.1 \\
 worm               & 14808  & 7.6 \\
 backdoor           & 13268  & 6.8 \\
 ransomware         & 8244   & 4.2 \\
 virus              & 7381   & 3.8 \\
 spyware            & 4515   & 2.3 \\
 miner              & 2520   & 1.3 \\
 rogueware          & 2134   & 1.1 \\
 dialer             & 1102   & 0.6 \\
 clicker            & 1054   & 0.5 \\
 rootkit            & 886    & 0.5 \\
 keylogger          & 710    & 0.4 \\
 hoax               & 272    & 0.1 \\
 grayware:tool      & 217    & 0.1 \\
 hoax:smshoax       & 176    & 0.1 \\
 bot                & 176    & 0.1 \\
 infector           & 72     & 0.0 \\
 fakeantivirus      & 3      & 0.0 \\
 rooter             & 1      & 0.0 \\
 dialer:porndialer  & 1      & 0.0 \\

\hline
\end{tabular}
\caption{AVClass2 malware classes.}
\label{tbl:avc2_class}
\end{table}

% cat avc2_class.csv |  tail -n+2 | awk -F $'\t' '{print $1 " & " $2 " & " $3 " \\\\"}' | sed 's/_/\\_/g' |  sed 's/,/ /g' | ocdTex


==> tbl/tbl_avc2_fams.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{llrr}
\hline
\textbf{Family} & \textbf{Samples} & \textbf{Samples Perc} \\
\hline
 Unknown                        & 11246  & 5.7 \\
 zusy                           & 5366   & 2.7 \\
 flystudio                      & 1509   & 0.8 \\
 onlinegames                    & 1483   & 0.8 \\
 vobfus                         & 1241   & 0.6 \\
 loadmoney                      & 1172   & 0.6 \\
 fareit                         & 1097   & 0.6 \\
 zbot                           & 1050   & 0.5 \\
 farfli                         & 703    & 0.4 \\
 banload                        & 682    & 0.3 \\
 hupigon                        & 627    & 0.3 \\
 packer                         & 615    & 0.3 \\
 hotbar                         & 584    & 0.3 \\
 gamarue                        & 580    & 0.3 \\
 dynamer                        & 539    & 0.3 \\
 spigot                         & 501    & 0.3 \\
 ramnit                         & 485    & 0.2 \\
 gamania                        & 483    & 0.2 \\
 virut                          & 480    & 0.2 \\
 fakefolder                     & 460    & 0.2 \\
%  bancos                         & 460    & 0.2 \\
%  sality                         & 447    & 0.2 \\
%  brontok                        & 445    & 0.2 \\
%  nymaim                         & 441    & 0.2 \\
%  rbot                           & 437    & 0.2 \\
%  cosmu                          & 418    & 0.2 \\
%  bifrose                        & 411    & 0.2 \\
%  sfone                          & 409    & 0.2 \\
%  berbew                         & 404    & 0.2 \\
%  vundo                          & 399    & 0.2 \\
%  metasploit                     & 391    & 0.2 \\
%  icloader                       & 386    & 0.2 \\
%  softcnapp                      & 383    & 0.2 \\
%  poison                         & 379    & 0.2 \\
%  bladabindi                     & 376    & 0.2 \\
%  dridex                         & 366    & 0.2 \\
%  daws                           & 365    & 0.2 \\
%  sdbot                          & 361    & 0.2 \\
%  dlhelper                       & 345    & 0.2 \\
%  cryxos                         & 337    & 0.2 \\
%  installmonster                 & 335    & 0.2 \\
%  swisyn                         & 332    & 0.2 \\
%  zegost                         & 330    & 0.2 \\
%  tdss                           & 327    & 0.2 \\
%  nitol                          & 321    & 0.2 \\
%  presenoker                     & 319    & 0.2 \\
%  installerex                    & 315    & 0.2 \\
%  dofoil                         & 310    & 0.2 \\
%  kelihos                        & 309    & 0.2 \\
%  spyeye                         & 300    & 0.2 \\
%  installcore                    & 298    & 0.2 \\

\hline
\end{tabular}
\caption{Top 20 AVClass2 families.}
\label{tbl:avc2_fams}
\end{table}

% cat avc2_fams.csv |  tail -n+2 | awk -F $'\t' '{print $1 " & " $2 " & " $3 " \\\\"}' | sed 's/_/\\_/g' |  sed 's/,/ /g' | ocdTex


==> tbl/tbl_binary_bestAndWorst_combined.tex <==
\begin{table}[h]
\centering
\small
\caption{Top-10 malware families with the lowest detection accuracy using
	combined features
	(i.e., highest mispredictions as goodware).}
\label{tbl:binary_combined_bestAndWorst}
\begin{tabular}{llcr}
\toprule
\multicolumn{4}{c}{\textbf{Combined binary classification}}\\
	\textbf{Family} & \textbf{Class} &  \textbf{Avg F1} &  \textbf{\% packed} \\
\midrule
sality              &       virus &         0.755 &       4\% \\
slugin              &       virus &         0.770 &       4\% \\
asparnet            &    grayware &         0.775 &       5\% \\
pioneer             &       virus &         0.790 &       6\% \\
expiro              &       virus &         0.825 &      10\% \\
iobit               &    grayware &         0.874 &      38\% \\
speedingupmypc      &    grayware &         0.875 &      11\% \\
conduit             &    grayware &         0.875 &      35\% \\
softcnapp           &      adware &         0.880 &       0\% \\
installcore         &    grayware &         0.895 &      10\% \\
%systweak            &    grayware &         0.900 &      19 \\
%copidmbe            &       virus &         0.900 &       9 \\
%passview            &    grayware &         0.901 &      35 \\
%wajam               &      adware &         0.915 &       2 \\
%ekstak              &    grayware &         0.935 &      31 \\
%zpevdo              &    grayware &         0.935 &      15 \\
%getnow              &    grayware &         0.935 &      88 \\
%driverpack          &    grayware &         0.935 &      13 \\
%mywebsearch         &    grayware &         0.935 &       1 \\
%kuaiba              &      adware &         0.935 &       5 \\
%rozena              &    backdoor &         0.940 &       3 \\
%elex                &      adware &         0.940 &       9 \\
%shopper             &    grayware &         0.940 &       1 \\
%bulz                &    grayware &         0.940 &      15 \\
%citeary             &        worm &         0.947 &      16 \\
%sogou               &    grayware &         0.950 &      17 \\
%virut               &       virus &         0.950 &       3 \\
%burden              &      adware &         0.950 &       2 \\
%geral               &  downloader &         0.950 &      23 \\
%tisandr             &        worm &         0.950 &       0 \\
%gamevance           &      adware &         0.955 &       5 \\
%yandex              &    grayware &         0.955 &       0 \\
%toptools            &    grayware &         0.955 &       0 \\
%ursu                &    grayware &         0.955 &      23 \\
%sodinokibi          &    grayware &         0.955 &       2 \\
%uwamson             &    grayware &         0.955 &      15 \\
%relevantknowledge   &      adware &         0.955 &       0 \\
%cobra               &    grayware &         0.955 &      60 \\
%bandoo              &    grayware &         0.955 &       0 \\
%diztakun            &    grayware &         0.960 &      27 \\
%skillis             &    grayware &         0.960 &      19 \\
%smartpcsolutions    &    grayware &         0.960 &      46 \\
%downloadassistant   &    grayware &         0.960 &      18 \\
%techsnab            &    grayware &         0.960 &       2 \\
%alien               &  downloader &         0.960 &      20 \\
%presenoker          &    grayware &         0.960 &      16 \\
%schoolboy           &    grayware &         0.960 &       7 \\
%parite              &       virus &         0.960 &       7 \\
%diskwriter          &    grayware &         0.963 &      29 \\
%staser              &  downloader &         0.965 &      61 \\
%cjishu              &      adware &         0.965 &       1 \\
%chir                &        worm &         0.965 &      12 \\
%jatif               &    grayware &         0.965 &       2 \\
%sabsik              &    grayware &         0.965 &      30 \\
%adgazelle           &    grayware &         0.965 &       0 \\
%emotet              &  downloader &         0.965 &       1 \\
%vrbrothers          &      adware &         0.970 &      88 \\
%gamini              &    grayware &         0.970 &       0 \\
%bestafera           &    grayware &         0.970 &      57 \\
%opensupdater        &      adware &         0.970 &      14 \\
%vitro               &       virus &         0.970 &       3 \\
%cridex              &    grayware &         0.970 &      15 \\
%polypatch           &    grayware &         0.970 &      99 \\
%rbot                &        worm &         0.970 &      19 \\
%fugrafa             &    grayware &         0.970 &       8 \\
%kraddare            &      adware &         0.970 &      36 \\
%wakme               &  downloader &         0.975 &       0 \\
%zard                &    grayware &         0.975 &       3 \\
%downloadadmin       &    grayware &         0.975 &       3 \\
%lotok               &    backdoor &         0.975 &      15 \\
%midie               &    grayware &         0.975 &      33 \\
%utorrent            &    grayware &         0.975 &      72 \\
%taranis             &    grayware &         0.975 &       4 \\
%petya               &  ransomware &         0.975 &      16 \\
%mediaget            &    grayware &         0.975 &      33 \\
%constructor         &    grayware &         0.975 &      13 \\
%expressdownloader   &    grayware &         0.975 &      62 \\
%remoteutilities     &    grayware &         0.975 &      90 \\
%sdum                &    grayware &         0.975 &      24 \\
%clipbanker          &    grayware &         0.975 &      11 \\
%scrop               &  downloader &         0.975 &      12 \\
%menti               &        worm &         0.975 &      11 \\
%lamer               &       virus &         0.978 &      43 \\
%installbrain        &    grayware &         0.980 &       2 \\
%filetour            &    grayware &         0.980 &       4 \\
%anmalpro            &    grayware &         0.980 &       0 \\
%vkontaktedj         &    grayware &         0.980 &       4 \\
%buzus               &  downloader &         0.980 &       3 \\
%buzy                &        worm &         0.980 &      35 \\
%pcacceleratepro     &    grayware &         0.980 &       1 \\
%binder              &  downloader &         0.980 &      16 \\
%farfli              &    backdoor &         0.980 &      38 \\
%speedbit            &    grayware &         0.980 &       8 \\
%inlog               &  downloader &         0.980 &       0 \\
%cerbu               &    grayware &         0.980 &       4 \\
%deceptpcclean       &    grayware &         0.980 &       4 \\
%dupzom              &  downloader &         0.980 &      14 \\
%glupteba            &    grayware &         0.980 &       1 \\
%convagent           &    grayware &         0.980 &      23 \\
%cobaltstrike        &  downloader &         0.980 &       3 \\
%ipamor              &    grayware &         0.980 &      39 \\
%offergenerator      &    grayware &         0.985 &       0 \\
%slimware            &    grayware &         0.985 &       0 \\
%kuaizip             &      adware &         0.985 &       1 \\
%pasta               &    grayware &         0.985 &      28 \\
%oficla              &    backdoor &         0.985 &      36 \\
%macoute             &        worm &         0.985 &       0 \\
%predator            &    grayware &         0.985 &      13 \\
%bladabindi          &    backdoor &         0.985 &      19 \\
%pcclient            &    backdoor &         0.985 &      30 \\
%ibryte              &      adware &         0.985 &       9 \\
%mucc                &    grayware &         0.985 &       0 \\
%mudrop              &  downloader &         0.985 &      37 \\
%imali               &      adware &         0.985 &       0 \\
%chifrax             &    grayware &         0.985 &      41 \\
%youxun              &    grayware &         0.985 &      11 \\
%refroso             &    backdoor &         0.985 &      41 \\
%trickster           &  downloader &         0.985 &       1 \\
%hotbar              &    grayware &         0.985 &      45 \\
%dealply             &    grayware &         0.985 &      19 \\
%fujacks             &       virus &         0.985 &      35 \\
%dorkbot             &        worm &         0.985 &       7 \\
%fraudpack           &   rogueware &         0.985 &       3 \\
%spigot              &    grayware &         0.985 &      20 \\
%plurox              &    backdoor &         0.985 &       0 \\
%tibia               &    grayware &         0.985 &      31 \\
%bifrose             &    backdoor &         0.985 &      33 \\
%alman               &       virus &         0.985 &      11 \\
%ulise               &    grayware &         0.985 &       2 \\
%qjwmonkey           &    grayware &         0.985 &      47 \\
%rising              &    grayware &         0.985 &      34 \\
%tenga               &       virus &         0.985 &       6 \\
%tdss                &  downloader &         0.985 &       6 \\
%crossrider          &    grayware &         0.985 &       1 \\
%shutdowner          &    grayware &         0.989 &       6 \\
%turkojan            &    backdoor &         0.990 &      16 \\
%auslogics           &    grayware &         0.990 &       3 \\
%perion              &    grayware &         0.990 &       0 \\
%jeefo               &       virus &         0.990 &      99 \\
%occamy              &    grayware &         0.990 &      26 \\
%amonetize           &    grayware &         0.990 &       7 \\
%omaneat             &     spyware &         0.990 &       7 \\
%jaik                &    grayware &         0.990 &       5 \\
%onescan             &    grayware &         0.990 &      38 \\
%kingsoft            &    grayware &         0.990 &      37 \\
%vbkryjetor          &  downloader &         0.990 &       4 \\
%usteal              &    grayware &         0.990 &      31 \\
%kelihos             &    backdoor &         0.990 &      12 \\
%kiser               &    grayware &         0.990 &      55 \\
%detrahere           &    grayware &         0.990 &       4 \\
%opencandy           &    grayware &         0.990 &      92 \\
%jacard              &    grayware &         0.990 &      34 \\
%upatre              &  downloader &         0.990 &       4 \\
%bancos              &     spyware &         0.990 &      44 \\
%tasker              &    grayware &         0.990 &      11 \\
%filefinder          &      adware &         0.990 &       3 \\
%strab               &  ransomware &         0.990 &      38 \\
%babar               &    grayware &         0.990 &       5 \\
%lockbit             &  ransomware &         0.990 &       0 \\
%lightstone          &    backdoor &         0.990 &      17 \\
%remcos              &    backdoor &         0.990 &       4 \\
%elemental           &    grayware &         0.990 &       0 \\
%tremp               &    grayware &         0.990 &       0 \\
%browsefox           &    grayware &         0.990 &       6 \\
%bredolab            &  downloader &         0.990 &      19 \\
%blackhole           &    backdoor &         0.990 &      32 \\
%installerex         &    grayware &         0.990 &       0 \\
%khalesi             &    grayware &         0.990 &       2 \\
%installmonster      &    grayware &         0.990 &      83 \\
%sillyfdc            &        worm &         0.990 &      55 \\
%cheatengine         &    grayware &         0.995 &       0 \\
%veil                &    grayware &         0.995 &       1 \\
%shandaadd           &      adware &         0.995 &      88 \\
%coins               &    grayware &         0.995 &      18 \\
%dynamer             &  downloader &         0.995 &      20 \\
%megasearch          &      adware &         0.995 &       0 \\
%ursnif              &       virus &         0.995 &      25 \\
%silentall           &    grayware &         0.995 &      77 \\
%emotetu             &  downloader &         0.995 &       5 \\
%dumpy               &        worm &         0.995 &       0 \\
%icloader            &    grayware &         0.995 &       2 \\
%mokes               &    backdoor &         0.995 &       1 \\
%idsohtu             &    grayware &         0.995 &       6 \\
%primecasino         &    grayware &         0.995 &       0 \\
%plugx               &    backdoor &         0.995 &       5 \\
%doina               &    grayware &         0.995 &      50 \\
%swisyn              &        worm &         0.995 &       7 \\
%loadmoney           &    grayware &         0.995 &       8 \\
%mytob               &        worm &         0.995 &      30 \\
%dstudio             &    grayware &         0.995 &       2 \\
%poison              &    backdoor &         0.995 &      24 \\
%explorerhijack      &  downloader &         0.995 &       1 \\
%guloader            &  downloader &         0.995 &       0 \\
%urelas              &    backdoor &         0.995 &      38 \\
%induc               &       virus &         0.995 &      56 \\
%zurgop              &  downloader &         0.995 &       3 \\
%lazy                &    grayware &         0.995 &       6 \\
%hacdef              &    backdoor &         0.995 &      21 \\
%crysis              &  ransomware &         0.995 &      27 \\
%spyrix              &    grayware &         0.995 &      56 \\
%palevo              &    backdoor &         0.995 &      22 \\
%windigo             &    grayware &         0.995 &       3 \\
%hpdefender          &    grayware &         0.995 &       0 \\
%necurs              &  downloader &         0.995 &       8 \\
%woool               &    grayware &         0.995 &      94 \\
%netwiredrc          &    backdoor &         0.995 &      24 \\
%tibs                &  downloader &         0.995 &      29 \\
%fragtor             &    grayware &         0.995 &      10 \\
%nanocore            &    backdoor &         0.995 &      22 \\
%adpack              &      adware &         0.995 &       2 \\
%avemaria            &     spyware &         0.995 &      12 \\
%quasar              &    backdoor &         0.995 &      48 \\
%gendal              &    grayware &         0.995 &      62 \\
%trickbot            &       miner &         0.995 &       0 \\
%triusor             &       virus &         0.995 &       0 \\
%dlhelper            &    grayware &         0.995 &      13 \\
%racealer            &    grayware &         0.995 &      32 \\
%atraps              &    grayware &         0.995 &      20 \\
%tufik               &       virus &         0.995 &       0 \\
%xyligan             &    backdoor &         0.995 &      55 \\
%bezigate            &    backdoor &         1.000 &      15 \\
%brontok             &        worm &         1.000 &      95 \\
%bingoml             &    grayware &         1.000 &      22 \\
%bitmin              &       miner &         1.000 &      25 \\
%blackie             &    grayware &         1.000 &       0 \\
%blackmoon           &    grayware &         1.000 &      74 \\
%blackshades         &        worm &         1.000 &       2 \\
%blamon              &    grayware &         1.000 &      33 \\
%blihan              &    backdoor &         1.000 &       0 \\
%bloored             &        worm &         1.000 &       0 \\
%bayrob              &     spyware &         1.000 &       1 \\
%carberp             &  downloader &         1.000 &       6 \\
%broskod             &  downloader &         1.000 &       1 \\
%brresmon            &    grayware &         1.000 &       1 \\
%bsymem              &    grayware &         1.000 &      25 \\
%bublik              &  downloader &         1.000 &      79 \\
%bundlore            &      adware &         1.000 &       2 \\
%bunitu              &    grayware &         1.000 &       0 \\
%burn                &    backdoor &         1.000 &       0 \\
%buterat             &     clicker &         1.000 &      17 \\
%bzub                &  downloader &         1.000 &       2 \\
%cambot              &        worm &         1.000 &       0 \\
%betload             &    grayware &         1.000 &       3 \\
%cardspy             &     spyware &         1.000 &     100 \\
%brook               &  ransomware &         1.000 &       0 \\
%berbew              &    backdoor &         1.000 &       0 \\
%memery              &       virus &         1.000 &       9 \\
%bebloh              &    backdoor &         1.000 &       1 \\
%catalina            &    grayware &         1.000 &       0 \\
%ludbaruma           &        worm &         1.000 &       0 \\
%lulusoftware        &    grayware &         1.000 &      13 \\
%lunastorm           &        worm &         1.000 &      97 \\
%mimail              &        worm &         1.000 &       0 \\
%lydra               &     spyware &         1.000 &       5 \\
%lyposit             &  ransomware &         1.000 &       0 \\
%mabezat             &        worm &         1.000 &       0 \\
%zygug               &    grayware &         1.000 &      52 \\
%maener              &       miner &         1.000 &       0 \\
%mailru              &    grayware &         1.000 &       0 \\
%benjamin            &        worm &         1.000 &      94 \\
%malex               &  downloader &         1.000 &       1 \\
%mapsgory            &  downloader &         1.000 &       0 \\
%mbrlock             &  downloader &         1.000 &       2 \\
%mepaow              &       virus &         1.000 &      97 \\
%mewsspy             &    backdoor &         1.000 &       6 \\
%miancha             &  downloader &         1.000 &      11 \\
%fraudrop            &  downloader &         1.000 &      31 \\
%fosniw              &  downloader &         1.000 &      42 \\
%formbook            &     spyware &         1.000 &      37 \\
%lovgate             &        worm &         1.000 &      29 \\
%bobax               &        worm &         1.000 &       3 \\
%beastdoor           &    backdoor &         1.000 &      71 \\
%manbat              &        worm &         1.000 &      44 \\
%bcryptinject        &  downloader &         1.000 &       0 \\
%ceatrg              &  downloader &         1.000 &      66 \\
%flystudio           &    grayware &         1.000 &      34 \\
%balrok              &        worm &         1.000 &       0 \\
%banbra              &    backdoor &         1.000 &      50 \\
%cerber              &  ransomware &         1.000 &      16 \\
%chrop               &      adware &         1.000 &      63 \\
%esecn               &      adware &         1.000 &     100 \\
%downer              &    grayware &         1.000 &      96 \\
%downloadguide       &    grayware &         1.000 &       0 \\
%downloadsponsor     &    grayware &         1.000 &      87 \\
%dpsk                &       miner &         1.000 &     100 \\
%drolnux             &        worm &         1.000 &       0 \\
%dropware            &      adware &         1.000 &       1 \\
%bactera             &        worm &         1.000 &       0 \\
%drstwex             &  downloader &         1.000 &       0 \\
%duote               &      adware &         1.000 &      98 \\
%eggnog              &        worm &         1.000 &       0 \\
%egroupdial          &    grayware &         1.000 &      87 \\
%emogen              &  downloader &         1.000 &      31 \\
%enosch              &        worm &         1.000 &       0 \\
%esaprof             &  downloader &         1.000 &      84 \\
%esfury              &        worm &         1.000 &       5 \\
%clipspy             &    grayware &         1.000 &       2 \\
%eyestye             &  downloader &         1.000 &      27 \\
%eyoorun             &    grayware &         1.000 &       0 \\
%loring              &        worm &         1.000 &     100 \\
%dumpex              &    grayware &         1.000 &      40 \\
%babonock            &        worm &         1.000 &       0 \\
%azorult             &    grayware &         1.000 &      57 \\
%axespec             &    grayware &         1.000 &       2 \\
%amigo               &    grayware &         1.000 &       0 \\
%aauto               &    grayware &         1.000 &      56 \\
%adaebook            &    grayware &         1.000 &     100 \\
%addlyrics           &      adware &         1.000 &       0 \\
%adposhel            &    grayware &         1.000 &       0 \\
%aenjaris            &    grayware &         1.000 &       0 \\
%agentb              &    grayware &         1.000 &      13 \\
%agentc              &    grayware &         1.000 &       0 \\
%agentcrypt          &    grayware &         1.000 &       0 \\
%agentino            &  downloader &         1.000 &       0 \\
%agobot              &    backdoor &         1.000 &      32 \\
%airinstaller        &    grayware &         1.000 &      87 \\
%aitinject           &    backdoor &         1.000 &       1 \\
%allaple             &        worm &         1.000 &       0 \\
%alyak               &  downloader &         1.000 &      55 \\
%antavmu             &        worm &         1.000 &       0 \\
%bandit              &  downloader &         1.000 &      61 \\
%apost               &  downloader &         1.000 &       1 \\
%ardamax             &    grayware &         1.000 &       1 \\
%arkeistealer        &    grayware &         1.000 &       6 \\
%ascentive           &    grayware &         1.000 &       0 \\
%atcpa               &       virus &         1.000 &       0 \\
%autinject           &        tool &         1.000 &       4 \\
%autog               &  downloader &         1.000 &       0 \\
%autoitinject        &    backdoor &         1.000 &      16 \\
%banload             &       miner &         1.000 &      49 \\
%lolojan             &    grayware &         1.000 &      95 \\
%hupigon             &    backdoor &         1.000 &      59 \\
%lolbot              &        worm &         1.000 &       0 \\
%kuluoz              &  downloader &         1.000 &       4 \\
%laqma               &    grayware &         1.000 &      12 \\
%horst               &    backdoor &         1.000 &      30 \\
%hematite            &       virus &         1.000 &       1 \\
%ldpinch             &        worm &         1.000 &      47 \\
%gigex               &        worm &         1.000 &       0 \\
%frosparf            &     clicker &         1.000 &      73 \\
%fsysna              &        worm &         1.000 &      66 \\
%gamania             &  downloader &         1.000 &       5 \\
%gamarue             &  downloader &         1.000 &      10 \\
%gamemodding         &    grayware &         1.000 &       6 \\
%ksdler              &      adware &         1.000 &      69 \\
%gametea             &  downloader &         1.000 &     100 \\
%gandcrypt           &  ransomware &         1.000 &       2 \\
%garrun              &    grayware &         1.000 &       0 \\
%gatak               &    grayware &         1.000 &      11 \\
%gator               &      adware &         1.000 &      47 \\
%geegly              &       virus &         1.000 &     100 \\
%gepys               &  downloader &         1.000 &       0 \\
%gify                &    grayware &         1.000 &       0 \\
%gimemo              &  ransomware &         1.000 &      54 \\
%hebogo              &    grayware &         1.000 &       0 \\
%gippers             &  ransomware &         1.000 &       0 \\
%goabeny             &    grayware &         1.000 &      75 \\
%gandcrab            &  ransomware &         1.000 &       3 \\
%gobot               &    backdoor &         1.000 &       4 \\
%kronosbot           &    backdoor &         1.000 &       0 \\
%kovter              &    grayware &         1.000 &       0 \\
%houndhack           &    backdoor &         1.000 &     100 \\
%ezsoftwareupdater   &    grayware &         1.000 &       0 \\
%icedid              &  downloader &         1.000 &       4 \\
%inbox               &    grayware &         1.000 &       0 \\
%injuke              &    grayware &         1.000 &      70 \\
%installiq           &    grayware &         1.000 &       2 \\
%istartsurf          &    grayware &         1.000 &       1 \\
%itorrent            &    grayware &         1.000 &       0 \\
%jevafus             &  downloader &         1.000 &      45 \\
%jimmy               &  ransomware &         1.000 &       0 \\
%johnnie             &    grayware &         1.000 &      65 \\
%krol                &        worm &         1.000 &       0 \\
%jpgiframe           &    grayware &         1.000 &       0 \\
%keydoor             &     spyware &         1.000 &       0 \\
%killwin             &    grayware &         1.000 &      58 \\
%hider               &    grayware &         1.000 &      59 \\
%klez                &        worm &         1.000 &       1 \\
%klone               &  downloader &         1.000 &      70 \\
%kolab               &    grayware &         1.000 &       1 \\
%kolovorot           &    grayware &         1.000 &       3 \\
%kolweb              &    grayware &         1.000 &      96 \\
%konus               &    backdoor &         1.000 &       0 \\
%koobface            &        worm &         1.000 &      77 \\
%koutodoor           &    backdoor &         1.000 &      16 \\
%kasidet             &    grayware &         1.000 &      19 \\
%gofot               &  downloader &         1.000 &      88 \\
%gogo                &       virus &         1.000 &       0 \\
%goldrv              &        worm &         1.000 &       0 \\
%ngrbot              &    backdoor &         1.000 &       0 \\
%nitol               &  downloader &         1.000 &       7 \\
%noon                &     spyware &         1.000 &      19 \\
%nymaim              &    backdoor &         1.000 &       1 \\
%nymeria             &    grayware &         1.000 &      32 \\
%oberal              &  downloader &         1.000 &       0 \\
%obit                &  downloader &         1.000 &       0 \\
%offend              &    grayware &         1.000 &      98 \\
%offercore           &    grayware &         1.000 &       0 \\
%onlinegames         &    grayware &         1.000 &      14 \\
%openinstall         &    grayware &         1.000 &      22 \\
%nevereg             &        worm &         1.000 &      51 \\
%orcus               &    backdoor &         1.000 &      42 \\
%mint                &    grayware &         1.000 &       3 \\
%mimdau              &  downloader &         1.000 &     100 \\
%lecna               &    backdoor &         1.000 &      24 \\
%lunam               &        worm &         1.000 &      99 \\
%lethic              &  downloader &         1.000 &       1 \\
%linkury             &    grayware &         1.000 &       0 \\
%lipler              &  downloader &         1.000 &       0 \\
%llac                &        worm &         1.000 &      30 \\
%lmir                &       virus &         1.000 &       2 \\
%locky               &  downloader &         1.000 &       5 \\
%lokibot             &    backdoor &         1.000 &      88 \\
%outbyte             &    grayware &         1.000 &       4 \\
%miniduke            &    backdoor &         1.000 &       0 \\
%neutrinopos         &  ransomware &         1.000 &      12 \\
%neshta              &       virus &         1.000 &       2 \\
%gorillaprice        &      adware &         1.000 &       6 \\
%gozi                &     spyware &         1.000 &       1 \\
%grenam              &       virus &         1.000 &       0 \\
%griptolo            &        worm &         1.000 &       7 \\
%growtopia           &    grayware &         1.000 &      69 \\
%hafen               &    grayware &         1.000 &       0 \\
%havex               &    grayware &         1.000 &       0 \\
%hebchengjiu         &      adware &         1.000 &       7 \\
%lassorm             &        worm &         1.000 &       0 \\
%lebreat             &    grayware &         1.000 &     100 \\
%pahooka             &        worm &         1.000 &     100 \\
%netstream           &    grayware &         1.000 &       0 \\
%mira                &        worm &         1.000 &      23 \\
%moarider            &        worm &         1.000 &      98 \\
%mocrt               &     spyware &         1.000 &      73 \\
%moonlight           &        worm &         1.000 &       8 \\
%mooqkel             &  downloader &         1.000 &     100 \\
%msposer             &  downloader &         1.000 &       4 \\
%mulinex             &  downloader &         1.000 &      65 \\
%multibar            &    grayware &         1.000 &      23 \\
%multiplier          &    grayware &         1.000 &       0 \\
%mydoom              &        worm &         1.000 &      83 \\
%neconyd             &     clicker &         1.000 &       0 \\
%neojit              &  downloader &         1.000 &       0 \\
%neoreklami          &      adware &         1.000 &       0 \\
%lollipop            &      adware &         1.000 &       0 \\
%facido              &  downloader &         1.000 &       0 \\
%winwrapper          &    grayware &         1.000 &      44 \\
%fakefire            &        worm &         1.000 &       3 \\
%vilsel              &  downloader &         1.000 &      41 \\
%virbox              &    grayware &         1.000 &       1 \\
%virfire             &        worm &         1.000 &       0 \\
%virlock             &       virus &         1.000 &       0 \\
%vittalia            &    grayware &         1.000 &       3 \\
%vobfus              &        worm &         1.000 &       0 \\
%voltar              &     clicker &         1.000 &       0 \\
%vundo               &        worm &         1.000 &      89 \\
%wenper              &        worm &         1.000 &      42 \\
%vybab               &        worm &         1.000 &       0 \\
%wabot               &    backdoor &         1.000 &      19 \\
%viking              &       virus &         1.000 &      98 \\
%wacatac             &    grayware &         1.000 &      14 \\
%wannacry            &  ransomware &         1.000 &       1 \\
%wapomi              &       virus &         1.000 &       8 \\
%wavipeg             &    backdoor &         1.000 &       0 \\
%webalta             &    grayware &         1.000 &       5 \\
%webcompanion        &    grayware &         1.000 &       0 \\
%webdialer           &      dialer &         1.000 &      86 \\
%webprefix           &  downloader &         1.000 &      12 \\
%wecod               &     spyware &         1.000 &      94 \\
%scrarev             &    grayware &         1.000 &       5 \\
%spyeye              &     spyware &         1.000 &       9 \\
%schoolgirl          &    grayware &         1.000 &       2 \\
%waldek              &    grayware &         1.000 &       0 \\
%rikihaki            &        worm &         1.000 &       0 \\
%vemply              &    grayware &         1.000 &      61 \\
%vbinder             &        tool &         1.000 &       1 \\
%xcnfe               &    grayware &         1.000 &       0 \\
%xiaobaminer         &       miner &         1.000 &      74 \\
%xihet               &  downloader &         1.000 &       8 \\
%xolxo               &        worm &         1.000 &      99 \\
%xorer               &       virus &         1.000 &      11 \\
%xtrat               &    backdoor &         1.000 &      58 \\
%winloadsda          &    grayware &         1.000 &      86 \\
%yahlover            &        worm &         1.000 &      65 \\
%ymacco              &    grayware &         1.000 &      68 \\
%yoddos              &    backdoor &         1.000 &      19 \\
%zapchast            &  downloader &         1.000 &       4 \\
%vebzenpak           &    grayware &         1.000 &       0 \\
%zbot                &  downloader &         1.000 &      24 \\
%zenlod              &  downloader &         1.000 &      22 \\
%zepfod              &        worm &         1.000 &       0 \\
%zeroaccess          &  downloader &         1.000 &      10 \\
%zlob                &  downloader &         1.000 &      21 \\
%zusy                &    grayware &         1.000 &       7 \\
%zvuzona             &    grayware &         1.000 &      79 \\
%winner              &    grayware &         1.000 &       0 \\
%winactivator        &        tool &         1.000 &       6 \\
%vawtrak             &    backdoor &         1.000 &       0 \\
%vtflooder           &  downloader &         1.000 &      55 \\
%vbclone             &  downloader &         1.000 &       0 \\
%zegost              &    backdoor &         1.000 &      28 \\
%qbot                &  downloader &         1.000 &       0 \\
%qihoo               &    grayware &         1.000 &       3 \\
%qqhack              &        tool &         1.000 &      98 \\
%pirminay            &  downloader &         1.000 &       9 \\
%pistolar            &  downloader &         1.000 &      76 \\
%plingky             &  downloader &         1.000 &      93 \\
%protux              &    backdoor &         1.000 &       4 \\
%pluto               &        worm &         1.000 &      34 \\
%pochi               &        worm &         1.000 &       0 \\
%pondfull            &        worm &         1.000 &       5 \\
%pornoblocker        &  ransomware &         1.000 &      14 \\
%powerless           &  downloader &         1.000 &      10 \\
%powerspider         &    backdoor &         1.000 &       0 \\
%prepscram           &    grayware &         1.000 &     100 \\
%pincav              &    backdoor &         1.000 &      18 \\
%privateexeprotector &    grayware &         1.000 &      19 \\
%rifdoor             &    backdoor &         1.000 &       0 \\
%4shared             &    grayware &         1.000 &       1 \\
%rostpay             &    grayware &         1.000 &      96 \\
%roxer               &    grayware &         1.000 &      97 \\
%ruledor             &    backdoor &         1.000 &       0 \\
%safebytes           &    grayware &         1.000 &      99 \\
%ruskill             &    backdoor &         1.000 &       7 \\
%scarsi              &  downloader &         1.000 &       8 \\
%salgorea            &  downloader &         1.000 &       0 \\
%rums                &  downloader &         1.000 &       0 \\
%rungbu              &        worm &         1.000 &      18 \\
%prorat              &    backdoor &         1.000 &      69 \\
%pidgeon             &       virus &         1.000 &      16 \\
%picsys              &        worm &         1.000 &     100 \\
%phorpiex            &        worm &         1.000 &      12 \\
%qqpass              &  downloader &         1.000 &      94 \\
%qqware              &    grayware &         1.000 &      50 \\
%qshell              &    grayware &         1.000 &       0 \\
%qzonit              &     spyware &         1.000 &      87 \\
%raccrypt            &  ransomware &         1.000 &       0 \\
%ramnit              &       virus &         1.000 &      50 \\
%ranumbot            &    grayware &         1.000 &      28 \\
%rebhip              &        worm &         1.000 &      16 \\
%recex               &       miner &         1.000 &      11 \\
%recodrop            &  downloader &         1.000 &       0 \\
%reconyc             &    grayware &         1.000 &      36 \\
%redcap              &  downloader &         1.000 &      18 \\
%refinka             &    grayware &         1.000 &       1 \\
%regrun              &  ransomware &         1.000 &     100 \\
%regsup              &  downloader &         1.000 &       1 \\
%reline              &     spyware &         1.000 &      57 \\
%renos               &  downloader &         1.000 &      17 \\
%reptile             &    grayware &         1.000 &       0 \\
%qaccel              &     clicker &         1.000 &       0 \\
%pykspa              &        worm &         1.000 &       0 \\
%pterodo             &  downloader &         1.000 &       0 \\
%plemood             &        worm &         1.000 &       0 \\
%paneidix            &    backdoor &         1.000 &       0 \\
%pedex               &    backdoor &         1.000 &     100 \\
%phishbank           &        worm &         1.000 &       0 \\
%xanfpezes           &    grayware &         1.000 &     100 \\
%fakedoc             &        worm &         1.000 &       0 \\
%wsgame              &    grayware &         1.000 &      49 \\
%wonton              &  downloader &         1.000 &       2 \\
%daws                &  downloader &         1.000 &       2 \\
%detroie             &       virus &         1.000 &       2 \\
%dexel               &  downloader &         1.000 &       0 \\
%deyma               &  downloader &         1.000 &      21 \\
%diamin              &      dialer &         1.000 &      80 \\
%digs                &       miner &         1.000 &       0 \\
%dinwod              &  downloader &         1.000 &      98 \\
%diss                &    grayware &         1.000 &       3 \\
%disttrack           &    grayware &         1.000 &       0 \\
%dluca               &  downloader &         1.000 &      84 \\
%dodiw               &    backdoor &         1.000 &      83 \\
%darkkomet           &    backdoor &         1.000 &      14 \\
%dofoil              &  downloader &         1.000 &       6 \\
%pacex               &       miner &         1.000 &       0 \\
%macri               &    backdoor &         1.000 &      58 \\
%pajetbin            &        worm &         1.000 &      91 \\
%schwarzesonne       &    backdoor &         1.000 &      48 \\
%stampado            &  ransomware &         1.000 &      58 \\
%startsurf           &    grayware &         1.000 &       3 \\
%stelega             &    grayware &         1.000 &      50 \\
%stihat              &        worm &         1.000 &     100 \\
%stone               &       virus &         1.000 &      97 \\
%stop                &  ransomware &         1.000 &       0 \\
%stopcrypt           &  ransomware &         1.000 &       0 \\
%domaiq              &    grayware &         1.000 &      53 \\
%stormattack         &  downloader &         1.000 &       0 \\
%dalexis             &  downloader &         1.000 &       0 \\
%cyfin               &    grayware &         1.000 &       5 \\
%fakefolder          &        worm &         1.000 &      71 \\
%fakens              &      adware &         1.000 &       0 \\
%fareit              &    grayware &         1.000 &      14 \\
%fasong              &        worm &         1.000 &      78 \\
%fesber              &        worm &         1.000 &      33 \\
%ficker              &    grayware &         1.000 &      15 \\
%finfish             &    backdoor &         1.000 &       0 \\
%firseria            &    grayware &         1.000 &       8 \\
%dostre              &  downloader &         1.000 &       0 \\
%dorv                &  downloader &         1.000 &       8 \\
%dorifel             &  downloader &         1.000 &       5 \\
%dadobra             &  downloader &         1.000 &      63 \\
%dorgam              &  downloader &         1.000 &      19 \\
%connectwise         &        tool &         1.000 &       0 \\
%contenedor          &       virus &         1.000 &       0 \\
%convertad           &      adware &         1.000 &       1 \\
%coroxy              &    backdoor &         1.000 &       0 \\
%cosmicduke          &    backdoor &         1.000 &       4 \\
%cosmu               &       virus &         1.000 &       0 \\
%cossta              &    grayware &         1.000 &      13 \\
%cryptinject         &  downloader &         1.000 &      34 \\
%cryptowall          &  ransomware &         1.000 &       2 \\
%cutwail             &  downloader &         1.000 &      10 \\
%cycbot              &    backdoor &         1.000 &       0 \\
%cmy3u               &    grayware &         1.000 &      98 \\
%subseven            &    backdoor &         1.000 &      69 \\
%swizzor             &    grayware &         1.000 &       6 \\
%swjoy               &    grayware &         1.000 &       0 \\
%shyape              &  downloader &         1.000 &      39 \\
%shylock             &    backdoor &         1.000 &       3 \\
%sillyp2p            &        worm &         1.000 &       1 \\
%simda               &    backdoor &         1.000 &      11 \\
%soulclose           &        worm &         1.000 &       0 \\
%sinau               &       virus &         1.000 &       0 \\
%siscos              &  downloader &         1.000 &      48 \\
%sivis               &       virus &         1.000 &      72 \\
%skintrim            &      adware &         1.000 &       2 \\
%snojan              &  downloader &         1.000 &       1 \\
%socelars            &     spyware &         1.000 &       1 \\
%shodi               &       virus &         1.000 &       0 \\
%socks               &        worm &         1.000 &      18 \\
%softpulse           &    grayware &         1.000 &      34 \\
%sohana              &  downloader &         1.000 &      18 \\
%sohanad             &        worm &         1.000 &      66 \\
%solmyr              &     spyware &         1.000 &      58 \\
%unruy               &  downloader &         1.000 &      13 \\
%upantix             &  downloader &         1.000 &     100 \\
%updane              &    grayware &         1.000 &       0 \\
%xorist              &  downloader &         1.000 &      24 \\
%winwebsec           &   rogueware &         1.000 &      21 \\
%killmbr             &    grayware &         1.000 &       9 \\
%wlksm               &       virus &         1.000 &       1 \\
%softonic            &      adware &         1.000 &      79 \\
%shiz                &    backdoor &         1.000 &       0 \\
%shipup              &  downloader &         1.000 &      30 \\
%shade               &  ransomware &         1.000 &       5 \\
%syncopate           &    grayware &         1.000 &      20 \\
%sysn                &  downloader &         1.000 &      19 \\
%sytro               &        worm &         1.000 &      45 \\
%taskloader          &      adware &         1.000 &       0 \\
%tempedreve          &       virus &         1.000 &       0 \\
%teslacrypt          &  ransomware &         1.000 &       1 \\
%tiggre              &    grayware &         1.000 &      88 \\
%tinba               &  downloader &         1.000 &      15 \\
%titirez             &    grayware &         1.000 &       5 \\
%tnega               &  downloader &         1.000 &      33 \\
%tofsee              &    backdoor &         1.000 &       9 \\
%tonmye              &    grayware &         1.000 &      84 \\
%tougle              &    grayware &         1.000 &       0 \\
%trymedia            &      adware &         1.000 &      73 \\
%tupym               &        worm &         1.000 &       0 \\
%umbra               &  downloader &         1.000 &       0 \\
%spybot              &        worm &         1.000 &      15 \\
%spesr               &        worm &         1.000 &       0 \\
%speedcat            &    grayware &         1.000 &       0 \\
%simbot              &    backdoor &         1.000 &       1 \\
%screenmate          &    grayware &         1.000 &       1 \\
%sdbot               &    backdoor &         1.000 &      92 \\
%seraph              &  downloader &         1.000 &       0 \\
%seven               &  ransomware &         1.000 &       0 \\
%sfone               &        worm &         1.000 &      65 \\
%woozlist            &    grayware &         1.000 &      90 \\
%zylom               &  downloader &         1.000 &       0 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_binary_bestAndWorst_dynamic.tex <==
\begin{table}[h]
\setlength\tabcolsep{4pt}
\centering
\small
\caption{Top-10 malware families with the lowest binary classification accuracy using
	dynamic features (i.e., highest mispredictions as goodware).}
\label{tbl:binary_dyn_bestAndWorst}
\begin{tabular}{llccc}
\toprule
\multicolumn{5}{c}{\textbf{Dynamic binary classification}}\\
\textbf{Family} & \textbf{Class} & \textbf{Avg Recall} & \textbf{Packed} &  \textbf{FMR}\\
\midrule
tasker   		&       grayware	   	&  	0.0 	& 11\%  & 0.77	\\
malex           &       downloader		&   0.0		& 1\%	& 0.77 	\\
rostpay      	&       grayware    	&   0.0		& 96\%	& 0.76	\\
constructor     &       grayware      	&   0.0		& 13\%	& 0.78	\\
atcpa           &       virus     		&   0.0		& 0\%	& 0.78	\\
mocrt          	&       spyware  		&  	0.0		& 73\%	& 0.80	\\
mokes           &       backdoor  		&   0.0		& 1\%	& 0.65	\\
bingoml         &       grayware  		&   0.0		& 22\%	& 0.72  \\
safebytes       &       grayware  		&   0.0		& 99\%	& 0.81	\\
trymedia        &       adware  		&   0.0		& 73\%	& 0.70	\\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_binary_bestAndWorst_static.tex <==
\begin{table}[h]
\centering
\small
\caption{Top-10 malware families with the lowest binary classification accuracy using the
	static features (i.e., highest mispredictions as goodware).}
\label{tbl:binary_static_bestAndWorst}
\begin{tabular}{llcr}
\toprule
\multicolumn{4}{c}{\textbf{Static binary classification}}\\
	\textbf{Family} & \textbf{Class} &  \textbf{Avg Recall} &  \textbf{\% packed} \\
\midrule
pioneer             &       virus &         0.401 &       6\% \\
asparnet            &    grayware &         0.410 &       5\% \\
systweak            &    grayware &         0.458 &      19\% \\
shopper             &    grayware &         0.500 &       1\% \\
sality              &       virus &         0.516 &       4\% \\
vitro               &       virus &         0.553 &       3\% \\
installcore         &    grayware &         0.596 &      10\% \\
slugin              &       virus &         0.598 &       4\% \\
elex                &      adware &         0.603 &       9\% \\
passview            &    grayware &         0.617 &      35\% \\
%conduit             &    grayware &         0.627 &      35\% \\
%zpevdo              &    grayware &         0.636 &      15\% \\
%copidmbe            &       virus &         0.646 &       9\% \\
%wajam               &      adware &         0.650 &       2\% \\
%iobit               &    grayware &         0.654 &      38\% \\
%mywebsearch         &    grayware &         0.656 &       1\% \\
%wlksm               &       virus &         0.667 &       1\% \\
%toptools            &    grayware &         0.703 &       0\% \\
%kraddare            &      adware &         0.706 &      36\% \\
%tenga               &       virus &         0.716 &       6\% \\
%expiro              &       virus &         0.722 &      10\% \\
%opensupdater        &      adware &         0.724 &      14\% \\
%chir                &        worm &         0.737 &      12\% \\
%driverpack          &    grayware &         0.748 &      13\% \\
%parite              &       virus &         0.752 &       7\% \\
%kuaiba              &      adware &         0.753 &       5\% \\
%softcnapp           &      adware &         0.758 &       0\% \\
%uwamson             &    grayware &         0.758 &      15\% \\
%citeary             &        worm &         0.759 &      16\% \\
%browsefox           &    grayware &         0.759 &       6\% \\
%presenoker          &    grayware &         0.761 &      16\% \\
%deceptpcclean       &    grayware &         0.766 &       4\% \\
%diztakun            &    grayware &         0.770 &      27\% \\
%diskwriter          &    grayware &         0.781 &      29\% \\
%petya               &  ransomware &         0.782 &      16\% \\
%gamevance           &      adware &         0.786 &       5\% \\
%onescan             &    grayware &         0.787 &      38\% \\
%dupzom              &  downloader &         0.795 &      14\% \\
%pcclient            &    backdoor &         0.796 &      30\% \\
%vrbrothers          &      adware &         0.797 &      88\% \\
%rozena              &    backdoor &         0.802 &       3\% \\
%expressdownloader   &    grayware &         0.802 &      62\% \\
%schoolboy           &    grayware &         0.807 &       7\% \\
%rbot                &        worm &         0.812 &      19\% \\
%alman               &       virus &         0.814 &      11\% \\
%geral               &  downloader &         0.815 &      23\% \\
%tibia               &    grayware &         0.816 &      31\% \\
%mediaget            &    grayware &         0.821 &      33\% \\
%polypatch           &    grayware &         0.821 &      99\% \\
%bulz                &    grayware &         0.821 &      15\% \\
%buzy                &        worm &         0.828 &      35\% \\
%burden              &      adware &         0.832 &       2\% \\
%zurgop              &  downloader &         0.832 &       3\% \\
%filefinder          &      adware &         0.833 &       3\% \\
%speedingupmypc      &    grayware &         0.836 &      11\% \\
%zvuzona             &    grayware &         0.840 &      79\% \\
%sogou               &    grayware &         0.840 &      17\% \\
%relevantknowledge   &      adware &         0.841 &       0\% \\
%downloadadmin       &    grayware &         0.842 &       3\% \\
%loadmoney           &    grayware &         0.846 &       8\% \\
%induc               &       virus &         0.851 &      56\% \\
%bestafera           &    grayware &         0.851 &      57\% \\
%mudrop              &  downloader &         0.852 &      37\% \\
%virut               &       virus &         0.852 &       3\% \\
%bandoo              &    grayware &         0.854 &       0\% \\
%kingsoft            &    grayware &         0.854 &      37\% \\
%ymacco              &    grayware &         0.854 &      68\% \\
%mokes               &    backdoor &         0.855 &       1\% \\
%ibryte              &      adware &         0.857 &       9\% \\
%ipamor              &    grayware &         0.859 &      39\% \\
%emotet              &  downloader &         0.860 &       1\% \\
%installbrain        &    grayware &         0.860 &       2\% \\
%techsnab            &    grayware &         0.862 &       2\% \\
%alien               &  downloader &         0.862 &      20\% \\
%qihoo               &    grayware &         0.863 &       3\% \\
%pcacceleratepro     &    grayware &         0.864 &       1\% \\
%auslogics           &    grayware &         0.865 &       3\% \\
%convagent           &    grayware &         0.868 &      23\% \\
%triusor             &       virus &         0.869 &       0\% \\
%siscos              &  downloader &         0.871 &      48\% \\
%ekstak              &    grayware &         0.872 &      31\% \\
%clipbanker          &    grayware &         0.873 &      11\% \\
%adgazelle           &    grayware &         0.873 &       0\% \\
%crossrider          &    grayware &         0.874 &       1\% \\
%lotok               &    backdoor &         0.875 &      15\% \\
%menti               &        worm &         0.876 &      11\% \\
%skillis             &    grayware &         0.877 &      19\% \\
%fakefire            &        worm &         0.878 &       3\% \\
%bancos              &     spyware &         0.879 &      44\% \\
%blackie             &    grayware &         0.879 &       0\% \\
%kiser               &    grayware &         0.880 &      55\% \\
%amonetize           &    grayware &         0.887 &       7\% \\
%killmbr             &    grayware &         0.887 &       9\% \\
%constructor         &    grayware &         0.887 &      13\% \\
%netwiredrc          &    backdoor &         0.888 &      24\% \\
%cobra               &    grayware &         0.888 &      60\% \\
%mabezat             &        worm &         0.890 &       0\% \\
%remoteutilities     &    grayware &         0.893 &      90\% \\
%reline              &     spyware &         0.893 &      57\% \\
%smartpcsolutions    &    grayware &         0.894 &      46\% \\
%nanocore            &    backdoor &         0.897 &      22\% \\
%crysis              &  ransomware &         0.897 &      27\% \\
%jatif               &    grayware &         0.898 &       2\% \\
%anmalpro            &    grayware &         0.898 &       0\% \\
%bladabindi          &    backdoor &         0.898 &      19\% \\
%neshta              &       virus &         0.900 &       2\% \\
%rising              &    grayware &         0.901 &      34\% \\
%buterat             &     clicker &         0.901 &      17\% \\
%waldek              &    grayware &         0.902 &       0\% \\
%ramnit              &       virus &         0.903 &      50\% \\
%fujacks             &       virus &         0.904 &      35\% \\
%cryptowall          &  ransomware &         0.904 &       2\% \\
%lazy                &    grayware &         0.904 &       6\% \\
%chifrax             &    grayware &         0.905 &      41\% \\
%airinstaller        &    grayware &         0.905 &      87\% \\
%buzus               &  downloader &         0.906 &       3\% \\
%zlob                &  downloader &         0.907 &      21\% \\
%pterodo             &  downloader &         0.908 &       0\% \\
%shutdowner          &    grayware &         0.908 &       6\% \\
%speedbit            &    grayware &         0.909 &       8\% \\
%usteal              &    grayware &         0.911 &      31\% \\
%sdum                &    grayware &         0.911 &      24\% \\
%xyligan             &    backdoor &         0.912 &      55\% \\
%installiq           &    grayware &         0.914 &       2\% \\
%bingoml             &    grayware &         0.914 &      22\% \\
%utorrent            &    grayware &         0.914 &      72\% \\
%bifrose             &    backdoor &         0.916 &      33\% \\
%cjishu              &      adware &         0.917 &       1\% \\
%lulusoftware        &    grayware &         0.918 &      13\% \\
%sabsik              &    grayware &         0.918 &      30\% \\
%gamini              &    grayware &         0.918 &       0\% \\
%dorgam              &  downloader &         0.919 &      19\% \\
%imali               &      adware &         0.919 &       0\% \\
%bsymem              &    grayware &         0.920 &      25\% \\
%fugrafa             &    grayware &         0.921 &       8\% \\
%mucc                &    grayware &         0.923 &       0\% \\
%pornoblocker        &  ransomware &         0.924 &      14\% \\
%winner              &    grayware &         0.924 &       0\% \\
%spigot              &    grayware &         0.924 &      20\% \\
%binder              &  downloader &         0.925 &      16\% \\
%gorillaprice        &      adware &         0.925 &       6\% \\
%scrop               &  downloader &         0.925 &      12\% \\
%babar               &    grayware &         0.926 &       5\% \\
%coins               &    grayware &         0.926 &      18\% \\
%llac                &        worm &         0.929 &      30\% \\
%plugx               &    backdoor &         0.929 &       5\% \\
%macri               &    backdoor &         0.929 &      58\% \\
%dealply             &    grayware &         0.930 &      19\% \\
%agentb              &    grayware &         0.931 &      13\% \\
%sodinokibi          &    grayware &         0.932 &       2\% \\
%veil                &    grayware &         0.932 &       1\% \\
%slimware            &    grayware &         0.933 &       0\% \\
%pirminay            &  downloader &         0.933 &       9\% \\
%hpdefender          &    grayware &         0.935 &       0\% \\
%winwrapper          &    grayware &         0.936 &      44\% \\
%shade               &  ransomware &         0.936 &       5\% \\
%neutrinopos         &  ransomware &         0.937 &      12\% \\
%adpack              &      adware &         0.937 &       2\% \\
%noon                &     spyware &         0.937 &      19\% \\
%firseria            &    grayware &         0.937 &       8\% \\
%banbra              &    backdoor &         0.937 &      50\% \\
%jacard              &    grayware &         0.937 &      34\% \\
%dumpex              &    grayware &         0.937 &      40\% \\
%titirez             &    grayware &         0.938 &       5\% \\
%poison              &    backdoor &         0.938 &      24\% \\
%taranis             &    grayware &         0.938 &       4\% \\
%xorer               &       virus &         0.938 &      11\% \\
%oficla              &    backdoor &         0.938 &      36\% \\
%palevo              &    backdoor &         0.938 &      22\% \\
%emotetu             &  downloader &         0.938 &       5\% \\
%openinstall         &    grayware &         0.939 &      22\% \\
%trickbot            &       miner &         0.939 &       0\% \\
%webalta             &    grayware &         0.942 &       5\% \\
%kelihos             &    backdoor &         0.942 &      12\% \\
%cossta              &    grayware &         0.943 &      13\% \\
%bayrob              &     spyware &         0.943 &       1\% \\
%linkury             &    grayware &         0.943 &       0\% \\
%cryptinject         &  downloader &         0.944 &      34\% \\
%quasar              &    backdoor &         0.944 &      48\% \\
%zbot                &  downloader &         0.945 &      24\% \\
%zard                &    grayware &         0.945 &       3\% \\
%swisyn              &        worm &         0.946 &       7\% \\
%pasta               &    grayware &         0.948 &      28\% \\
%cerbu               &    grayware &         0.948 &       4\% \\
%gendal              &    grayware &         0.949 &      62\% \\
%brresmon            &    grayware &         0.949 &       1\% \\
%downloadassistant   &    grayware &         0.949 &      18\% \\
%rostpay             &    grayware &         0.949 &      96\% \\
%youxun              &    grayware &         0.950 &      11\% \\
%nymaim              &    backdoor &         0.950 &       1\% \\
%zegost              &    backdoor &         0.950 &      28\% \\
%ldpinch             &        worm &         0.950 &      47\% \\
%orcus               &    backdoor &         0.950 &      42\% \\
%wonton              &  downloader &         0.950 &       2\% \\
%tisandr             &        worm &         0.951 &       0\% \\
%farfli              &    backdoor &         0.951 &      38\% \\
%fragtor             &    grayware &         0.951 &      10\% \\
%flystudio           &    grayware &         0.951 &      34\% \\
%sysn                &  downloader &         0.951 &      19\% \\
%soulclose           &        worm &         0.951 &       0\% \\
%fosniw              &  downloader &         0.951 &      42\% \\
%onlinegames         &    grayware &         0.951 &      14\% \\
%midie               &    grayware &         0.952 &      33\% \\
%dstudio             &    grayware &         0.952 &       2\% \\
%prorat              &    backdoor &         0.955 &      69\% \\
%vkontaktedj         &    grayware &         0.955 &       4\% \\
%webprefix           &  downloader &         0.955 &      12\% \\
%zapchast            &  downloader &         0.955 &       4\% \\
%lovgate             &        worm &         0.955 &      29\% \\
%bandit              &  downloader &         0.956 &      61\% \\
%ksdler              &      adware &         0.956 &      69\% \\
%tnega               &  downloader &         0.956 &      33\% \\
%hotbar              &    grayware &         0.956 &      45\% \\
%mint                &    grayware &         0.956 &       3\% \\
%dynamer             &  downloader &         0.956 &      20\% \\
%carberp             &  downloader &         0.956 &       6\% \\
%gamarue             &  downloader &         0.956 &      10\% \\
%viking              &       virus &         0.956 &      98\% \\
%occamy              &    grayware &         0.956 &      26\% \\
%remcos              &    backdoor &         0.957 &       4\% \\
%ardamax             &    grayware &         0.957 &       1\% \\
%gimemo              &  ransomware &         0.957 &      54\% \\
%getnow              &    grayware &         0.957 &      88\% \\
%silentall           &    grayware &         0.957 &      77\% \\
%ursu                &    grayware &         0.957 &      23\% \\
%jaik                &    grayware &         0.957 &       5\% \\
%yoddos              &    backdoor &         0.961 &      19\% \\
%icloader            &    grayware &         0.961 &       2\% \\
%koutodoor           &    backdoor &         0.962 &      16\% \\
%installerex         &    grayware &         0.962 &       0\% \\
%avemaria            &     spyware &         0.962 &      12\% \\
%ursnif              &       virus &         0.962 &      25\% \\
%redcap              &  downloader &         0.962 &      18\% \\
%yandex              &    grayware &         0.962 &       0\% \\
%cosmicduke          &    backdoor &         0.962 &       4\% \\
%primecasino         &    grayware &         0.962 &       0\% \\
%klone               &  downloader &         0.962 &      70\% \\
%kuaizip             &      adware &         0.962 &       1\% \\
%sinau               &       virus &         0.962 &       0\% \\
%softonic            &      adware &         0.963 &      79\% \\
%emogen              &  downloader &         0.963 &      31\% \\
%ruskill             &    backdoor &         0.963 &       7\% \\
%subseven            &    backdoor &         0.963 &      69\% \\
%aenjaris            &    grayware &         0.963 &       0\% \\
%explorerhijack      &  downloader &         0.963 &       1\% \\
%bitmin              &       miner &         0.963 &      25\% \\
%shandaadd           &      adware &         0.968 &      88\% \\
%offergenerator      &    grayware &         0.968 &       0\% \\
%jeefo               &       virus &         0.968 &      99\% \\
%refroso             &    backdoor &         0.968 &      41\% \\
%stelega             &    grayware &         0.968 &      50\% \\
%autinject           &        tool &         0.968 &       4\% \\
%convertad           &      adware &         0.968 &       1\% \\
%woool               &    grayware &         0.968 &      94\% \\
%schoolgirl          &    grayware &         0.968 &       2\% \\
%horst               &    backdoor &         0.969 &      30\% \\
%zusy                &    grayware &         0.969 &       7\% \\
%hupigon             &    backdoor &         0.969 &      59\% \\
%tremp               &    grayware &         0.969 &       0\% \\
%cridex              &    grayware &         0.969 &      15\% \\
%lethic              &  downloader &         0.969 &       1\% \\
%scarsi              &  downloader &         0.969 &       8\% \\
%lockbit             &  ransomware &         0.969 &       0\% \\
%gogo                &       virus &         0.969 &       0\% \\
%installmonster      &    grayware &         0.969 &      83\% \\
%khalesi             &    grayware &         0.969 &       2\% \\
%staser              &  downloader &         0.969 &      61\% \\
%frosparf            &     clicker &         0.969 &      73\% \\
%4shared             &    grayware &         0.969 &       1\% \\
%webcompanion        &    grayware &         0.970 &       0\% \\
%cobaltstrike        &  downloader &         0.970 &       3\% \\
%trickster           &  downloader &         0.970 &       1\% \\
%fraudrop            &  downloader &         0.974 &      31\% \\
%tasker              &    grayware &         0.974 &      11\% \\
%istartsurf          &    grayware &         0.975 &       1\% \\
%alyak               &  downloader &         0.975 &      55\% \\
%blamon              &    grayware &         0.975 &      33\% \\
%fsysna              &        worm &         0.975 &      66\% \\
%inbox               &    grayware &         0.975 &       0\% \\
%aauto               &    grayware &         0.975 &      56\% \\
%zeroaccess          &  downloader &         0.975 &      10\% \\
%atraps              &    grayware &         0.975 &      20\% \\
%dodiw               &    backdoor &         0.975 &      83\% \\
%autoitinject        &    backdoor &         0.975 &      16\% \\
%bloored             &        worm &         0.975 &       0\% \\
%tibs                &  downloader &         0.975 &      29\% \\
%detrahere           &    grayware &         0.975 &       4\% \\
%updane              &    grayware &         0.975 &       0\% \\
%darkkomet           &    backdoor &         0.975 &      14\% \\
%screenmate          &    grayware &         0.975 &       1\% \\
%predator            &    grayware &         0.975 &      13\% \\
%dlhelper            &    grayware &         0.975 &      13\% \\
%sohanad             &        worm &         0.976 &      66\% \\
%diss                &    grayware &         0.976 &       3\% \\
%fareit              &    grayware &         0.976 &      14\% \\
%hacdef              &    backdoor &         0.976 &      21\% \\
%teslacrypt          &  ransomware &         0.976 &       1\% \\
%shylock             &    backdoor &         0.981 &       3\% \\
%antavmu             &        worm &         0.981 &       0\% \\
%vbkryjetor          &  downloader &         0.981 &       4\% \\
%nitol               &  downloader &         0.981 &       7\% \\
%fesber              &        worm &         0.981 &      33\% \\
%cycbot              &    backdoor &         0.981 &       0\% \\
%gippers             &  ransomware &         0.981 &       0\% \\
%wapomi              &       virus &         0.981 &       8\% \\
%ficker              &    grayware &         0.981 &      15\% \\
%winloadsda          &    grayware &         0.981 &      86\% \\
%qjwmonkey           &    grayware &         0.981 &      47\% \\
%cheatengine         &    grayware &         0.981 &       0\% \\
%opencandy           &    grayware &         0.981 &      92\% \\
%msposer             &  downloader &         0.981 &       4\% \\
%megasearch          &      adware &         0.981 &       0\% \\
%gozi                &     spyware &         0.981 &       1\% \\
%racealer            &    grayware &         0.981 &      32\% \\
%esfury              &        worm &         0.981 &       5\% \\
%plurox              &    backdoor &         0.981 &       0\% \\
%mytob               &        worm &         0.981 &      30\% \\
%lamer               &       virus &         0.981 &      43\% \\
%xtrat               &    backdoor &         0.981 &      58\% \\
%tinba               &  downloader &         0.981 &      15\% \\
%hematite            &       virus &         0.981 &       1\% \\
%fraudpack           &   rogueware &         0.981 &       3\% \\
%omaneat             &     spyware &         0.981 &       7\% \\
%grenam              &       virus &         0.981 &       0\% \\
%turkojan            &    backdoor &         0.981 &      16\% \\
%paneidix            &    backdoor &         0.981 &       0\% \\
%lightstone          &    backdoor &         0.981 &      17\% \\
%killwin             &    grayware &         0.981 &      58\% \\
%sillyfdc            &        worm &         0.981 &      55\% \\
%safebytes           &    grayware &         0.981 &      99\% \\
%hafen               &    grayware &         0.981 &       0\% \\
%bezigate            &    backdoor &         0.981 &      15\% \\
%benjamin            &        worm &         0.982 &      94\% \\
%agobot              &    backdoor &         0.982 &      32\% \\
%vebzenpak           &    grayware &         0.982 &       0\% \\
%swizzor             &    grayware &         0.982 &       6\% \\
%gamania             &  downloader &         0.982 &       5\% \\
%glupteba            &    grayware &         0.987 &       1\% \\
%spybot              &        worm &         0.987 &      15\% \\
%domaiq              &    grayware &         0.987 &      53\% \\
%strab               &  ransomware &         0.987 &      38\% \\
%tiggre              &    grayware &         0.987 &      88\% \\
%malex               &  downloader &         0.987 &       1\% \\
%softpulse           &    grayware &         0.987 &      34\% \\
%tufik               &       virus &         0.987 &       0\% \\
%tdss                &  downloader &         0.987 &       6\% \\
%dumpy               &        worm &         0.987 &       0\% \\
%vemply              &    grayware &         0.987 &      61\% \\
%azorult             &    grayware &         0.987 &      57\% \\
%arkeistealer        &    grayware &         0.987 &       6\% \\
%qbot                &  downloader &         0.987 &       0\% \\
%neconyd             &     clicker &         0.987 &       0\% \\
%solmyr              &     spyware &         0.988 &      58\% \\
%regsup              &  downloader &         0.988 &       1\% \\
%vilsel              &  downloader &         0.988 &      41\% \\
%fakefolder          &        worm &         0.988 &      71\% \\
%deyma               &  downloader &         0.988 &      21\% \\
%zylom               &  downloader &         0.988 &       0\% \\
%vittalia            &    grayware &         0.988 &       3\% \\
%nymeria             &    grayware &         0.988 &      32\% \\
%lydra               &     spyware &         0.988 &       5\% \\
%stop                &  ransomware &         0.988 &       0\% \\
%sdbot               &    backdoor &         0.988 &      92\% \\
%growtopia           &    grayware &         0.988 &      69\% \\
%spesr               &        worm &         0.988 &       0\% \\
%kolab               &    grayware &         0.988 &       1\% \\
%spyrix              &    grayware &         0.988 &      56\% \\
%miancha             &  downloader &         0.988 &      11\% \\
%snojan              &  downloader &         0.988 &       1\% \\
%sillyp2p            &        worm &         0.988 &       1\% \\
%duote               &      adware &         0.988 &      98\% \\
%rebhip              &        worm &         0.988 &      16\% \\
%dorifel             &  downloader &         0.988 &       5\% \\
%blackmoon           &    grayware &         0.988 &      74\% \\
%gatak               &    grayware &         0.988 &      11\% \\
%startsurf           &    grayware &         0.988 &       3\% \\
%lokibot             &    backdoor &         0.988 &      88\% \\
%webdialer           &      dialer &         0.988 &      86\% \\
%cmy3u               &    grayware &         0.988 &      98\% \\
%zenlod              &  downloader &         0.988 &      22\% \\
%winwebsec           &   rogueware &         0.988 &      21\% \\
%outbyte             &    grayware &         0.988 &       4\% \\
%schwarzesonne       &    backdoor &         0.988 &      48\% \\
%ranumbot            &    grayware &         0.988 &      28\% \\
%clipspy             &    grayware &         0.988 &       2\% \\
%spyeye              &     spyware &         0.988 &       9\% \\
%bredolab            &  downloader &         0.994 &      19\% \\
%mira                &        worm &         0.994 &      23\% \\
%elemental           &    grayware &         0.994 &       0\% \\
%guloader            &  downloader &         0.994 &       0\% \\
%memery              &       virus &         0.994 &       9\% \\
%macoute             &        worm &         0.994 &       0\% \\
%formbook            &     spyware &         0.994 &      37\% \\
%bundlore            &      adware &         0.994 &       2\% \\
%shyape              &  downloader &         0.994 &      39\% \\
%urelas              &    backdoor &         0.994 &      38\% \\
%wannacry            &  ransomware &         0.994 &       1\% \\
%stopcrypt           &  ransomware &         0.994 &       0\% \\
%betload             &    grayware &         0.994 &       3\% \\
%babonock            &        worm &         0.994 &       0\% \\
%apost               &  downloader &         0.994 &       1\% \\
%pincav              &    backdoor &         0.994 &      18\% \\
%cerber              &  ransomware &         0.994 &      16\% \\
%klez                &        worm &         0.994 &       1\% \\
%esaprof             &  downloader &         0.994 &      84\% \\
%dorv                &  downloader &         0.994 &       8\% \\
%mepaow              &       virus &         0.994 &      97\% \\
%esecn               &      adware &         0.994 &     100\% \\
%dalexis             &  downloader &         0.994 &       0\% \\
%ulise               &    grayware &         0.994 &       2\% \\
%bublik              &  downloader &         0.994 &      79\% \\
%cosmu               &       virus &         0.994 &       0\% \\
%daws                &  downloader &         0.994 &       2\% \\
%kuluoz              &  downloader &         0.994 &       4\% \\
%upatre              &  downloader &         0.994 &       4\% \\
%shodi               &       virus &         0.994 &       0\% \\
%blackhole           &    backdoor &         0.994 &      32\% \\
%pidgeon             &       virus &         0.994 &      16\% \\
%renos               &  downloader &         0.994 &      17\% \\
%speedcat            &    grayware &         0.994 &       0\% \\
%cutwail             &  downloader &         0.994 &      10\% \\
%winactivator        &        tool &         0.994 &       6\% \\
%simda               &    backdoor &         0.994 &      11\% \\
%ngrbot              &    backdoor &         0.994 &       0\% \\
%vybab               &        worm &         0.994 &       0\% \\
%necurs              &  downloader &         0.994 &       8\% \\
%garrun              &    grayware &         0.994 &       0\% \\
%bebloh              &    backdoor &         0.994 &       1\% \\
%coroxy              &    backdoor &         1.000 &       0\% \\
%lassorm             &        worm &         1.000 &       0\% \\
%gofot               &  downloader &         1.000 &      88\% \\
%kovter              &    grayware &         1.000 &       0\% \\
%goabeny             &    grayware &         1.000 &      75\% \\
%krol                &        worm &         1.000 &       0\% \\
%kronosbot           &    backdoor &         1.000 &       0\% \\
%laqma               &    grayware &         1.000 &      12\% \\
%gigex               &        worm &         1.000 &       0\% \\
%obit                &  downloader &         1.000 &       0\% \\
%gobot               &    backdoor &         1.000 &       4\% \\
%offend              &    grayware &         1.000 &      98\% \\
%doina               &    grayware &         1.000 &      50\% \\
%disttrack           &    grayware &         1.000 &       0\% \\
%dluca               &  downloader &         1.000 &      84\% \\
%icedid              &  downloader &         1.000 &       4\% \\
%refinka             &    grayware &         1.000 &       1\% \\
%dofoil              &  downloader &         1.000 &       6\% \\
%reconyc             &    grayware &         1.000 &      36\% \\
%recodrop            &  downloader &         1.000 &       0\% \\
%recex               &       miner &         1.000 &      11\% \\
%konus               &    backdoor &         1.000 &       0\% \\
%raccrypt            &  ransomware &         1.000 &       0\% \\
%qzonit              &     spyware &         1.000 &      87\% \\
%qshell              &    grayware &         1.000 &       0\% \\
%qqware              &    grayware &         1.000 &      50\% \\
%reptile             &    grayware &         1.000 &       0\% \\
%gify                &    grayware &         1.000 &       0\% \\
%houndhack           &    backdoor &         1.000 &     100\% \\
%lecna               &    backdoor &         1.000 &      24\% \\
%qqpass              &  downloader &         1.000 &      94\% \\
%lolbot              &        worm &         1.000 &       0\% \\
%locky               &  downloader &         1.000 &       5\% \\
%gator               &      adware &         1.000 &      47\% \\
%goldrv              &        worm &         1.000 &       0\% \\
%keydoor             &     spyware &         1.000 &       0\% \\
%griptolo            &        worm &         1.000 &       7\% \\
%kasidet             &    grayware &         1.000 &      19\% \\
%jpgiframe           &    grayware &         1.000 &       0\% \\
%johnnie             &    grayware &         1.000 &      65\% \\
%jimmy               &  ransomware &         1.000 &       0\% \\
%kolovorot           &    grayware &         1.000 &       3\% \\
%jevafus             &  downloader &         1.000 &      45\% \\
%havex               &    grayware &         1.000 &       0\% \\
%hebchengjiu         &      adware &         1.000 &       7\% \\
%hebogo              &    grayware &         1.000 &       0\% \\
%hider               &    grayware &         1.000 &      59\% \\
%inlog               &  downloader &         1.000 &       0\% \\
%injuke              &    grayware &         1.000 &      70\% \\
%itorrent            &    grayware &         1.000 &       0\% \\
%oberal              &  downloader &         1.000 &       0\% \\
%kolweb              &    grayware &         1.000 &      96\% \\
%koobface            &        worm &         1.000 &      77\% \\
%lmir                &       virus &         1.000 &       2\% \\
%geegly              &       virus &         1.000 &     100\% \\
%lipler              &  downloader &         1.000 &       0\% \\
%gepys               &  downloader &         1.000 &       0\% \\
%lebreat             &    grayware &         1.000 &     100\% \\
%rifdoor             &    backdoor &         1.000 &       0\% \\
%privateexeprotector &    grayware &         1.000 &      19\% \\
%dinwod              &  downloader &         1.000 &      98\% \\
%eyestye             &  downloader &         1.000 &      27\% \\
%eyoorun             &    grayware &         1.000 &       0\% \\
%ezsoftwareupdater   &    grayware &         1.000 &       0\% \\
%facido              &  downloader &         1.000 &       0\% \\
%fakedoc             &        worm &         1.000 &       0\% \\
%offercore           &    grayware &         1.000 &       0\% \\
%pahooka             &        worm &         1.000 &     100\% \\
%fakens              &      adware &         1.000 &       0\% \\
%drstwex             &  downloader &         1.000 &       0\% \\
%plemood             &        worm &         1.000 &       0\% \\
%protux              &    backdoor &         1.000 &       4\% \\
%dostre              &  downloader &         1.000 &       0\% \\
%pacex               &       miner &         1.000 &       0\% \\
%multiplier          &    grayware &         1.000 &       0\% \\
%downloadguide       &    grayware &         1.000 &       0\% \\
%prepscram           &    grayware &         1.000 &     100\% \\
%powerspider         &    backdoor &         1.000 &       0\% \\
%pistolar            &  downloader &         1.000 &      76\% \\
%powerless           &  downloader &         1.000 &      10\% \\
%pondfull            &        worm &         1.000 &       5\% \\
%dpsk                &       miner &         1.000 &     100\% \\
%drolnux             &        worm &         1.000 &       0\% \\
%pochi               &        worm &         1.000 &       0\% \\
%pluto               &        worm &         1.000 &      34\% \\
%dropware            &      adware &         1.000 &       1\% \\
%plingky             &  downloader &         1.000 &      93\% \\
%downer              &    grayware &         1.000 &      96\% \\
%pajetbin            &        worm &         1.000 &      91\% \\
%picsys              &        worm &         1.000 &     100\% \\
%enosch              &        worm &         1.000 &       0\% \\
%digs                &       miner &         1.000 &       0\% \\
%shiz                &    backdoor &         1.000 &       0\% \\
%shipup              &  downloader &         1.000 &      30\% \\
%cyfin               &    grayware &         1.000 &       5\% \\
%dadobra             &  downloader &         1.000 &      63\% \\
%sfone               &        worm &         1.000 &      65\% \\
%seven               &  ransomware &         1.000 &       0\% \\
%seraph              &  downloader &         1.000 &       0\% \\
%qqhack              &        tool &         1.000 &      98\% \\
%scrarev             &    grayware &         1.000 &       5\% \\
%salgorea            &  downloader &         1.000 &       0\% \\
%dexel               &  downloader &         1.000 &       0\% \\
%rungbu              &        worm &         1.000 &      18\% \\
%rums                &  downloader &         1.000 &       0\% \\
%ruledor             &    backdoor &         1.000 &       0\% \\
%diamin              &      dialer &         1.000 &      80\% \\
%roxer               &    grayware &         1.000 &      97\% \\
%detroie             &       virus &         1.000 &       2\% \\
%dorkbot             &        worm &         1.000 &       7\% \\
%qaccel              &     clicker &         1.000 &       0\% \\
%pykspa              &        worm &         1.000 &       0\% \\
%phorpiex            &        worm &         1.000 &      12\% \\
%phishbank           &        worm &         1.000 &       0\% \\
%perion              &    grayware &         1.000 &       0\% \\
%pedex               &    backdoor &         1.000 &     100\% \\
%eggnog              &        worm &         1.000 &       0\% \\
%egroupdial          &    grayware &         1.000 &      87\% \\
%rikihaki            &        worm &         1.000 &       0\% \\
%miniduke            &    backdoor &         1.000 &       0\% \\
%bcryptinject        &  downloader &         1.000 &       0\% \\
%mocrt               &     spyware &         1.000 &      73\% \\
%connectwise         &        tool &         1.000 &       0\% \\
%amigo               &    grayware &         1.000 &       0\% \\
%yahlover            &        worm &         1.000 &      65\% \\
%xorist              &  downloader &         1.000 &      24\% \\
%socelars            &     spyware &         1.000 &       1\% \\
%socks               &        worm &         1.000 &      18\% \\
%xolxo               &        worm &         1.000 &      99\% \\
%allaple             &        worm &         1.000 &       0\% \\
%xihet               &  downloader &         1.000 &       8\% \\
%wacatac             &    grayware &         1.000 &      14\% \\
%wabot               &    backdoor &         1.000 &      19\% \\
%berbew              &    backdoor &         1.000 &       0\% \\
%skintrim            &      adware &         1.000 &       2\% \\
%upantix             &  downloader &         1.000 &     100\% \\
%syncopate           &    grayware &         1.000 &      20\% \\
%unruy               &  downloader &         1.000 &      13\% \\
%umbra               &  downloader &         1.000 &       0\% \\
%tupym               &        worm &         1.000 &       0\% \\
%sytro               &        worm &         1.000 &      45\% \\
%bunitu              &    grayware &         1.000 &       0\% \\
%broskod             &  downloader &         1.000 &       1\% \\
%taskloader          &      adware &         1.000 &       0\% \\
%blackshades         &        worm &         1.000 &       2\% \\
%tougle              &    grayware &         1.000 &       0\% \\
%brook               &  ransomware &         1.000 &       0\% \\
%tempedreve          &       virus &         1.000 &       0\% \\
%swjoy               &    grayware &         1.000 &       0\% \\
%aitinject           &    backdoor &         1.000 &       1\% \\
%xiaobaminer         &       miner &         1.000 &      74\% \\
%agentino            &  downloader &         1.000 &       0\% \\
%wsgame              &    grayware &         1.000 &      49\% \\
%woozlist            &    grayware &         1.000 &      90\% \\
%ascentive           &    grayware &         1.000 &       0\% \\
%chrop               &      adware &         1.000 &      63\% \\
%atcpa               &       virus &         1.000 &       0\% \\
%autog               &  downloader &         1.000 &       0\% \\
%windigo             &    grayware &         1.000 &       3\% \\
%wenper              &        worm &         1.000 &      42\% \\
%sohana              &  downloader &         1.000 &      18\% \\
%wecod               &     spyware &         1.000 &      94\% \\
%axespec             &    grayware &         1.000 &       2\% \\
%ceatrg              &  downloader &         1.000 &      66\% \\
%catalina            &    grayware &         1.000 &       0\% \\
%wavipeg             &    backdoor &         1.000 &       0\% \\
%cardspy             &     spyware &         1.000 &     100\% \\
%wakme               &  downloader &         1.000 &       0\% \\
%xanfpezes           &    grayware &         1.000 &     100\% \\
%xcnfe               &    grayware &         1.000 &       0\% \\
%blihan              &    backdoor &         1.000 &       0\% \\
%cambot              &        worm &         1.000 &       0\% \\
%adaebook            &    grayware &         1.000 &     100\% \\
%contenedor          &       virus &         1.000 &       0\% \\
%addlyrics           &      adware &         1.000 &       0\% \\
%adposhel            &    grayware &         1.000 &       0\% \\
%zepfod              &        worm &         1.000 &       0\% \\
%agentc              &    grayware &         1.000 &       0\% \\
%agentcrypt          &    grayware &         1.000 &       0\% \\
%brontok             &        worm &         1.000 &      95\% \\
%moarider            &        worm &         1.000 &      98\% \\
%tonmye              &    grayware &         1.000 &      84\% \\
%trymedia            &      adware &         1.000 &      73\% \\
%zygug               &    grayware &         1.000 &      52\% \\
%gandcrab            &  ransomware &         1.000 &       3\% \\
%lyposit             &  ransomware &         1.000 &       0\% \\
%lunastorm           &        worm &         1.000 &      97\% \\
%lunam               &        worm &         1.000 &      99\% \\
%gandcrypt           &  ransomware &         1.000 &       2\% \\
%ludbaruma           &        worm &         1.000 &       0\% \\
%loring              &        worm &         1.000 &     100\% \\
%lolojan             &    grayware &         1.000 &      95\% \\
%gamemodding         &    grayware &         1.000 &       6\% \\
%mewsspy             &    backdoor &         1.000 &       6\% \\
%mimail              &        worm &         1.000 &       0\% \\
%maener              &       miner &         1.000 &       0\% \\
%mimdau              &  downloader &         1.000 &     100\% \\
%nevereg             &        worm &         1.000 &      51\% \\
%netstream           &    grayware &         1.000 &       0\% \\
%filetour            &    grayware &         1.000 &       4\% \\
%neoreklami          &      adware &         1.000 &       0\% \\
%neojit              &  downloader &         1.000 &       0\% \\
%finfish             &    backdoor &         1.000 &       0\% \\
%lollipop            &      adware &         1.000 &       0\% \\
%mydoom              &        worm &         1.000 &      83\% \\
%multibar            &    grayware &         1.000 &      23\% \\
%mulinex             &  downloader &         1.000 &      65\% \\
%mooqkel             &  downloader &         1.000 &     100\% \\
%moonlight           &        worm &         1.000 &       8\% \\
%fasong              &        worm &         1.000 &      78\% \\
%mailru              &    grayware &         1.000 &       0\% \\
%manbat              &        worm &         1.000 &      44\% \\
%mapsgory            &  downloader &         1.000 &       0\% \\
%bobax               &        worm &         1.000 &       3\% \\
%burn                &    backdoor &         1.000 &       0\% \\
%stormattack         &  downloader &         1.000 &       0\% \\
%vundo               &        worm &         1.000 &      89\% \\
%vtflooder           &  downloader &         1.000 &      55\% \\
%bactera             &        worm &         1.000 &       0\% \\
%voltar              &     clicker &         1.000 &       0\% \\
%vobfus              &        worm &         1.000 &       0\% \\
%stampado            &  ransomware &         1.000 &      58\% \\
%balrok              &        worm &         1.000 &       0\% \\
%banload             &       miner &         1.000 &      49\% \\
%vawtrak             &    backdoor &         1.000 &       0\% \\
%bzub                &  downloader &         1.000 &       2\% \\
%downloadsponsor     &    grayware &         1.000 &      87\% \\
%stone               &       virus &         1.000 &      97\% \\
%virlock             &       virus &         1.000 &       0\% \\
%virfire             &        worm &         1.000 &       0\% \\
%virbox              &    grayware &         1.000 &       1\% \\
%beastdoor           &    backdoor &         1.000 &      71\% \\
%vbinder             &        tool &         1.000 &       1\% \\
%vbclone             &  downloader &         1.000 &       0\% \\
%stihat              &        worm &         1.000 &     100\% \\
%sivis               &       virus &         1.000 &      72\% \\
%idsohtu             &    grayware &         1.000 &       6\% \\
%simbot              &    backdoor &         1.000 &       1\% \\
%gametea             &  downloader &         1.000 &     100\% \\
%mbrlock             &  downloader &         1.000 &       2\% \\
%tofsee              &    backdoor &         1.000 &       9\% \\
%regrun              &  ransomware &         1.000 &     100\% \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_binary_classificationReport_dynamic.tex <==
\begin{table}[h]
\caption{Binary classification report with dynamic model.}
\label{tbl:binary_accuracy_dynamic}
\begin{tabular}{lrrrr}
\toprule
\textbf{Class} &  \textbf{Precision} &    \textbf{Recall} &  \textbf{F1-score}  \\
\midrule
Positive (Malware)  &   0.9886 &  0.9185 &  0.9522 \\
Negative (Benignware)   &   0.9327 &  0.9893 &  0.9599  \\
\hline
Overall   &   0.9587 &  0.9539 & 0.9562   \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_binary_classificationReport_static.tex <==
\begin{table}[h]
\caption{Binary classification report with static model.}
\label{tbl:binary_accuracy_static}
\begin{tabular}{lrrrr}
\toprule
\textbf{Group} &  \textbf{Precision} &    \textbf{Recall} &  \textbf{F1-score} &  \textbf{Accuracy} \\
\midrule
Goodware  &   0.9599 &  0.9644 &  0.9621 &  0.9644 \\
Malware   &   0.9556 &  0.9499 &  0.9528 &  0.9499 \\
\hline
Overall   &   0.9639 &  0.9501 &   &   \\
\bottomrule
\end{tabular}
\end{table}



==> tbl/tbl_binary_confusionMatrix.tex <==
\noindent
\begin{table}[h]
	\begin{small}
	\setlength\tabcolsep{0pt}
	\caption{Confusion matrix for binary classification}
	\label{sec:static-tbl:binaryCM}
		\begin{tabular}{c >{\hspace{0.6em}}r @{\hspace{0.6em}}c @{\hspace{0.4em}}l @{\hspace{0.7em}}l}
			\multirow{11}{*}{\rotatebox{90}{\parbox{2.0cm}{\bfseries\centering
			Actual value}}} & & &\\
			& Goodware & Malware & \\[0.3em]
			&  \cmBox{0.9644} & \cmBox{0.0356} & Goodware \\[2.0em]
			&  \cmBox{0.0499} & \cmBox{0.9501} & Malware \\[2.0em]
			&  \multicolumn{2}{c}{\bfseries Predicted value} & \\
		\end{tabular}
	\end{small}
\end{table}


==> tbl/tbl_binary_featImportance.tex <==
\begin{table}[h]
\centering
\caption{Feature importance for binary classification.}
%Feature importance is measured using an average MDI score in range [0,100] 
%with higher being more important.}
\label{tbl:binary_FeatImportance}
\begin{tabular}{lrrr}
\toprule
%\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Importance}} \\
\textbf{Feature Class} &  \textbf{Combined} & \textbf{Static} & \textbf{Dynamic} \\
\midrule
s-bytegrams      &  40.88 & 51.38 &     - \\
d-registry       &  17.19 &     - & 25.00 \\
s-opcodegrams    &  13.44 & 21.08 &     - \\
s-strings        &   9.09 & 15.27 &     - \\
d-file           &   7.74 &     - & 29.70 \\
s-sections       &   3.05 &  6.73 &     - \\
s-imports        &   2.48 &  4.17 &     - \\
d-thread         &   2.06 &     - &  7.34 \\
d-network        &   1.51 &     - &  3.50 \\
d-process        &   1.47 &     - & 32.90 \\
s-headers        &   0.34 &  0.72 &     - \\
d-mutex          &   0.25 &     - &  0.16 \\
d-service        &   0.19 &     - &  1.40 \\
s-dll            &   0.17 &  0.28 &     - \\
s-file           &   0.13 &  0.35 &     - \\
\bottomrule
\end{tabular}
\end{table}



==> tbl/tbl_binary_featImportance_combined.tex <==
\begin{table}[h]
\centering
\caption{Importance of each feature class in the binary detection combined model.}
\label{tbl:binary_combined_FeatImportance}
\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Importance} \\
\midrule
s-bytegrams      &  40.88 \\
d-registry       &  17.19 \\
s-opcodegrams    &  13.44 \\
s-strings        &   9.09 \\
d-file           &   7.74 \\
s-sections       &   3.05 \\
s-imports        &   2.48 \\
d-thread         &   2.06 \\
d-network        &   1.51 \\
d-process        &   1.47 \\
s-headers        &   0.34 \\
d-mutex          &   0.25 \\
d-service        &   0.19 \\
s-dll            &   0.17 \\
s-file           &   0.13 \\
\bottomrule
\end{tabular}
\end{table}



==> tbl/tbl_binary_featImportance_dynamic.tex <==
\begin{table}[h]
\centering
\caption{Importance of each feature class in the binary detection dynamic model.}
\label{tbl:binary_FeatImportance_dynamic}
\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Importance} \\
\midrule
d-process   &  32.90 \\
d-file      &  29.70 \\
d-registry  &  25.00 \\
d-thread    &   7.34 \\
d-network   &   3.50 \\
d-service   &   1.40 \\
d-mutex     &   0.16 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_binary_featImportance_static.tex <==
\begin{table}[h]
\centering
\caption{Importance of each feature class in the binary detection static model.}
\label{tbl:binary_FeatImportance}
\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Importance} \\
\midrule
s-bytegrams   &         51.38 \\
s-opcodegrams &         21.08 \\
s-strings     &         15.27 \\
s-sections    &          6.73 \\
s-imports     &          4.17 \\
s-headers     &          0.72 \\
s-file        &          0.35 \\
s-dll         &          0.28 \\
\bottomrule
\end{tabular}
\end{table}



==> tbl/tbl_binary_no_packed_featImportance_static.tex <==
\begin{table}[h]
\centering
\caption{Feature importance for binary classification when excluding packed files.}
\label{tbl:binary_no_packed_static_featImportance}
	\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Static} \\
\midrule
s-bytegrams      & 49.30 \\
s-opcodegrams    & 22.69  \\
s-strings        & 16.16 \\
s-sections       & 6.29   \\
s-imports        & 4.35   \\
s-headers        & 0.63   \\
s-file           & 0.36   \\
s-dll            & 0.21   \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_binary_packedOnly_featImportance_static.tex <==
\begin{table}[h]
\centering
\caption{Feature importance for binary classification when only considering packed files.}
\label{tbl:binary_packed_only_static_featImportance}
	\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Static} \\
\midrule
s-bytegrams      & 62.22 \\
s-strings        & 16.80 \\
s-opcodegrams    & 8.30  \\
s-sections       & 7.50  \\
s-imports        & 2.29  \\
s-headers        & 1.42  \\
s-dll            & 1.06  \\
s-file           & 0.40  \\
\bottomrule
\end{tabular}
\end{table}



==> tbl/tbl_multiclass_bestAndWorst_combined.tex <==
\begin{table}[h]
\centering
\small
\caption{Top-10 families with the lowest family classification accuracy 
(i.e., highest mispredictions to other families)}
\label{tbl:multiclass_combined_bestAndWorst}
\begin{tabular}{llrr}
\toprule
\multicolumn{4}{c}{\textbf{Combined family classification}}\\
\textbf{Family} & \textbf{Class} &  \textbf{Avg F1} & \textbf{\% packed} \\
\midrule
zpevdo              &    grayware &         0.031 &      15\% \\
sdbot               &    backdoor &         0.160 &      92\% \\
alman               &       virus &         0.175 &      11\% \\
dumpex              &    grayware &         0.259 &      40\% \\
vitro               &       virus &         0.267 &       3\% \\
uwamson             &    grayware &         0.275 &      15\% \\
copidmbe            &       virus &         0.312 &       9\% \\
fugrafa             &    grayware &         0.314 &       8\% \\
sality              &       virus &         0.326 &       4\% \\
refroso             &    backdoor &         0.350 &      41\% \\
%bulz                &    grayware &         0.364 &      15 \\
%bifrose             &    backdoor &         0.376 &      33 \\
%spybot              &        worm &         0.400 &      15 \\
%ldpinch             &        worm &         0.400 &      47 \\
%tenga               &       virus &         0.412 &       6 \\
%pioneer             &       virus &         0.424 &       6 \\
%vbinder             &        tool &         0.430 &       1 \\
%wsgame              &    grayware &         0.432 &      49 \\
%pasta               &    grayware &         0.432 &      28 \\
%cobra               &    grayware &         0.442 &      60 \\
%gendal              &    grayware &         0.442 &      62 \\
%presenoker          &    grayware &         0.446 &      16 \\
%bancos              &     spyware &         0.447 &      44 \\
%poison              &    backdoor &         0.456 &      24 \\
%coins               &    grayware &         0.463 &      18 \\
%bestafera           &    grayware &         0.467 &      57 \\
%parite              &       virus &         0.471 &       7 \\
%sdum                &    grayware &         0.473 &      24 \\
%shutdowner          &    grayware &         0.475 &       6 \\
%llac                &        worm &         0.478 &      30 \\
%atraps              &    grayware &         0.484 &      20 \\
%geral               &  downloader &         0.486 &      23 \\
%menti               &        worm &         0.488 &      11 \\
%klone               &  downloader &         0.500 &      70 \\
%diztakun            &    grayware &         0.518 &      27 \\
%cerber              &  ransomware &         0.525 &      16 \\
%buzy                &        worm &         0.533 &      35 \\
%alien               &  downloader &         0.540 &      20 \\
%kiser               &    grayware &         0.547 &      55 \\
%neconyd             &     clicker &         0.560 &       0 \\
%pcclient            &    backdoor &         0.565 &      30 \\
%bredolab            &  downloader &         0.567 &      19 \\
%tibia               &    grayware &         0.568 &      31 \\
%noon                &     spyware &         0.570 &      19 \\
%dynamer             &  downloader &         0.576 &      20 \\
%emogen              &  downloader &         0.579 &      31 \\
%siscos              &  downloader &         0.588 &      48 \\
%ekstak              &    grayware &         0.589 &      31 \\
%speedingupmypc      &    grayware &         0.600 &      11 \\
%lethic              &  downloader &         0.611 &       1 \\
%ramnit              &       virus &         0.611 &      50 \\
%carberp             &  downloader &         0.612 &       6 \\
%diskwriter          &    grayware &         0.612 &      29 \\
%tdss                &  downloader &         0.613 &       6 \\
%dorgam              &  downloader &         0.613 &      19 \\
%virut               &       virus &         0.621 &       3 \\
%flystudio           &    grayware &         0.621 &      34 \\
%occamy              &    grayware &         0.624 &      26 \\
%midie               &    grayware &         0.625 &      33 \\
%convagent           &    grayware &         0.630 &      23 \\
%jacard              &    grayware &         0.632 &      34 \\
%kasidet             &    grayware &         0.632 &      19 \\
%bingoml             &    grayware &         0.632 &      22 \\
%farfli              &    backdoor &         0.633 &      38 \\
%gimemo              &  ransomware &         0.635 &      54 \\
%kraddare            &      adware &         0.638 &      36 \\
%zegost              &    backdoor &         0.638 &      28 \\
%vemply              &    grayware &         0.640 &      61 \\
%locky               &  downloader &         0.640 &       5 \\
%constructor         &    grayware &         0.643 &      13 \\
%quasar              &    backdoor &         0.644 &      48 \\
%fraudpack           &   rogueware &         0.644 &       3 \\
%scarsi              &  downloader &         0.650 &       8 \\
%predator            &    grayware &         0.653 &      13 \\
%injuke              &    grayware &         0.653 &      70 \\
%ruskill             &    backdoor &         0.653 &       7 \\
%mucc                &    grayware &         0.660 &       0 \\
%zard                &    grayware &         0.662 &       3 \\
%slugin              &       virus &         0.663 &       4 \\
%macri               &    backdoor &         0.663 &      58 \\
%oficla              &    backdoor &         0.667 &      36 \\
%tnega               &  downloader &         0.667 &      33 \\
%dorkbot             &        worm &         0.667 &       7 \\
%sabsik              &    grayware &         0.671 &      30 \\
%induc               &       virus &         0.671 &      56 \\
%titirez             &    grayware &         0.671 &       5 \\
%netwiredrc          &    backdoor &         0.674 &      24 \\
%mudrop              &  downloader &         0.674 &      37 \\
%clipbanker          &    grayware &         0.674 &      11 \\
%fraudrop            &  downloader &         0.680 &      31 \\
%emotet              &  downloader &         0.682 &       1 \\
%winwebsec           &   rogueware &         0.682 &      21 \\
%rbot                &        worm &         0.683 &      19 \\
%cridex              &    grayware &         0.684 &      15 \\
%jaik                &    grayware &         0.684 &       5 \\
%babar               &    grayware &         0.693 &       5 \\
%cossta              &    grayware &         0.695 &      13 \\
%hupigon             &    backdoor &         0.695 &      59 \\
%prorat              &    backdoor &         0.700 &      69 \\
%duote               &      adware &         0.700 &      98 \\
%expiro              &       virus &         0.705 &      10 \\
%ursnif              &       virus &         0.705 &      25 \\
%ymacco              &    grayware &         0.705 &      68 \\
%brresmon            &    grayware &         0.709 &       1 \\
%onlinegames         &    grayware &         0.710 &      14 \\
%waldek              &    grayware &         0.710 &       0 \\
%usteal              &    grayware &         0.710 &      31 \\
%cerbu               &    grayware &         0.712 &       4 \\
%nanocore            &    backdoor &         0.716 &      22 \\
%wacatac             &    grayware &         0.716 &      14 \\
%nymaim              &    backdoor &         0.716 &       1 \\
%wlksm               &       virus &         0.718 &       1 \\
%pornoblocker        &  ransomware &         0.722 &      14 \\
%polypatch           &    grayware &         0.722 &      99 \\
%citeary             &        worm &         0.723 &      16 \\
%sillyfdc            &        worm &         0.725 &      55 \\
%rozena              &    backdoor &         0.725 &       3 \\
%gamarue             &  downloader &         0.726 &      10 \\
%crysis              &  ransomware &         0.729 &      27 \\
%xtrat               &    backdoor &         0.729 &      58 \\
%stelega             &    grayware &         0.730 &      50 \\
%sysn                &  downloader &         0.730 &      19 \\
%zusy                &    grayware &         0.730 &       7 \\
%racealer            &    grayware &         0.733 &      32 \\
%kelihos             &    backdoor &         0.733 &      12 \\
%bebloh              &    backdoor &         0.733 &       1 \\
%ulise               &    grayware &         0.733 &       2 \\
%zurgop              &  downloader &         0.740 &       3 \\
%lotok               &    backdoor &         0.740 &      15 \\
%simda               &    backdoor &         0.741 &      11 \\
%stop                &  ransomware &         0.741 &       0 \\
%ursu                &    grayware &         0.743 &      23 \\
%buterat             &     clicker &         0.747 &      17 \\
%banbra              &    backdoor &         0.750 &      50 \\
%spyeye              &     spyware &         0.750 &       9 \\
%rebhip              &        worm &         0.750 &      16 \\
%spesr               &        worm &         0.750 &       0 \\
%zeroaccess          &  downloader &         0.756 &      10 \\
%garrun              &    grayware &         0.758 &       0 \\
%buzus               &  downloader &         0.758 &       3 \\
%deyma               &  downloader &         0.760 &      21 \\
%cryptinject         &  downloader &         0.760 &      34 \\
%bladabindi          &    backdoor &         0.765 &      19 \\
%zlob                &  downloader &         0.767 &      21 \\
%emotetu             &  downloader &         0.768 &       5 \\
%blackhole           &    backdoor &         0.768 &      32 \\
%killwin             &    grayware &         0.770 &      58 \\
%tibs                &  downloader &         0.773 &      29 \\
%elex                &      adware &         0.775 &       9 \\
%fareit              &    grayware &         0.778 &      14 \\
%gamevance           &      adware &         0.778 &       5 \\
%palevo              &    backdoor &         0.778 &      22 \\
%renos               &  downloader &         0.779 &      17 \\
%tonmye              &    grayware &         0.779 &      84 \\
%dadobra             &  downloader &         0.779 &      63 \\
%pincav              &    backdoor &         0.779 &      18 \\
%yoddos              &    backdoor &         0.779 &      19 \\
%bsymem              &    grayware &         0.780 &      25 \\
%dorifel             &  downloader &         0.780 &       5 \\
%xorist              &  downloader &         0.783 &      24 \\
%blamon              &    grayware &         0.789 &      33 \\
%orcus               &    backdoor &         0.790 &      42 \\
%qqware              &    grayware &         0.800 &      50 \\
%autinject           &        tool &         0.800 &       4 \\
%kuluoz              &  downloader &         0.800 &       4 \\
%startsurf           &    grayware &         0.800 &       3 \\
%asparnet            &    grayware &         0.800 &       5 \\
%kuaizip             &      adware &         0.800 &       1 \\
%ipamor              &    grayware &         0.800 &      39 \\
%dupzom              &  downloader &         0.800 &      14 \\
%mokes               &    backdoor &         0.800 &       1 \\
%burden              &      adware &         0.800 &       2 \\
%cutwail             &  downloader &         0.800 &      10 \\
%jatif               &    grayware &         0.800 &       2 \\
%gamini              &    grayware &         0.810 &       0 \\
%shopper             &    grayware &         0.811 &       1 \\
%fsysna              &        worm &         0.811 &      66 \\
%fujacks             &       virus &         0.811 &      35 \\
%ngrbot              &    backdoor &         0.811 &       0 \\
%vittalia            &    grayware &         0.811 &       3 \\
%iobit               &    grayware &         0.812 &      38 \\
%killmbr             &    grayware &         0.813 &       9 \\
%stopcrypt           &  ransomware &         0.814 &       0 \\
%vebzenpak           &    grayware &         0.820 &       0 \\
%doina               &    grayware &         0.820 &      50 \\
%staser              &  downloader &         0.821 &      61 \\
%nymeria             &    grayware &         0.821 &      32 \\
%deceptpcclean       &    grayware &         0.821 &       4 \\
%conduit             &    grayware &         0.821 &      35 \\
%utorrent            &    grayware &         0.821 &      72 \\
%passview            &    grayware &         0.821 &      35 \\
%gatak               &    grayware &         0.821 &      11 \\
%blackmoon           &    grayware &         0.827 &      74 \\
%dorv                &  downloader &         0.827 &       8 \\
%hacdef              &    backdoor &         0.829 &      21 \\
%dlhelper            &    grayware &         0.830 &      13 \\
%teslacrypt          &  ransomware &         0.832 &       1 \\
%windigo             &    grayware &         0.832 &       3 \\
%qbot                &  downloader &         0.832 &       0 \\
%remcos              &    backdoor &         0.832 &       4 \\
%agentb              &    grayware &         0.832 &      13 \\
%fakefire            &        worm &         0.833 &       3 \\
%skillis             &    grayware &         0.833 &      19 \\
%amonetize           &    grayware &         0.835 &       7 \\
%vbkryjetor          &  downloader &         0.840 &       4 \\
%lazy                &    grayware &         0.840 &       6 \\
%voltar              &     clicker &         0.840 &       0 \\
%tofsee              &    backdoor &         0.840 &       9 \\
%redcap              &  downloader &         0.840 &      18 \\
%avemaria            &     spyware &         0.842 &      12 \\
%glupteba            &    grayware &         0.842 &       1 \\
%xyligan             &    backdoor &         0.842 &      55 \\
%fragtor             &    grayware &         0.842 &      10 \\
%swizzor             &    grayware &         0.842 &       6 \\
%installmonster      &    grayware &         0.844 &      83 \\
%skintrim            &      adware &         0.847 &       2 \\
%strab               &  ransomware &         0.850 &      38 \\
%installcore         &    grayware &         0.850 &      10 \\
%spigot              &    grayware &         0.850 &      20 \\
%autoitinject        &    backdoor &         0.850 &      16 \\
%diss                &    grayware &         0.850 &       3 \\
%ficker              &    grayware &         0.850 &      15 \\
%balrok              &        worm &         0.850 &       0 \\
%dofoil              &  downloader &         0.853 &       6 \\
%trickster           &  downloader &         0.853 &       1 \\
%tiggre              &    grayware &         0.853 &      88 \\
%petya               &  ransomware &         0.853 &      16 \\
%bandit              &  downloader &         0.853 &      61 \\
%pterodo             &  downloader &         0.855 &       0 \\
%shade               &  ransomware &         0.856 &       5 \\
%lovgate             &        worm &         0.856 &      29 \\
%gandcrab            &  ransomware &         0.856 &       3 \\
%lollipop            &      adware &         0.857 &       0 \\
%brook               &  ransomware &         0.860 &       0 \\
%zapchast            &  downloader &         0.860 &       4 \\
%bunitu              &    grayware &         0.860 &       0 \\
%miancha             &  downloader &         0.860 &      11 \\
%tasker              &    grayware &         0.860 &      11 \\
%stihat              &        worm &         0.863 &     100 \\
%plugx               &    backdoor &         0.863 &       5 \\
%dalexis             &  downloader &         0.863 &       0 \\
%woozlist            &    grayware &         0.863 &      90 \\
%schoolboy           &    grayware &         0.863 &       7 \\
%cryptowall          &  ransomware &         0.863 &       2 \\
%kovter              &    grayware &         0.867 &       0 \\
%hpdefender          &    grayware &         0.870 &       0 \\
%manbat              &        worm &         0.870 &      44 \\
%cyfin               &    grayware &         0.870 &       5 \\
%yandex              &    grayware &         0.871 &       0 \\
%mytob               &        worm &         0.874 &      30 \\
%driverpack          &    grayware &         0.878 &      13 \\
%sodinokibi          &    grayware &         0.878 &       2 \\
%raccrypt            &  ransomware &         0.878 &       0 \\
%omaneat             &     spyware &         0.880 &       7 \\
%onescan             &    grayware &         0.880 &      38 \\
%vundo               &        worm &         0.880 &      89 \\
%malex               &  downloader &         0.880 &       1 \\
%wonton              &  downloader &         0.880 &       2 \\
%bandoo              &    grayware &         0.884 &       0 \\
%chifrax             &    grayware &         0.884 &      41 \\
%neutrinopos         &  ransomware &         0.884 &      12 \\
%gamania             &  downloader &         0.884 &       5 \\
%schoolgirl          &    grayware &         0.884 &       2 \\
%darkkomet           &    backdoor &         0.884 &      14 \\
%mabezat             &        worm &         0.888 &       0 \\
%johnnie             &    grayware &         0.889 &      65 \\
%binder              &  downloader &         0.889 &      16 \\
%multiplier          &    grayware &         0.890 &       0 \\
%reline              &     spyware &         0.890 &      57 \\
%bactera             &        worm &         0.890 &       0 \\
%turkojan            &    backdoor &         0.890 &      16 \\
%zbot                &  downloader &         0.890 &      24 \\
%bobax               &        worm &         0.890 &       3 \\
%guloader            &  downloader &         0.890 &       0 \\
%softcnapp           &      adware &         0.893 &       0 \\
%kolovorot           &    grayware &         0.895 &       3 \\
%zenlod              &  downloader &         0.895 &      22 \\
%azorult             &    grayware &         0.895 &      57 \\
%shylock             &    backdoor &         0.895 &       3 \\
%netstream           &    grayware &         0.900 &       0 \\
%subseven            &    backdoor &         0.900 &      69 \\
%techsnab            &    grayware &         0.900 &       2 \\
%istartsurf          &    grayware &         0.900 &       1 \\
%msposer             &  downloader &         0.900 &       4 \\
%jimmy               &  ransomware &         0.900 &       0 \\
%formbook            &     spyware &         0.900 &      37 \\
%opensupdater        &      adware &         0.900 &      14 \\
%lightstone          &    backdoor &         0.900 &      17 \\
%bitmin              &       miner &         0.900 &      25 \\
%lamer               &       virus &         0.900 &      43 \\
%ranumbot            &    grayware &         0.900 &      28 \\
%solmyr              &     spyware &         0.900 &      58 \\
%yahlover            &        worm &         0.905 &      65 \\
%mepaow              &       virus &         0.910 &      97 \\
%bezigate            &    backdoor &         0.910 &      15 \\
%urelas              &    backdoor &         0.910 &      38 \\
%speedbit            &    grayware &         0.910 &       8 \\
%cobaltstrike        &  downloader &         0.910 &       3 \\
%stampado            &  ransomware &         0.910 &      58 \\
%trickbot            &       miner &         0.910 &       0 \\
%opencandy           &    grayware &         0.910 &      92 \\
%agobot              &    backdoor &         0.911 &      32 \\
%beastdoor           &    backdoor &         0.911 &      71 \\
%chir                &        worm &         0.912 &      12 \\
%relevantknowledge   &      adware &         0.914 &       0 \\
%lockbit             &  ransomware &         0.916 &       0 \\
%esfury              &        worm &         0.916 &       5 \\
%khalesi             &    grayware &         0.920 &       2 \\
%scrop               &  downloader &         0.920 &      12 \\
%refinka             &    grayware &         0.920 &       1 \\
%blackie             &    grayware &         0.920 &       0 \\
%vawtrak             &    backdoor &         0.920 &       0 \\
%wajam               &      adware &         0.920 &       2 \\
%rostpay             &    grayware &         0.920 &      96 \\
%sohanad             &        worm &         0.920 &      66 \\
%webprefix           &  downloader &         0.922 &      12 \\
%mbrlock             &  downloader &         0.922 &       2 \\
%privateexeprotector &    grayware &         0.922 &      19 \\
%systweak            &    grayware &         0.923 &      19 \\
%growtopia           &    grayware &         0.925 &      69 \\
%gandcrypt           &  ransomware &         0.926 &       2 \\
%pirminay            &  downloader &         0.926 &       9 \\
%hotbar              &    grayware &         0.926 &      45 \\
%winwrapper          &    grayware &         0.926 &      44 \\
%xorer               &       virus &         0.926 &      11 \\
%taranis             &    grayware &         0.929 &       4 \\
%hematite            &       virus &         0.929 &       1 \\
%hider               &    grayware &         0.929 &      59 \\
%wapomi              &       virus &         0.929 &       8 \\
%shandaadd           &      adware &         0.929 &      88 \\
%mulinex             &  downloader &         0.930 &      65 \\
%schwarzesonne       &    backdoor &         0.930 &      48 \\
%winactivator        &        tool &         0.933 &       6 \\
%qjwmonkey           &    grayware &         0.933 &      47 \\
%ardamax             &    grayware &         0.933 &       1 \\
%nitol               &  downloader &         0.937 &       7 \\
%xiaobaminer         &       miner &         0.937 &      74 \\
%dodiw               &    backdoor &         0.940 &      83 \\
%disttrack           &    grayware &         0.940 &       0 \\
%speedcat            &    grayware &         0.940 &       0 \\
%bublik              &  downloader &         0.940 &      79 \\
%koobface            &        worm &         0.940 &      77 \\
%kuaiba              &      adware &         0.940 &       5 \\
%silentall           &    grayware &         0.940 &      77 \\
%explorerhijack      &  downloader &         0.940 &       1 \\
%auslogics           &    grayware &         0.941 &       3 \\
%installerex         &    grayware &         0.944 &       0 \\
%icedid              &  downloader &         0.947 &       4 \\
%sogou               &    grayware &         0.947 &      17 \\
%crossrider          &    grayware &         0.947 &       1 \\
%recex               &       miner &         0.950 &      11 \\
%seraph              &  downloader &         0.950 &       0 \\
%firseria            &    grayware &         0.950 &       8 \\
%adpack              &      adware &         0.950 &       2 \\
%snojan              &  downloader &         0.950 &       1 \\
%plingky             &  downloader &         0.950 &      93 \\
%upatre              &  downloader &         0.950 &       4 \\
%adgazelle           &    grayware &         0.950 &       0 \\
%necurs              &  downloader &         0.950 &       8 \\
%filefinder          &      adware &         0.950 &       3 \\
%scrarev             &    grayware &         0.950 &       5 \\
%wannacry            &  ransomware &         0.953 &       1 \\
%gozi                &     spyware &         0.958 &       1 \\
%gofot               &  downloader &         0.958 &      88 \\
%cjishu              &      adware &         0.958 &       1 \\
%klez                &        worm &         0.958 &       1 \\
%filetour            &    grayware &         0.958 &       4 \\
%socelars            &     spyware &         0.958 &       1 \\
%toptools            &    grayware &         0.958 &       0 \\
%browsefox           &    grayware &         0.958 &       6 \\
%fakefolder          &        worm &         0.958 &      71 \\
%multibar            &    grayware &         0.958 &      23 \\
%betload             &    grayware &         0.958 &       3 \\
%frosparf            &     clicker &         0.960 &      73 \\
%daws                &  downloader &         0.960 &       2 \\
%virbox              &    grayware &         0.960 &       1 \\
%vilsel              &  downloader &         0.960 &      41 \\
%miniduke            &    backdoor &         0.960 &       0 \\
%horst               &    backdoor &         0.960 &      30 \\
%eyestye             &  downloader &         0.960 &      27 \\
%arkeistealer        &    grayware &         0.960 &       6 \\
%tougle              &    grayware &         0.960 &       0 \\
%loadmoney           &    grayware &         0.960 &       8 \\
%agentc              &    grayware &         0.960 &       0 \\
%pcacceleratepro     &    grayware &         0.960 &       1 \\
%woool               &    grayware &         0.960 &      94 \\
%downloadsponsor     &    grayware &         0.960 &      87 \\
%shiz                &    backdoor &         0.960 &       0 \\
%veil                &    grayware &         0.960 &       1 \\
%wecod               &     spyware &         0.960 &      94 \\
%xanfpezes           &    grayware &         0.960 &     100 \\
%koutodoor           &    backdoor &         0.960 &      16 \\
%cheatengine         &    grayware &         0.964 &       0 \\
%fesber              &        worm &         0.964 &      33 \\
%winner              &    grayware &         0.967 &       0 \\
%imali               &      adware &         0.968 &       0 \\
%webdialer           &      dialer &         0.968 &      86 \\
%xolxo               &        worm &         0.968 &      99 \\
%webalta             &    grayware &         0.968 &       5 \\
%4shared             &    grayware &         0.968 &       1 \\
%lokibot             &    backdoor &         0.968 &      88 \\
%downloadadmin       &    grayware &         0.968 &       3 \\
%dealply             &    grayware &         0.968 &      19 \\
%detrahere           &    grayware &         0.968 &       4 \\
%paneidix            &    backdoor &         0.970 &       0 \\
%vrbrothers          &      adware &         0.970 &      88 \\
%swisyn              &        worm &         0.970 &       7 \\
%vobfus              &        worm &         0.970 &       0 \\
%cmy3u               &    grayware &         0.970 &      98 \\
%dropware            &      adware &         0.970 &       1 \\
%convertad           &      adware &         0.970 &       1 \\
%spyrix              &    grayware &         0.970 &      56 \\
%winloadsda          &    grayware &         0.970 &      86 \\
%smartpcsolutions    &    grayware &         0.970 &      46 \\
%tremp               &    grayware &         0.970 &       0 \\
%qzonit              &     spyware &         0.970 &      87 \\
%cosmu               &       virus &         0.970 &       0 \\
%sohana              &  downloader &         0.970 &      18 \\
%tupym               &        worm &         0.970 &       0 \\
%qihoo               &    grayware &         0.970 &       3 \\
%lmir                &       virus &         0.970 &       2 \\
%mocrt               &     spyware &         0.970 &      73 \\
%prepscram           &    grayware &         0.970 &     100 \\
%kolweb              &    grayware &         0.970 &      96 \\
%benjamin            &        worm &         0.970 &      94 \\
%regsup              &  downloader &         0.970 &       1 \\
%linkury             &    grayware &         0.971 &       0 \\
%pajetbin            &        worm &         0.971 &      91 \\
%bundlore            &      adware &         0.973 &       2 \\
%remoteutilities     &    grayware &         0.975 &      90 \\
%mywebsearch         &    grayware &         0.976 &       1 \\
%cycbot              &    backdoor &         0.976 &       0 \\
%screenmate          &    grayware &         0.976 &       1 \\
%kolab               &    grayware &         0.978 &       1 \\
%mint                &    grayware &         0.978 &       3 \\
%sillyp2p            &        worm &         0.979 &       1 \\
%wakme               &  downloader &         0.979 &       0 \\
%zygug               &    grayware &         0.979 &      52 \\
%tinba               &  downloader &         0.979 &      15 \\
%pidgeon             &       virus &         0.980 &      16 \\
%egroupdial          &    grayware &         0.980 &      87 \\
%shipup              &  downloader &         0.980 &      30 \\
%pistolar            &  downloader &         0.980 &      76 \\
%agentino            &  downloader &         0.980 &       0 \\
%neoreklami          &      adware &         0.980 &       0 \\
%simbot              &    backdoor &         0.980 &       1 \\
%phorpiex            &        worm &         0.980 &      12 \\
%gorillaprice        &      adware &         0.980 &       6 \\
%alyak               &  downloader &         0.980 &      55 \\
%seven               &  ransomware &         0.980 &       0 \\
%moarider            &        worm &         0.980 &      98 \\
%agentcrypt          &    grayware &         0.980 &       0 \\
%offend              &    grayware &         0.980 &      98 \\
%qshell              &    grayware &         0.980 &       0 \\
%offergenerator      &    grayware &         0.980 &       0 \\
%banload             &       miner &         0.980 &      49 \\
%bloored             &        worm &         0.980 &       0 \\
%bayrob              &     spyware &         0.980 &       1 \\
%dumpy               &        worm &         0.980 &       0 \\
%cardspy             &     spyware &         0.980 &     100 \\
%mediaget            &    grayware &         0.980 &      33 \\
%webcompanion        &    grayware &         0.980 &       0 \\
%idsohtu             &    grayware &         0.980 &       6 \\
%ceatrg              &  downloader &         0.980 &      66 \\
%gepys               &  downloader &         0.980 &       0 \\
%aauto               &    grayware &         0.980 &      56 \\
%reconyc             &    grayware &         0.980 &      36 \\
%sytro               &        worm &         0.980 &      45 \\
%allaple             &        worm &         0.987 &       0 \\
%ibryte              &      adware &         0.988 &       9 \\
%laqma               &    grayware &         0.988 &      12 \\
%unruy               &  downloader &         0.988 &      13 \\
%dexel               &  downloader &         0.989 &       0 \\
%macoute             &        worm &         0.989 &       0 \\
%fosniw              &  downloader &         0.989 &      42 \\
%jevafus             &  downloader &         0.989 &      45 \\
%axespec             &    grayware &         0.989 &       2 \\
%mira                &        worm &         0.989 &      23 \\
%fasong              &        worm &         0.989 &      78 \\
%antavmu             &        worm &         0.989 &       0 \\
%softpulse           &    grayware &         0.989 &      34 \\
%zvuzona             &    grayware &         0.989 &      79 \\
%virlock             &       virus &         0.989 &       0 \\
%lecna               &    backdoor &         0.989 &      24 \\
%installiq           &    grayware &         0.989 &       2 \\
%lipler              &  downloader &         0.989 &       0 \\
%pykspa              &        worm &         0.989 &       0 \\
%openinstall         &    grayware &         0.989 &      22 \\
%virfire             &        worm &         0.989 &       0 \\
%installbrain        &    grayware &         0.989 &       2 \\
%viking              &       virus &         0.989 &      98 \\
%reptile             &    grayware &         0.990 &       0 \\
%brontok             &        worm &         0.990 &      95 \\
%bcryptinject        &  downloader &         0.990 &       0 \\
%lydra               &     spyware &         0.990 &       5 \\
%aenjaris            &    grayware &         0.990 &       0 \\
%gify                &    grayware &         0.990 &       0 \\
%adaebook            &    grayware &         0.990 &     100 \\
%megasearch          &      adware &         0.990 &       0 \\
%lolbot              &        worm &         0.990 &       0 \\
%downloadassistant   &    grayware &         0.990 &      18 \\
%outbyte             &    grayware &         0.990 &       4 \\
%kronosbot           &    backdoor &         0.990 &       0 \\
%chrop               &      adware &         0.990 &      63 \\
%pacex               &       miner &         0.990 &       0 \\
%blackshades         &        worm &         0.990 &       2 \\
%mydoom              &        worm &         0.990 &      83 \\
%perion              &    grayware &         0.990 &       0 \\
%xcnfe               &    grayware &         0.990 &       0 \\
%dinwod              &  downloader &         0.990 &      98 \\
%plurox              &    backdoor &         0.990 &       0 \\
%connectwise         &        tool &         0.990 &       0 \\
%gator               &      adware &         0.990 &      47 \\
%hafen               &    grayware &         0.990 &       0 \\
%detroie             &       virus &         0.990 &       2 \\
%slimware            &    grayware &         0.990 &       0 \\
%dluca               &  downloader &         0.990 &      84 \\
%inbox               &    grayware &         0.990 &       0 \\
%hebchengjiu         &      adware &         0.990 &       7 \\
%vkontaktedj         &    grayware &         0.990 &       4 \\
%dstudio             &    grayware &         0.990 &       2 \\
%broskod             &  downloader &         0.990 &       1 \\
%anmalpro            &    grayware &         0.990 &       0 \\
%apost               &  downloader &         0.990 &       1 \\
%protux              &    backdoor &         0.990 &       4 \\
%gippers             &  ransomware &         0.990 &       0 \\
%autog               &  downloader &         0.990 &       0 \\
%pochi               &        worm &         1.000 &       0 \\
%drstwex             &  downloader &         1.000 &       0 \\
%ksdler              &      adware &         1.000 &      69 \\
%konus               &    backdoor &         1.000 &       0 \\
%getnow              &    grayware &         1.000 &      88 \\
%geegly              &       virus &         1.000 &     100 \\
%swjoy               &    grayware &         1.000 &       0 \\
%gamemodding         &    grayware &         1.000 &       6 \\
%syncopate           &    grayware &         1.000 &      20 \\
%finfish             &    backdoor &         1.000 &       0 \\
%fakens              &      adware &         1.000 &       0 \\
%fakedoc             &        worm &         1.000 &       0 \\
%mimdau              &  downloader &         1.000 &     100 \\
%stormattack         &  downloader &         1.000 &       0 \\
%qaccel              &     clicker &         1.000 &       0 \\
%pluto               &        worm &         1.000 &      34 \\
%moonlight           &        worm &         1.000 &       8 \\
%phishbank           &        worm &         1.000 &       0 \\
%picsys              &        worm &         1.000 &     100 \\
%obit                &  downloader &         1.000 &       0 \\
%oberal              &  downloader &         1.000 &       0 \\
%nevereg             &        worm &         1.000 &      51 \\
%plemood             &        worm &         1.000 &       0 \\
%primecasino         &    grayware &         1.000 &       0 \\
%neshta              &       virus &         1.000 &       2 \\
%gigex               &        worm &         1.000 &       0 \\
%neojit              &  downloader &         1.000 &       0 \\
%pondfull            &        worm &         1.000 &       5 \\
%powerless           &  downloader &         1.000 &      10 \\
%powerspider         &    backdoor &         1.000 &       0 \\
%mooqkel             &  downloader &         1.000 &     100 \\
%qqpass              &  downloader &         1.000 &      94 \\
%taskloader          &      adware &         1.000 &       0 \\
%tisandr             &        worm &         1.000 &       0 \\
%tempedreve          &       virus &         1.000 &       0 \\
%pedex               &    backdoor &         1.000 &     100 \\
%grenam              &       virus &         1.000 &       0 \\
%griptolo            &        worm &         1.000 &       7 \\
%soulclose           &        worm &         1.000 &       0 \\
%havex               &    grayware &         1.000 &       0 \\
%hebogo              &    grayware &         1.000 &       0 \\
%softonic            &      adware &         1.000 &      79 \\
%houndhack           &    backdoor &         1.000 &     100 \\
%socks               &        worm &         1.000 &      18 \\
%icloader            &    grayware &         1.000 &       2 \\
%sivis               &       virus &         1.000 &      72 \\
%gobot               &    backdoor &         1.000 &       4 \\
%sinau               &       virus &         1.000 &       0 \\
%itorrent            &    grayware &         1.000 &       0 \\
%jeefo               &       virus &         1.000 &      99 \\
%shyape              &  downloader &         1.000 &      39 \\
%jpgiframe           &    grayware &         1.000 &       0 \\
%eyoorun             &    grayware &         1.000 &       0 \\
%expressdownloader   &    grayware &         1.000 &      62 \\
%esecn               &      adware &         1.000 &     100 \\
%esaprof             &  downloader &         1.000 &      84 \\
%enosch              &        worm &         1.000 &       0 \\
%elemental           &    grayware &         1.000 &       0 \\
%ezsoftwareupdater   &    grayware &         1.000 &       0 \\
%facido              &  downloader &         1.000 &       0 \\
%goabeny             &    grayware &         1.000 &      75 \\
%goldrv              &        worm &         1.000 &       0 \\
%sfone               &        worm &         1.000 &      65 \\
%kingsoft            &    grayware &         1.000 &      37 \\
%shodi               &       virus &         1.000 &       0 \\
%keydoor             &     spyware &         1.000 &       0 \\
%krol                &        worm &         1.000 &       0 \\
%offercore           &    grayware &         1.000 &       0 \\
%inlog               &  downloader &         1.000 &       0 \\
%mimail              &        worm &         1.000 &       0 \\
%cambot              &        worm &         1.000 &       0 \\
%bzub                &  downloader &         1.000 &       2 \\
%burn                &    backdoor &         1.000 &       0 \\
%blihan              &    backdoor &         1.000 &       0 \\
%digs                &       miner &         1.000 &       0 \\
%berbew              &    backdoor &         1.000 &       0 \\
%babonock            &        worm &         1.000 &       0 \\
%xihet               &  downloader &         1.000 &       8 \\
%atcpa               &       virus &         1.000 &       0 \\
%ascentive           &    grayware &         1.000 &       0 \\
%amigo               &    grayware &         1.000 &       0 \\
%youxun              &    grayware &         1.000 &      11 \\
%aitinject           &    backdoor &         1.000 &       1 \\
%airinstaller        &    grayware &         1.000 &      87 \\
%zepfod              &        worm &         1.000 &       0 \\
%adposhel            &    grayware &         1.000 &       0 \\
%addlyrics           &      adware &         1.000 &       0 \\
%triusor             &       virus &         1.000 &       0 \\
%drolnux             &        worm &         1.000 &       0 \\
%dostre              &  downloader &         1.000 &       0 \\
%tufik               &       virus &         1.000 &       0 \\
%dpsk                &       miner &         1.000 &     100 \\
%umbra               &  downloader &         1.000 &       0 \\
%wavipeg             &    backdoor &         1.000 &       0 \\
%domaiq              &    grayware &         1.000 &      53 \\
%updane              &    grayware &         1.000 &       0 \\
%downer              &    grayware &         1.000 &      96 \\
%trymedia            &      adware &         1.000 &      73 \\
%downloadguide       &    grayware &         1.000 &       0 \\
%pahooka             &        worm &         1.000 &     100 \\
%vbclone             &  downloader &         1.000 &       0 \\
%upantix             &  downloader &         1.000 &     100 \\
%qqhack              &        tool &         1.000 &      98 \\
%clipspy             &    grayware &         1.000 &       2 \\
%vybab               &        worm &         1.000 &       0 \\
%lassorm             &        worm &         1.000 &       0 \\
%ludbaruma           &        worm &         1.000 &       0 \\
%salgorea            &  downloader &         1.000 &       0 \\
%rungbu              &        worm &         1.000 &      18 \\
%ruledor             &    backdoor &         1.000 &       0 \\
%lolojan             &    grayware &         1.000 &      95 \\
%roxer               &    grayware &         1.000 &      97 \\
%loring              &        worm &         1.000 &     100 \\
%rising              &    grayware &         1.000 &      34 \\
%rikihaki            &        worm &         1.000 &       0 \\
%rifdoor             &    backdoor &         1.000 &       0 \\
%lulusoftware        &    grayware &         1.000 &      13 \\
%mewsspy             &    backdoor &         1.000 &       6 \\
%lunam               &        worm &         1.000 &      99 \\
%lunastorm           &        worm &         1.000 &      97 \\
%regrun              &  ransomware &         1.000 &     100 \\
%lyposit             &  ransomware &         1.000 &       0 \\
%vtflooder           &  downloader &         1.000 &      55 \\
%contenedor          &       virus &         1.000 &       0 \\
%coroxy              &    backdoor &         1.000 &       0 \\
%cosmicduke          &    backdoor &         1.000 &       4 \\
%diamin              &      dialer &         1.000 &      80 \\
%wenper              &        worm &         1.000 &      42 \\
%wabot               &    backdoor &         1.000 &      19 \\
%catalina            &    grayware &         1.000 &       0 \\
%eggnog              &        worm &         1.000 &       0 \\
%memery              &       virus &         1.000 &       9 \\
%mapsgory            &  downloader &         1.000 &       0 \\
%mailru              &    grayware &         1.000 &       0 \\
%maener              &       miner &         1.000 &       0 \\
%recodrop            &  downloader &         1.000 &       0 \\
%gogo                &       virus &         1.000 &       0 \\
%zylom               &  downloader &         1.000 &       0 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_multiclass_bestAndWorst_dynamic.tex <==
\begin{table}[h]
\centering
\small
\caption{Top-10 families with the lowest family classification accuracy using
	dynamic features
(i.e., highest mispredictions to other families)}
\label{tbl:multiclass_dyn_bestAndWorst}
\begin{tabular}{llrrr}
\toprule
\multicolumn{5}{c}{\textbf{Dynamic family classification}}\\
\textbf{Family} & \textbf{Class} &  \textbf{Avg F1} & \textbf{\% packed} & \textbf{FMR} \\
\midrule
bancos      	&  spyware      &   0.0  	& 44\%	& 0.76	\\
kovter        	&  grayware     &   0.0 	& 0\%	& 0.78	\\
safebytes     	&  grayware     &   0.0 	& 99\%	& 0.80	\\
winner      	&  grayware     &   0.0 	& 0\%	& 0.80	\\
umbra         	&  downloader   &   0.0 	& 0\%	& 0.80	\\
ulise        	&  grayware     &   0.0 	& 2\%	& 0.80	\\
contenedor      &  virus    	&   0.0  	& 0\% 	& 0.80  \\
cobra     		&  grayware 	&   0.0 	& 60\% 	& 0.79	\\
kuaizip         &  adware   	&   0.0 	& 1\%	& 0.80	\\
zpevdo          &  grayware 	&   0.0 	& 15\%	& 0.77	\\	
\bottomrule
\end{tabular}
\end{table}



==> tbl/tbl_multiclass_bestAndWorst_static.tex <==
\begin{table}[h]
\centering
\small
\caption{Top-10 families with the lowest family classification accuracy using
	static features (i.e., highest mispredictions to other families)}
\label{tbl:multiclass_static_bestAndWorst}
\begin{tabular}{llrr}
\toprule
\multicolumn{4}{c}{\textbf{Static family classification}}\\
\textbf{Family} & \textbf{Class} &  \textbf{Avg F1} & \textbf{\% packed} \\
\midrule
zpevdo              &    grayware &         0.150 &      15\%  \\
vitro               &       virus &         0.240 &      3\% \\
uwamson             &    grayware &         0.252 &      15\%  \\
gendal              &    grayware &         0.280 &      62\%  \\
dumpex              &    grayware &         0.290 &      40\%  \\
alman               &       virus &         0.293 &      11\%  \\
sality              &       virus &         0.328 &      4\% \\
pasta               &    grayware &         0.346 &      28\%  \\
cobra               &    grayware &         0.381 &      60\%  \\
copidmbe            &       virus &         0.387 &      9\% \\
%refroso             &    backdoor &         0.393 &      41\%  \\
%llac                &        worm &         0.402 &      30\%  \\
%bifrose             &    backdoor &         0.402 &      33\%  \\
%atraps              &    grayware &         0.409 &      0.20 \\
%pioneer             &       virus &         0.419 &      0.06 \\
%coins               &    grayware &         0.435 &      0.18 \\
%bancos              &     spyware &         0.449 &      0.44 \\
%convagent           &    grayware &         0.451 &      0.23 \\
%kiser               &    grayware &         0.453 &      0.55 \\
%buzy                &        worm &         0.459 &      0.35 \\
%bestafera           &    grayware &         0.483 &      0.57 \\
%ldpinch             &        worm &         0.489 &      0.47 \\
%menti               &        worm &         0.490 &      0.11 \\
%midie               &    grayware &         0.491 &      0.33 \\
%alien               &  downloader &         0.493 &      0.20 \\
%occamy              &    grayware &         0.498 &      0.26 \\
%bulz                &    grayware &         0.504 &      0.15 \\
%wsgame              &    grayware &         0.509 &      0.49 \\
%sabsik              &    grayware &         0.514 &      0.30 \\
%diskwriter          &    grayware &         0.515 &      0.29 \\
%tibia               &    grayware &         0.522 &      0.31 \\
%oficla              &    backdoor &         0.523 &      0.36 \\
%klone               &  downloader &         0.528 &      0.70 \\
%sdum                &    grayware &         0.529 &      0.24 \\
%ramnit              &       virus &         0.532 &      0.50 \\
%presenoker          &    grayware &         0.540 &      0.16 \\
%ruskill             &    backdoor &         0.544 &      0.07 \\
%diztakun            &    grayware &         0.545 &      0.27 \\
%bredolab            &  downloader &         0.545 &      0.19 \\
%jatif               &    grayware &         0.558 &      0.02 \\
%jacard              &    grayware &         0.562 &      0.34 \\
%noon                &     spyware &         0.570 &      0.19 \\
%scarsi              &  downloader &         0.579 &      0.08 \\
%clipbanker          &    grayware &         0.580 &      0.11 \\
%poison              &    backdoor &         0.581 &      0.24 \\
%flystudio           &    grayware &         0.588 &      0.34 \\
%ulise               &    grayware &         0.591 &      0.02 \\
%pcclient            &    backdoor &         0.592 &      0.30 \\
%parite              &       virus &         0.594 &      0.07 \\
%dorkbot             &        worm &         0.595 &      0.07 \\
%gify                &    grayware &         0.597 &      0.00 \\
%kasidet             &    grayware &         0.598 &      0.19 \\
%emogen              &  downloader &         0.599 &      0.31 \\
%winwebsec           &   rogueware &         0.599 &      0.21 \\
%zard                &    grayware &         0.599 &      0.03 \\
%geral               &  downloader &         0.599 &      0.23 \\
%dynamer             &  downloader &         0.600 &      0.20 \\
%tdss                &  downloader &         0.606 &      0.06 \\
%lethic              &  downloader &         0.606 &      0.01 \\
%mucc                &    grayware &         0.607 &      0.00 \\
%fareit              &    grayware &         0.609 &      0.14 \\
%virut               &       virus &         0.609 &      0.03 \\
%gimemo              &  ransomware &         0.609 &      0.54 \\
%farfli              &    backdoor &         0.611 &      0.38 \\
%constructor         &    grayware &         0.614 &      0.13 \\
%mudrop              &  downloader &         0.617 &      0.37 \\
%netwiredrc          &    backdoor &         0.618 &      0.24 \\
%polypatch           &    grayware &         0.618 &      0.99 \\
%vemply              &    grayware &         0.619 &      0.61 \\
%cossta              &    grayware &         0.622 &      0.13 \\
%carberp             &  downloader &         0.624 &      0.06 \\
%usteal              &    grayware &         0.625 &      0.31 \\
%bingoml             &    grayware &         0.630 &      0.22 \\
%predator            &    grayware &         0.631 &      0.13 \\
%cridex              &    grayware &         0.632 &      0.15 \\
%ekstak              &    grayware &         0.633 &      0.31 \\
%rozena              &    backdoor &         0.634 &      0.03 \\
%fraudpack           &   rogueware &         0.634 &      0.03 \\
%buterat             &     clicker &         0.634 &      0.17 \\
%siscos              &  downloader &         0.637 &      0.48 \\
%crysis              &  ransomware &         0.638 &      0.27 \\
%palevo              &    backdoor &         0.638 &      0.22 \\
%ymacco              &    grayware &         0.643 &      0.68 \\
%emotet              &  downloader &         0.645 &      0.01 \\
%zlob                &  downloader &         0.647 &      0.21 \\
%quasar              &    backdoor &         0.650 &      0.48 \\
%tenga               &       virus &         0.654 &      0.06 \\
%macri               &    backdoor &         0.654 &      0.58 \\
%simda               &    backdoor &         0.654 &      0.11 \\
%locky               &  downloader &         0.656 &      0.05 \\
%kraddare            &      adware &         0.660 &      0.36 \\
%babar               &    grayware &         0.665 &      0.05 \\
%induc               &       virus &         0.668 &      0.56 \\
%banbra              &    backdoor &         0.669 &      0.50 \\
%dorgam              &  downloader &         0.670 &      0.19 \\
%gamarue             &  downloader &         0.671 &      0.10 \\
%fraudrop            &  downloader &         0.671 &      0.31 \\
%zeroaccess          &  downloader &         0.671 &      0.10 \\
%lotok               &    backdoor &         0.672 &      0.15 \\
%blackhole           &    backdoor &         0.673 &      0.32 \\
%tnega               &  downloader &         0.676 &      0.33 \\
%rebhip              &        worm &         0.677 &      0.16 \\
%titirez             &    grayware &         0.677 &      0.05 \\
%vbinder             &        tool &         0.680 &      0.01 \\
%spyeye              &     spyware &         0.681 &      0.09 \\
%ursnif              &       virus &         0.682 &      0.25 \\
%nanocore            &    backdoor &         0.683 &      0.22 \\
%mokes               &    backdoor &         0.685 &      0.01 \\
%buzus               &  downloader &         0.686 &      0.03 \\
%hupigon             &    backdoor &         0.694 &      0.59 \\
%fugrafa             &    grayware &         0.695 &      0.08 \\
%sysn                &  downloader &         0.696 &      0.19 \\
%slugin              &       virus &         0.700 &      0.04 \\
%onlinegames         &    grayware &         0.704 &      0.14 \\
%cerbu               &    grayware &         0.707 &      0.04 \\
%expiro              &       virus &         0.708 &      0.10 \\
%vittalia            &    grayware &         0.708 &      0.03 \\
%yoddos              &    backdoor &         0.711 &      0.19 \\
%injuke              &    grayware &         0.712 &      0.70 \\
%ursu                &    grayware &         0.714 &      0.23 \\
%elex                &      adware &         0.715 &      0.09 \\
%rbot                &        worm &         0.716 &      0.19 \\
%deyma               &  downloader &         0.716 &      0.21 \\
%emotetu             &  downloader &         0.716 &      0.05 \\
%gamini              &    grayware &         0.716 &      0.00 \\
%pornoblocker        &  ransomware &         0.717 &      0.14 \\
%waldek              &    grayware &         0.717 &      0.00 \\
%racealer            &    grayware &         0.718 &      0.32 \\
%wacatac             &    grayware &         0.719 &      0.14 \\
%killmbr             &    grayware &         0.721 &      0.09 \\
%xtrat               &    backdoor &         0.727 &      0.58 \\
%neconyd             &     clicker &         0.727 &      0.00 \\
%brresmon            &    grayware &         0.729 &      0.01 \\
%qqware              &    grayware &         0.729 &      0.50 \\
%stopcrypt           &  ransomware &         0.730 &      0.00 \\
%zegost              &    backdoor &         0.730 &      0.28 \\
%autinject           &        tool &         0.730 &      0.04 \\
%tonmye              &    grayware &         0.731 &      0.84 \\
%startsurf           &    grayware &         0.732 &      0.03 \\
%schoolboy           &    grayware &         0.733 &      0.07 \\
%tasker              &    grayware &         0.733 &      0.11 \\
%bsymem              &    grayware &         0.736 &      0.25 \\
%wlksm               &       virus &         0.736 &      0.01 \\
%garrun              &    grayware &         0.741 &      0.00 \\
%gamevance           &      adware &         0.743 &      0.05 \\
%sillyfdc            &        worm &         0.746 &      0.55 \\
%zapchast            &  downloader &         0.746 &      0.04 \\
%kuluoz              &  downloader &         0.747 &      0.04 \\
%agentb              &    grayware &         0.747 &      0.13 \\
%ipamor              &    grayware &         0.748 &      0.39 \\
%blamon              &    grayware &         0.749 &      0.33 \\
%orcus               &    backdoor &         0.749 &      0.42 \\
%dorifel             &  downloader &         0.752 &      0.05 \\
%stop                &  ransomware &         0.754 &      0.00 \\
%wajam               &      adware &         0.754 &      0.02 \\
%fragtor             &    grayware &         0.756 &      0.10 \\
%fsysna              &        worm &         0.757 &      0.66 \\
%conduit             &    grayware &         0.759 &      0.35 \\
%kelihos             &    backdoor &         0.759 &      0.12 \\
%bandit              &  downloader &         0.760 &      0.61 \\
%cutwail             &  downloader &         0.761 &      0.10 \\
%bladabindi          &    backdoor &         0.762 &      0.19 \\
%dadobra             &  downloader &         0.764 &      0.63 \\
%speedingupmypc      &    grayware &         0.766 &      0.11 \\
%passview            &    grayware &         0.766 &      0.35 \\
%zurgop              &  downloader &         0.768 &      0.03 \\
%shopper             &    grayware &         0.768 &      0.01 \\
%pincav              &    backdoor &         0.769 &      0.18 \\
%glupteba            &    grayware &         0.770 &      0.01 \\
%ngrbot              &    backdoor &         0.770 &      0.00 \\
%stelega             &    grayware &         0.770 &      0.50 \\
%spesr               &        worm &         0.772 &      0.00 \\
%jaik                &    grayware &         0.772 &      0.05 \\
%voltar              &     clicker &         0.772 &      0.00 \\
%swizzor             &    grayware &         0.773 &      0.06 \\
%nymeria             &    grayware &         0.774 &      0.32 \\
%vebzenpak           &    grayware &         0.776 &      0.00 \\
%windigo             &    grayware &         0.776 &      0.03 \\
%cryptowall          &  ransomware &         0.776 &      0.02 \\
%shutdowner          &    grayware &         0.777 &      0.06 \\
%tibs                &  downloader &         0.777 &      0.29 \\
%dupzom              &  downloader &         0.777 &      0.14 \\
%blackmoon           &    grayware &         0.782 &      0.74 \\
%teslacrypt          &  ransomware &         0.782 &      0.01 \\
%amonetize           &    grayware &         0.783 &      0.07 \\
%lazy                &    grayware &         0.783 &      0.06 \\
%wonton              &  downloader &         0.785 &      0.02 \\
%cerber              &  ransomware &         0.786 &      0.16 \\
%woozlist            &    grayware &         0.786 &      0.90 \\
%renos               &  downloader &         0.787 &      0.17 \\
%spigot              &    grayware &         0.789 &      0.20 \\
%sdbot               &    backdoor &         0.795 &      0.92 \\
%asparnet            &    grayware &         0.796 &      0.05 \\
%vbkryjetor          &  downloader &         0.798 &      0.04 \\
%iobit               &    grayware &         0.799 &      0.38 \\
%bitmin              &       miner &         0.800 &      0.25 \\
%dofoil              &  downloader &         0.801 &      0.06 \\
%lightstone          &    backdoor &         0.802 &      0.17 \\
%killwin             &    grayware &         0.803 &      0.58 \\
%fujacks             &       virus &         0.803 &      0.35 \\
%petya               &  ransomware &         0.803 &      0.16 \\
%ascentive           &    grayware &         0.803 &      0.00 \\
%remcos              &    backdoor &         0.804 &      0.04 \\
%doina               &    grayware &         0.807 &      0.50 \\
%mint                &    grayware &         0.808 &      0.03 \\
%nymaim              &    backdoor &         0.809 &      0.01 \\
%chifrax             &    grayware &         0.809 &      0.41 \\
%citeary             &        worm &         0.809 &      0.16 \\
%mytob               &        worm &         0.810 &      0.30 \\
%softcnapp           &      adware &         0.814 &      0.00 \\
%zbot                &  downloader &         0.814 &      0.24 \\
%plugx               &    backdoor &         0.818 &      0.05 \\
%speedbit            &    grayware &         0.818 &      0.08 \\
%binder              &  downloader &         0.821 &      0.16 \\
%cryptinject         &  downloader &         0.822 &      0.34 \\
%multiplier          &    grayware &         0.823 &      0.00 \\
%gatak               &    grayware &         0.823 &      0.11 \\
%xyligan             &    backdoor &         0.824 &      0.55 \\
%azorult             &    grayware &         0.824 &      0.57 \\
%dorv                &  downloader &         0.825 &      0.08 \\
%skillis             &    grayware &         0.827 &      0.19 \\
%arkeistealer        &    grayware &         0.828 &      0.06 \\
%scrop               &  downloader &         0.828 &      0.12 \\
%hacdef              &    backdoor &         0.829 &      0.21 \\
%brook               &  ransomware &         0.830 &      0.00 \\
%redcap              &  downloader &         0.830 &      0.18 \\
%tofsee              &    backdoor &         0.830 &      0.09 \\
%qbot                &  downloader &         0.834 &      0.00 \\
%darkkomet           &    backdoor &         0.835 &      0.14 \\
%staser              &  downloader &         0.835 &      0.61 \\
%systweak            &    grayware &         0.838 &      0.19 \\
%zusy                &    grayware &         0.839 &      0.07 \\
%taranis             &    grayware &         0.839 &      0.04 \\
%cyfin               &    grayware &         0.839 &      0.05 \\
%balrok              &        worm &         0.841 &      0.00 \\
%guloader            &  downloader &         0.841 &      0.00 \\
%johnnie             &    grayware &         0.841 &      0.65 \\
%diss                &    grayware &         0.841 &      0.03 \\
%prorat              &    backdoor &         0.844 &      0.69 \\
%tiggre              &    grayware &         0.844 &      0.88 \\
%autoitinject        &    backdoor &         0.845 &      0.16 \\
%mabezat             &        worm &         0.845 &      0.00 \\
%schoolgirl          &    grayware &         0.845 &      0.02 \\
%avemaria            &     spyware &         0.845 &      0.12 \\
%trickster           &  downloader &         0.846 &      0.01 \\
%beastdoor           &    backdoor &         0.847 &      0.71 \\
%hematite            &       virus &         0.847 &      0.01 \\
%reline              &     spyware &         0.847 &      0.57 \\
%shade               &  ransomware &         0.848 &      0.05 \\
%deceptpcclean       &    grayware &         0.849 &      0.04 \\
%gandcrypt           &  ransomware &         0.850 &      0.02 \\
%zenlod              &  downloader &         0.850 &      0.22 \\
%spybot              &        worm &         0.851 &      0.15 \\
%xanfpezes           &    grayware &         0.853 &      1.00 \\
%yandex              &    grayware &         0.853 &      0.00 \\
%gandcrab            &  ransomware &         0.853 &      0.03 \\
%stampado            &  ransomware &         0.854 &      0.58 \\
%bactera             &        worm &         0.854 &      0.00 \\
%khalesi             &    grayware &         0.855 &      0.02 \\
%omaneat             &     spyware &         0.855 &      0.07 \\
%jimmy               &  ransomware &         0.855 &      0.00 \\
%raccrypt            &  ransomware &         0.857 &      0.00 \\
%dalexis             &  downloader &         0.858 &      0.00 \\
%xorist              &  downloader &         0.858 &      0.24 \\
%webprefix           &  downloader &         0.858 &      0.12 \\
%installcore         &    grayware &         0.859 &      0.10 \\
%driverpack          &    grayware &         0.860 &      0.13 \\
%trickbot            &       miner &         0.861 &      0.00 \\
%sodinokibi          &    grayware &         0.863 &      0.02 \\
%manbat              &        worm &         0.864 &      0.44 \\
%utorrent            &    grayware &         0.866 &      0.72 \\
%offend              &    grayware &         0.866 &      0.98 \\
%burden              &      adware &         0.868 &      0.02 \\
%skintrim            &      adware &         0.871 &      0.02 \\
%lokibot             &    backdoor &         0.871 &      0.88 \\
%esfury              &        worm &         0.871 &      0.05 \\
%neutrinopos         &  ransomware &         0.872 &      0.12 \\
%recex               &       miner &         0.873 &      0.11 \\
%onescan             &    grayware &         0.873 &      0.38 \\
%hotbar              &    grayware &         0.877 &      0.45 \\
%smartpcsolutions    &    grayware &         0.878 &      0.46 \\
%solmyr              &     spyware &         0.878 &      0.58 \\
%shylock             &    backdoor &         0.879 &      0.03 \\
%subseven            &    backdoor &         0.880 &      0.69 \\
%bunitu              &    grayware &         0.881 &      0.00 \\
%lovgate             &        worm &         0.883 &      0.29 \\
%ficker              &    grayware &         0.884 &      0.15 \\
%turkojan            &    backdoor &         0.884 &      0.16 \\
%yahlover            &        worm &         0.884 &      0.65 \\
%mulinex             &  downloader &         0.885 &      0.65 \\
%crossrider          &    grayware &         0.885 &      0.01 \\
%stihat              &        worm &         0.886 &      1.00 \\
%sogou               &    grayware &         0.886 &      0.17 \\
%bezigate            &    backdoor &         0.888 &      0.15 \\
%opensupdater        &      adware &         0.889 &      0.14 \\
%strab               &  ransomware &         0.889 &      0.38 \\
%istartsurf          &    grayware &         0.890 &      0.01 \\
%xorer               &       virus &         0.890 &      0.11 \\
%dlhelper            &    grayware &         0.892 &      0.13 \\
%nitol               &  downloader &         0.892 &      0.07 \\
%pterodo             &  downloader &         0.893 &      0.00 \\
%mepaow              &       virus &         0.895 &      0.97 \\
%xiaobaminer         &       miner &         0.896 &      0.74 \\
%winwrapper          &    grayware &         0.896 &      0.44 \\
%necurs              &  downloader &         0.897 &      0.08 \\
%privateexeprotector &    grayware &         0.897 &      0.19 \\
%techsnab            &    grayware &         0.898 &      0.02 \\
%mbrlock             &  downloader &         0.901 &      0.02 \\
%hpdefender          &    grayware &         0.901 &      0.00 \\
%vawtrak             &    backdoor &         0.902 &      0.00 \\
%lockbit             &  ransomware &         0.902 &      0.00 \\
%miancha             &  downloader &         0.903 &      0.11 \\
%convertad           &      adware &         0.904 &      0.01 \\
%mywebsearch         &    grayware &         0.905 &      0.01 \\
%ardamax             &    grayware &         0.906 &      0.01 \\
%bobax               &        worm &         0.906 &      0.03 \\
%agobot              &    backdoor &         0.908 &      0.32 \\
%filefinder          &      adware &         0.909 &      0.03 \\
%gamania             &  downloader &         0.910 &      0.05 \\
%lamer               &       virus &         0.910 &      0.43 \\
%woool               &    grayware &         0.910 &      0.94 \\
%bebloh              &    backdoor &         0.911 &      0.01 \\
%pirminay            &  downloader &         0.911 &      0.09 \\
%bandoo              &    grayware &         0.911 &      0.00 \\
%relevantknowledge   &      adware &         0.912 &      0.00 \\
%cobaltstrike        &  downloader &         0.912 &      0.03 \\
%klez                &        worm &         0.913 &      0.01 \\
%kolovorot           &    grayware &         0.913 &      0.03 \\
%schwarzesonne       &    backdoor &         0.914 &      0.48 \\
%kovter              &    grayware &         0.915 &      0.00 \\
%sohanad             &        worm &         0.915 &      0.66 \\
%shandaadd           &      adware &         0.916 &      0.88 \\
%ranumbot            &    grayware &         0.917 &      0.28 \\
%dealply             &    grayware &         0.917 &      0.19 \\
%loadmoney           &    grayware &         0.918 &      0.08 \\
%linkury             &    grayware &         0.919 &      0.00 \\
%netstream           &    grayware &         0.920 &      0.00 \\
%hider               &    grayware &         0.921 &      0.59 \\
%koobface            &        worm &         0.921 &      0.77 \\
%lollipop            &      adware &         0.923 &      0.00 \\
%vilsel              &  downloader &         0.923 &      0.41 \\
%pidgeon             &       virus &         0.924 &      0.16 \\
%blackie             &    grayware &         0.924 &      0.00 \\
%icedid              &  downloader &         0.924 &      0.04 \\
%malex               &  downloader &         0.924 &      0.01 \\
%msposer             &  downloader &         0.925 &      0.04 \\
%scrarev             &    grayware &         0.925 &      0.05 \\
%fakefolder          &        worm &         0.926 &      0.71 \\
%toptools            &    grayware &         0.928 &      0.00 \\
%gozi                &     spyware &         0.928 &      0.01 \\
%cycbot              &    backdoor &         0.929 &      0.00 \\
%benjamin            &        worm &         0.931 &      0.94 \\
%browsefox           &    grayware &         0.931 &      0.06 \\
%eyestye             &  downloader &         0.933 &      0.27 \\
%urelas              &    backdoor &         0.933 &      0.38 \\
%fosniw              &  downloader &         0.934 &      0.42 \\
%auslogics           &    grayware &         0.934 &      0.03 \\
%agentc              &    grayware &         0.934 &      0.00 \\
%virbox              &    grayware &         0.936 &      0.01 \\
%upatre              &  downloader &         0.937 &      0.04 \\
%fakefire            &        worm &         0.938 &      0.03 \\
%opencandy           &    grayware &         0.938 &      0.92 \\
%adpack              &      adware &         0.939 &      0.02 \\
%pcacceleratepro     &    grayware &         0.939 &      0.01 \\
%aitinject           &    backdoor &         0.939 &      0.01 \\
%dodiw               &    backdoor &         0.940 &      0.83 \\
%remoteutilities     &    grayware &         0.941 &      0.90 \\
%horst               &    backdoor &         0.942 &      0.30 \\
%adgazelle           &    grayware &         0.942 &      0.00 \\
%silentall           &    grayware &         0.942 &      0.77 \\
%seraph              &  downloader &         0.942 &      0.00 \\
%refinka             &    grayware &         0.942 &      0.01 \\
%softpulse           &    grayware &         0.943 &      0.34 \\
%neoreklami          &      adware &         0.943 &      0.00 \\
%formbook            &     spyware &         0.943 &      0.37 \\
%imali               &      adware &         0.944 &      0.00 \\
%winactivator        &        tool &         0.944 &      0.06 \\
%qzonit              &     spyware &         0.944 &      0.87 \\
%explorerhijack      &  downloader &         0.944 &      0.01 \\
%multibar            &    grayware &         0.947 &      0.23 \\
%perion              &    grayware &         0.947 &      0.00 \\
%qshell              &    grayware &         0.949 &      0.00 \\
%tremp               &    grayware &         0.949 &      0.00 \\
%installerex         &    grayware &         0.950 &      0.00 \\
%offergenerator      &    grayware &         0.951 &      0.00 \\
%firseria            &    grayware &         0.951 &      0.08 \\
%screenmate          &    grayware &         0.951 &      0.01 \\
%tufik               &       virus &         0.951 &      0.00 \\
%chir                &        worm &         0.951 &      0.12 \\
%speedcat            &    grayware &         0.953 &      0.00 \\
%shiz                &    backdoor &         0.953 &      0.00 \\
%frosparf            &     clicker &         0.954 &      0.73 \\
%qihoo               &    grayware &         0.954 &      0.03 \\
%megasearch          &      adware &         0.955 &      0.00 \\
%duote               &      adware &         0.955 &      0.98 \\
%ibryte              &      adware &         0.955 &      0.09 \\
%domaiq              &    grayware &         0.956 &      0.53 \\
%zygug               &    grayware &         0.956 &      0.52 \\
%swisyn              &        worm &         0.956 &      0.07 \\
%daws                &  downloader &         0.956 &      0.02 \\
%installbrain        &    grayware &         0.956 &      0.02 \\
%vundo               &        worm &         0.957 &      0.89 \\
%xcnfe               &    grayware &         0.957 &      0.00 \\
%tinba               &  downloader &         0.958 &      0.15 \\
%downloadsponsor     &    grayware &         0.958 &      0.87 \\
%autog               &  downloader &         0.959 &      0.00 \\
%icloader            &    grayware &         0.959 &      0.02 \\
%veil                &    grayware &         0.960 &      0.01 \\
%lecna               &    backdoor &         0.960 &      0.24 \\
%downloadassistant   &    grayware &         0.960 &      0.18 \\
%mewsspy             &    backdoor &         0.960 &      0.06 \\
%regsup              &  downloader &         0.960 &      0.01 \\
%kuaizip             &      adware &         0.960 &      0.01 \\
%bublik              &  downloader &         0.961 &      0.79 \\
%simbot              &    backdoor &         0.961 &      0.01 \\
%vobfus              &        worm &         0.961 &      0.00 \\
%lunastorm           &        worm &         0.962 &      0.97 \\
%sohana              &  downloader &         0.962 &      0.18 \\
%downloadadmin       &    grayware &         0.962 &      0.03 \\
%filetour            &    grayware &         0.962 &      0.04 \\
%reptile             &    grayware &         0.963 &      0.00 \\
%kolweb              &    grayware &         0.963 &      0.96 \\
%pacex               &       miner &         0.964 &      0.00 \\
%xolxo               &        worm &         0.964 &      0.99 \\
%axespec             &    grayware &         0.964 &      0.02 \\
%betload             &    grayware &         0.965 &      0.03 \\
%kolab               &    grayware &         0.965 &      0.01 \\
%lydra               &     spyware &         0.965 &      0.05 \\
%idsohtu             &    grayware &         0.965 &      0.06 \\
%wapomi              &       virus &         0.966 &      0.08 \\
%miniduke            &    backdoor &         0.966 &      0.00 \\
%wannacry            &  ransomware &         0.966 &      0.01 \\
%wakme               &  downloader &         0.966 &      0.00 \\
%plurox              &    backdoor &         0.967 &      0.00 \\
%phorpiex            &        worm &         0.967 &      0.12 \\
%koutodoor           &    backdoor &         0.967 &      0.16 \\
%webcompanion        &    grayware &         0.967 &      0.00 \\
%installmonster      &    grayware &         0.967 &      0.83 \\
%protux              &    backdoor &         0.967 &      0.04 \\
%blackshades         &        worm &         0.967 &      0.02 \\
%detrahere           &    grayware &         0.968 &      0.04 \\
%rostpay             &    grayware &         0.969 &      0.96 \\
%moarider            &        worm &         0.969 &      0.98 \\
%gofot               &  downloader &         0.970 &      0.88 \\
%growtopia           &    grayware &         0.970 &      0.69 \\
%fesber              &        worm &         0.970 &      0.33 \\
%sytro               &        worm &         0.971 &      0.45 \\
%bayrob              &     spyware &         0.971 &      0.01 \\
%spyrix              &    grayware &         0.971 &      0.56 \\
%cosmu               &       virus &         0.972 &      0.00 \\
%shipup              &  downloader &         0.973 &      0.30 \\
%lmir                &       virus &         0.973 &      0.02 \\
%4shared             &    grayware &         0.973 &      0.01 \\
%snojan              &  downloader &         0.973 &      0.01 \\
%broskod             &  downloader &         0.974 &      0.01 \\
%socelars            &     spyware &         0.974 &      0.01 \\
%egroupdial          &    grayware &         0.974 &      0.87 \\
%dinwod              &  downloader &         0.974 &      0.98 \\
%havex               &    grayware &         0.974 &      0.00 \\
%dstudio             &    grayware &         0.974 &      0.02 \\
%memery              &       virus &         0.974 &      0.09 \\
%vrbrothers          &      adware &         0.975 &      0.88 \\
%alyak               &  downloader &         0.975 &      0.55 \\
%mooqkel             &  downloader &         0.975 &      1.00 \\
%mocrt               &     spyware &         0.975 &      0.73 \\
%bundlore            &      adware &         0.976 &      0.02 \\
%anmalpro            &    grayware &         0.976 &      0.00 \\
%getnow              &    grayware &         0.976 &      0.88 \\
%qqhack              &        tool &         0.976 &      0.98 \\
%webdialer           &      dialer &         0.976 &      0.86 \\
%maener              &       miner &         0.976 &      0.00 \\
%wecod               &     spyware &         0.976 &      0.94 \\
%expressdownloader   &    grayware &         0.976 &      0.62 \\
%unruy               &  downloader &         0.976 &      0.13 \\
%dexel               &  downloader &         0.977 &      0.00 \\
%reconyc             &    grayware &         0.977 &      0.36 \\
%installiq           &    grayware &         0.977 &      0.02 \\
%bcryptinject        &  downloader &         0.977 &      0.00 \\
%ceatrg              &  downloader &         0.978 &      0.66 \\
%tougle              &    grayware &         0.978 &      0.00 \\
%pajetbin            &        worm &         0.978 &      0.91 \\
%neshta              &       virus &         0.978 &      0.02 \\
%webalta             &    grayware &         0.979 &      0.05 \\
%lipler              &  downloader &         0.979 &      0.00 \\
%mira                &        worm &         0.979 &      0.23 \\
%aauto               &    grayware &         0.979 &      0.56 \\
%plingky             &  downloader &         0.980 &      0.93 \\
%cardspy             &     spyware &         0.980 &      1.00 \\
%banload             &       miner &         0.980 &      0.49 \\
%macoute             &        worm &         0.980 &      0.00 \\
%cjishu              &      adware &         0.980 &      0.01 \\
%kuaiba              &      adware &         0.980 &      0.05 \\
%slimware            &    grayware &         0.981 &      0.00 \\
%inbox               &    grayware &         0.981 &      0.00 \\
%airinstaller        &    grayware &         0.981 &      0.87 \\
%bloored             &        worm &         0.981 &      0.00 \\
%kingsoft            &    grayware &         0.981 &      0.37 \\
%youxun              &    grayware &         0.982 &      0.11 \\
%mediaget            &    grayware &         0.982 &      0.33 \\
%qjwmonkey           &    grayware &         0.982 &      0.47 \\
%disttrack           &    grayware &         0.983 &      0.00 \\
%softonic            &      adware &         0.983 &      0.79 \\
%fasong              &        worm &         0.983 &      0.78 \\
%safebytes           &    grayware &         0.984 &      0.99 \\
%babonock            &        worm &         0.984 &      0.00 \\
%goldrv              &        worm &         0.984 &      0.00 \\
%detroie             &       virus &         0.984 &      0.02 \\
%gobot               &    backdoor &         0.985 &      0.04 \\
%cosmicduke          &    backdoor &         0.985 &      0.04 \\
%openinstall         &    grayware &         0.985 &      0.22 \\
%paneidix            &    backdoor &         0.985 &      0.00 \\
%rising              &    grayware &         0.985 &      0.34 \\
%gepys               &  downloader &         0.986 &      0.00 \\
%ksdler              &      adware &         0.986 &      0.69 \\
%hebchengjiu         &      adware &         0.986 &      0.07 \\
%lolbot              &        worm &         0.986 &      0.00 \\
%cheatengine         &    grayware &         0.986 &      0.00 \\
%zvuzona             &    grayware &         0.986 &      0.79 \\
%outbyte             &    grayware &         0.987 &      0.04 \\
%laqma               &    grayware &         0.987 &      0.12 \\
%winloadsda          &    grayware &         0.987 &      0.86 \\
%powerless           &  downloader &         0.987 &      0.10 \\
%sillyp2p            &        worm &         0.987 &      0.01 \\
%agentino            &  downloader &         0.987 &      0.00 \\
%tupym               &        worm &         0.987 &      0.00 \\
%agentcrypt          &    grayware &         0.987 &      0.00 \\
%seven               &  ransomware &         0.987 &      0.00 \\
%kronosbot           &    backdoor &         0.987 &      0.00 \\
%dumpy               &        worm &         0.988 &      0.00 \\
%cmy3u               &    grayware &         0.988 &      0.98 \\
%elemental           &    grayware &         0.988 &      0.00 \\
%aenjaris            &    grayware &         0.988 &      0.00 \\
%dluca               &  downloader &         0.988 &      0.84 \\
%oberal              &  downloader &         0.988 &      0.00 \\
%antavmu             &        worm &         0.988 &      0.00 \\
%konus               &    backdoor &         0.989 &      0.00 \\
%apost               &  downloader &         0.989 &      0.01 \\
%virlock             &       virus &         0.989 &      0.00 \\
%addlyrics           &      adware &         0.989 &      0.00 \\
%viking              &       virus &         0.989 &      0.98 \\
%gippers             &  ransomware &         0.990 &      0.00 \\
%pluto               &        worm &         0.990 &      0.34 \\
%virfire             &        worm &         0.990 &      0.00 \\
%stone               &       virus &         0.990 &      0.97 \\
%connectwise         &        tool &         0.991 &      0.00 \\
%downer              &    grayware &         0.991 &      0.96 \\
%mailru              &    grayware &         0.991 &      0.00 \\
%lassorm             &        worm &         0.991 &      0.00 \\
%bzub                &  downloader &         0.991 &      0.02 \\
%pedex               &    backdoor &         0.991 &      1.00 \\
%lulusoftware        &    grayware &         0.992 &      0.13 \\
%pondfull            &        worm &         0.992 &      0.05 \\
%pistolar            &  downloader &         0.992 &      0.76 \\
%gorillaprice        &      adware &         0.992 &      0.06 \\
%taskloader          &      adware &         0.993 &      0.00 \\
%brontok             &        worm &         0.993 &      0.95 \\
%winner              &    grayware &         0.993 &      0.00 \\
%vkontaktedj         &    grayware &         0.994 &      0.04 \\
%hafen               &    grayware &         0.994 &      0.00 \\
%gigex               &        worm &         0.994 &      0.00 \\
%clipspy             &    grayware &         0.994 &      0.02 \\
%eyoorun             &    grayware &         0.995 &      0.00 \\
%lunam               &        worm &         0.995 &      0.99 \\
%tisandr             &        worm &         0.995 &      0.00 \\
%fakens              &      adware &         0.995 &      0.00 \\
%roxer               &    grayware &         0.995 &      0.97 \\
%gamemodding         &    grayware &         0.996 &      0.06 \\
%goabeny             &    grayware &         0.996 &      0.75 \\
%jevafus             &  downloader &         0.996 &      0.45 \\
%offercore           &    grayware &         0.996 &      0.00 \\
%pahooka             &        worm &         0.996 &      1.00 \\
%salgorea            &  downloader &         0.996 &      0.00 \\
%zepfod              &        worm &         0.997 &      0.00 \\
%qqpass              &  downloader &         0.997 &      0.94 \\
%lolojan             &    grayware &         0.998 &      0.95 \\
%pochi               &        worm &         0.998 &      0.00 \\
%mydoom              &        worm &         0.998 &      0.83 \\
%allaple             &        worm &         0.999 &      0.00 \\
%socks               &        worm &         0.999 &      0.18 \\
%xihet               &  downloader &         0.999 &      0.08 \\
%tempedreve          &       virus &         0.999 &      0.00 \\
%griptolo            &        worm &         0.999 &      0.07 \\
%shyape              &  downloader &         0.999 &      0.39 \\
%sivis               &       virus &         0.999 &      0.72 \\
%wabot               &    backdoor &         0.999 &      0.19 \\
%moonlight           &        worm &         0.999 &      0.08 \\
%prepscram           &    grayware &         1.000 &      1.00 \\
%grenam              &       virus &         1.000 &      0.00 \\
%phishbank           &        worm &         1.000 &      0.00 \\
%coroxy              &    backdoor &         1.000 &      0.00 \\
%jeefo               &       virus &         1.000 &      0.99 \\
%zylom               &  downloader &         1.000 &      0.00 \\
%hebogo              &    grayware &         1.000 &      0.00 \\
%loring              &        worm &         1.000 &      1.00 \\
%rums                &  downloader &         1.000 &      0.00 \\
%pykspa              &        worm &         1.000 &      0.00 \\
%fakedoc             &        worm &         1.000 &      0.00 \\
%houndhack           &    backdoor &         1.000 &      1.00 \\
%diamin              &      dialer &         1.000 &      0.80 \\
%syncopate           &    grayware &         1.000 &      0.20 \\
%drstwex             &  downloader &         1.000 &      0.00 \\
%enosch              &        worm &         1.000 &      0.00 \\
%neojit              &  downloader &         1.000 &      0.00 \\
%blihan              &    backdoor &         1.000 &      0.00 \\
%sfone               &        worm &         1.000 &      0.65 \\
%cambot              &        worm &         1.000 &      0.00 \\
%qaccel              &     clicker &         1.000 &      0.00 \\
%shodi               &       virus &         1.000 &      0.00 \\
%mimdau              &  downloader &         1.000 &      1.00 \\
%burn                &    backdoor &         1.000 &      0.00 \\
%mimail              &        worm &         1.000 &      0.00 \\
%mapsgory            &  downloader &         1.000 &      0.00 \\
%catalina            &    grayware &         1.000 &      0.00 \\
%adaebook            &    grayware &         1.000 &      1.00 \\
%nevereg             &        worm &         1.000 &      0.51 \\
%recodrop            &  downloader &         1.000 &      0.00 \\
%adposhel            &    grayware &         1.000 &      0.00 \\
%primecasino         &    grayware &         1.000 &      0.00 \\
%powerspider         &    backdoor &         1.000 &      0.00 \\
%regrun              &  ransomware &         1.000 &      1.00 \\
%plemood             &        worm &         1.000 &      0.00 \\
%berbew              &    backdoor &         1.000 &      0.00 \\
%rifdoor             &    backdoor &         1.000 &      0.00 \\
%picsys              &        worm &         1.000 &      1.00 \\
%amigo               &    grayware &         1.000 &      0.00 \\
%ruledor             &    backdoor &         1.000 &      0.00 \\
%atcpa               &       virus &         1.000 &      0.00 \\
%rungbu              &        worm &         1.000 &      0.18 \\
%sinau               &       virus &         1.000 &      0.00 \\
%rikihaki            &        worm &         1.000 &      0.00 \\
%obit                &  downloader &         1.000 &      0.00 \\
%triusor             &       virus &         1.000 &      0.00 \\
%wenper              &        worm &         1.000 &      0.42 \\
%dpsk                &       miner &         1.000 &      1.00 \\
%drolnux             &        worm &         1.000 &      0.00 \\
%dropware            &      adware &         1.000 &      0.01 \\
%vbclone             &  downloader &         1.000 &      0.00 \\
%gator               &      adware &         1.000 &      0.47 \\
%gametea             &  downloader &         1.000 &      1.00 \\
%eggnog              &        worm &         1.000 &      0.00 \\
%finfish             &    backdoor &         1.000 &      0.00 \\
%updane              &    grayware &         1.000 &      0.00 \\
%esaprof             &  downloader &         1.000 &      0.84 \\
%upantix             &  downloader &         1.000 &      1.00 \\
%facido              &  downloader &         1.000 &      0.00 \\
%umbra               &  downloader &         1.000 &      0.00 \\
%esecn               &      adware &         1.000 &      1.00 \\
%ezsoftwareupdater   &    grayware &         1.000 &      0.00 \\
%downloadguide       &    grayware &         1.000 &      0.00 \\
%geegly              &       virus &         1.000 &      1.00 \\
%gogo                &       virus &         1.000 &      0.00 \\
%dostre              &  downloader &         1.000 &      0.00 \\
%ludbaruma           &        worm &         1.000 &      0.00 \\
%chrop               &      adware &         1.000 &      0.63 \\
%lebreat             &    grayware &         1.000 &      1.00 \\
%trymedia            &      adware &         1.000 &      0.73 \\
%wavipeg             &    backdoor &         1.000 &      0.00 \\
%krol                &        worm &         1.000 &      0.00 \\
%keydoor             &     spyware &         1.000 &      0.00 \\
%lyposit             &  ransomware &         1.000 &      0.00 \\
%jpgiframe           &    grayware &         1.000 &      0.00 \\
%vybab               &        worm &         1.000 &      0.00 \\
%itorrent            &    grayware &         1.000 &      0.00 \\
%vtflooder           &  downloader &         1.000 &      0.55 \\
%inlog               &  downloader &         1.000 &      0.00 \\
%stormattack         &  downloader &         1.000 &      0.00 \\
%digs                &       miner &         1.000 &      0.00 \\
%swjoy               &    grayware &         1.000 &      0.00 \\
%contenedor          &       virus &         1.000 &      0.00 \\
%soulclose           &        worm &         1.000 &      0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_multiclass_featImportance.tex <==
\begin{table}[h]
\centering
\caption{Feature importance forfamily-classification.}
% Feature importance is measured using an average MDI score in range [0,100]
% with higher being more important.}
\label{tbl:multiclass_featImportance}
\begin{tabular}{lrrr}
\toprule
%\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Importance}} \\
\textbf{Feature Class} & \textbf{Combined} & \textbf{Static} & \textbf{Dynamic} \\
\midrule
s-bytegrams    &  38.60 & 41.67 &     - \\
s-opcodegrams  &  23.48 & 20.87 &     - \\
s-strings      &  17.62 & 19.27 &     - \\
s-imports      &   7.87 &  9.30 &     - \\
s-sections     &   5.62 &  6.48 &     - \\
d-file         &   3.16 &     - & 56.20 \\
d-process      &   0.87 &     - & 30.70 \\
s-headers      &   0.73 &  0.96 &     - \\
s-dll          &   0.52 &  0.57 &     - \\
d-registry     &   0.51 &     - &  0.60 \\
s-file         &   0.39 &  0.87 &     - \\
d-network      &   0.35 &     - &  3.70 \\
d-thread       &   0.16 &     - &  5.26 \\
d-service      &   0.07 &     - &  2.39 \\
d-mutex        &   0.03 &     - &  1.19 \\
\bottomrule
\end{tabular}
\end{table}



==> tbl/tbl_multiclass_featImportance_combined.tex <==
\begin{table}[h]
\centering
\caption{Importance of each feature class in the family classification combined model.}
\label{tbl:multiclass_combined_featImportance}
\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Importance} \\
\midrule
s-bytegrams    &  38.60 \\
s-opcodegrams	 &  23.48 \\
s-strings      &  17.62 \\
s-imports      &   7.87 \\
s-sections     &   5.62 \\
d-file         &   3.16 \\
d-process      &   0.87 \\
d-headers      &   0.73 \\
s-dll          &   0.52 \\
d-registry     &   0.51 \\
s-file         &   0.39 \\
d-network      &   0.35 \\
d-thread       &   0.16 \\
d-service      &   0.07 \\
d-mutex        &   0.03 \\
\bottomrule
\end{tabular}
\end{table}



==> tbl/tbl_multiclass_featImportance_dynamic.tex <==
\begin{table}[h]
\centering
\caption{Importance of each feature class in the family classification dynamic model.}
\label{tbl:family_FeatImportance_dynamic}
\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Importance} \\
\midrule
d-file      & 56.20 \\
d-process   & 30.70 \\
d-thread    &  5.26 \\
d-network   &  3.70 \\
d-service   &  2.39 \\
d-mutex     &  1.19 \\
d-registry  &  0.60 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_multiclass_featImportance_static.tex <==
\begin{table}
\centering
\caption{Importance of each feature class in the family classification static model.}
\label{tbl:multiclass_static_featImportance}
\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Importance} \\
\midrule
s-bytegrams  	&  41.67 \\
s-opcodegrams &  20.87 \\
s-strings  		&  19.27 \\
s-imports  		&   9.30 \\
s-sections 		&   6.48 \\
s-file  		  &   0.87 \\
s-headers   	&   0.96 \\
s-dll    		  &   0.57 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_multiclass_no_packed_featImportance_static.tex <==
\begin{table}
\centering
\caption{Feature importance for family classification when excluding packed files.}
\label{tbl:multiclass_no_packed_static_featImportance}
\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Importance} \\
\midrule
s-bytegrams  	&  38.59 \\
s-opcodegrams   &  25.02 \\
s-strings  		&  17.80 \\
s-imports  		&  10.17 \\
s-sections 		&  6.09 \\
s-file  		&  1.17 \\
s-headers   	&  0.78 \\
s-dll    		&  0.36 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/tbl_multiclass_packedOnly_featImportance_static.tex <==
\begin{table}
\centering
\caption{Feature importance for family classification when only considering packed files.}
\label{tbl:multiclass_packed_only_static_featImportance}
\begin{tabular}{lr}
\toprule
\textbf{Feature Class} &  \textbf{Importance} \\
\midrule
s-bytegrams  	&  53.66 \\
s-strings  		&  18.17 \\
s-opcodegrams   &  9.95  \\
s-sections 		&  9.39  \\
s-imports  		&  5.32  \\
s-headers   	&  1.30  \\
s-file  		&  1.29  \\
s-dll    		&  0.91  \\
\bottomrule
\end{tabular}
\end{table}











